The Role of Compute in Autonomous Aerial Vehicles

Autonomous-mobile cyber-physical machines are part of our future. Specifically, unmanned-aerial-vehicles have seen a resurgence in activity with use-cases such as package delivery. These systems face many challenges such as their low-endurance caused by limited onboard-energy, hence, improving the mission-time and energy are of importance. Such improvements traditionally are delivered through better algorithms. But our premise is that more powerful and efficient onboard-compute should also address the problem. This paper investigates how the compute subsystem, in a cyber-physical mobile machine, such as a Micro Aerial Vehicle, impacts mission-time and energy. Specifically, we pose the question as what is the role of computing for cyber-physical mobile robots? We show that compute and motion are tightly intertwined, hence a close examination of cyber and physical processes and their impact on one another is necessary. We show different impact paths through which compute impacts mission-metrics and examine them using analytical models, simulation, and end-to-end benchmarking. To enable similar studies, we open sourced MAVBench, our tool-set consisting of a closed-loop simulator and a benchmark suite. Our investigations show cyber-physical co-design, a methodology where robot's cyber and physical processes/quantities are developed with one another consideration, similar to hardware-software co-design, is necessary for optimal robot design.

==> tex/MAVBench.tex <==

\section{Benchmark Suite} 
\label{sec:mavbench}




To quantify the energy and performance demands of typical MAV applications and understand the cyber-physical interactions, we created a set of workloads that we compiled into a benchmark suite.
By combining this suite with our simulation setup, we get to study the robot's end-to-end behavior from both cyber and physical perspective, and further investigate various compute optimization techniques for MAV applications.
Our benchmarks run on top of our closed-loop simulation environment. 

% The suite aims to cover a wide range of representative applications. 

Each workload is an \textit{end-to-end} application that allows us to study the kernels' impact on the whole application as well as to investigate the interactions and dependencies between kernel. 
By providing holistic end-to-end applications instead of only focusing on individual kernels, MAVBench allows for the examination of kernels' impacts and their optimization at the application level. This is a lesson learned from Amdahl's law, which recognizes that the true impact of a component's improvement needs to be evaluated globally rather than locally.



The MAVBench workloads have different computational kernels, as shown in Table~\ref{kernel_makeup}. MAVBench aims at being comprehensive by (1) selecting applications that target different robotic domains (robotics in hazardous areas, construction, etc.) and (2) choosing kernels (e.g., point cloud, RRT) common across a range of applications, not limited to our benchmark-suite. The computational kernels (OctoMaps, RTT, etc.) that we use in the benchmarks are the building blocks of many robotics applications, and hence, they are platform agnostic. We present a high-level software pipeline associated (though not exclusive) to our workloads. Then, we provide functional summaries of the workloads in MAVBench, their use cases, and mappings from each workload to the high-level software pipeline. We describe in detail the prominent computational kernels that are incorporated into our workloads. Finally, we provide a short discussion regarding the Quality-of-Flight (QoF) metrics with which we can evaluate MAV applications success and further the role of compute.

 \begin{figure*}[t]
\centering
\includegraphics[height=1.65in, keepaspectratio]{figs/software_pipeline}
\caption{High-level application pipeline for a typical MAV application. The upper row presents a universal pipeline that all our MAVBench applications follow, which involves \emph{perception}, \emph{planning} and \emph{control}. The lower row presents how a specific workload in MAVBench (e.g. package delivery) maps to the universal high-level application pipeline.}
\label{fig:software_pipeline}
\end{figure*}

% Our insights carry over to rotorcraft UAVs and AUVs (Autonomous underwater vehicles), since in both cases constant power is required to maintain the position. Furthermore, ground mobile robots under high energy constraints can also exploit principles presented.


% Application architecture section
% Add low-level details like which kernels we use
% Mention that we have flexibility
% Add small details like SLAM-backtracking, Octomap, ROS
% Add new paragraphs after every benchmark
% Some analysis of benchmarks (length of runtime, number of ROS nodes)
% Literature survey (PARSEC, BioBench, WHISPER)
% Add annotated graphics to system architecture showing sensors
% Draw an end-to-end diagram or a table
% Talk about core kernels to foreshadow future characterization
%\subsection{Application Dataflow} \label{sec:sw_pipeline}

%In \Sec{sec:benchmarks}, we present functional summaries of the workloads in MAVBench, their use cases, and mappings from each workload to the high level software pipeline provided in
%section~\ref{sec:task_flow}. In \Sec{sec:kernels}, we describe in details of the prominent computational kernels that are incorporated into our workloads, and finally in \Sec{sec:QoF} we provide a short discussion regarding the Quality-of-Flight (QoF) metrics to evaluate MAV applications.

%The MAVBench workloads have different computational kernels, as shown in Table~\ref{kernel_makeup}. MAVBench aims at being comprehensive by (1) selecting applications that target different robotic domains (robotics in hazardous areas, construction, etc.) and (2) choosing kernels (e.g., point cloud, RRT) common across a range of applications, not limited to our benchmark-suite. The computational kernels (OctoMaps, RTT, etc.) that we use in the benchmarks are the building blocks of many robotics applications, and hence, they are platform agnostic. 

% Our insights carry over to rotorcraft UAVs and AUVs (Autonomous underwater vehicles), since in both cases constant power is required to maintain the position. Furthermore, ground mobile robots under high energy constraints can also exploit principles presented.


% Application architecture section
% Add low-level details like which kernels we use
% Mention that we have flexibility
% Add small details like SLAM-backtracking, Octomap, ROS
% Add new paragraphs after every benchmark
% Some analysis of benchmarks (length of runtime, number of ROS nodes)
% Literature survey (PARSEC, BioBench, WHISPER)
% Add annotated graphics to system architecture showing sensors
% Draw an end-to-end diagram or a table
% Talk about core kernels to foreshadow future characterization


%\subsection{Application Dataflow} \label{sec:sw_pipeline}



\subsection{Workloads and Their Data Flow} \label{sec:benchmarks}
The benchmark suite consists of five workloads, each equipped with the flexibility to configure its computational kernel composition (described later in \Sec{sec:kernels}).
%\red{Although only containing 5 end-to-end applications, MAVBench has 13 computationally intensive kernels (table blah). MAVBench aims at being comprehensive by 1.selecting applications carefully such that each targets a different robotic's domain (e.g., Robotics in Hazardous Applications, Construction, ...) 2. selecting kernels (e.g., point cloud, RRT, ...) common across a wide range of applications and not limited to our benchmark-suite.  
%We also believe that by providing end-to-end applications instead individual kernels (cite paper blah and blah), MAVBench allows for examination of  kernels' impacts and their optimization at the application level. This is a lesson learned from  Amdahl's law, which recognizes that the true impact of a component's improvement needs to be evaluated globally rather than locally.} 
The following section sheds light on the high-level data flow governing all the applications, each application's functional summary, and finally, the inner workings of these workloads as per the three-stage high-level application pipeline. 

There are three fundamental processing stages in each application: \emph{Perception}, \emph{Planning} and \emph{Control}. In the perception stage, the sensory data is processed to extract relevant states from the environment and the drone. This information is fed into the next two stages (i.e., planning and control). Planning ``plans'' flight motions and forwards them to the actuators in the control subsystem. \Fig{fig:software_pipeline} summarizes this high-level software pipeline, which each of our workloads embodies.

\textbf{Perception:}
It is defined as ``the task-oriented interpretation of sensor data''~\cite{Handbook_robotic}. Inputs to this stage, such as sensory data from cameras or depth sensors, are fused to develop an elaborate model in order to extract the MAV's and its environment's relevant states (e.g., the positions of obstacles around the MAV). This stage may include tasks such as Simultaneous Localization and Mapping (SLAM) that enables the MAV to infer its position in the absence of GPS data.

\textbf{Planning:}
 Planning generates a \textit{collision-free} path to a target using the output of the perception (e.g., an occupancy map of obstacles in the environment). In short, this step involves first generating a set of possible paths to the target, such as by using the probabilistic roadmap (PRM) algorithm and then choosing an optimal one among them using a path-planning algorithm, such as A*.

\textbf{Control:}
This stage is about following the desired path, which is absorbed from the previous stage while providing a set of guarantees such as feasibility, stability, and robustness~\cite{tech_problem}. In this stage, the MAV's kinematics and dynamics are considered, such as by smoothening paths to avoid high-acceleration turns, and then, finally, the flight commands are generated (e.g., by flight controllers such as the PX4) while ensuring the aforementioned guarantees are still respected.

\Fig{fig:bench_screenshot} presents screenshots of our workloads. The application dataflows are shown in \Fig{fig:benchmarks_data_flow}. Note that all the workloads follow the perception, planning, and control pipeline mentioned previously. For the ease of the reader, we have also labeled the data flow with these stages accordingly.

\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{1.385in}
        \centering
        \includegraphics[width=\textwidth, height=1in]{figs/benchmarks/scanning.jpg}
        \caption{Scanning.}\label{fig:benchmarks:scanning}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{1.385in}
        \centering
        \includegraphics[width=\textwidth, height=1in]{figs/benchmarks/aerial-photo.jpg}
        \caption{Aerial Photography.}\label{fig:benchmarks:aerial-photo}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{1.385in}
        \centering
        \includegraphics[width=\textwidth, height=1in]{figs/benchmarks/package-delivery.jpg}
        \caption{Package Delivery.}\label{fig:benchmarks:package-delivery}
    \end{subfigure}
    \hfill
    %\vspace{4pt}
    \begin{subfigure}[t]{1.385in}
        \centering
        \includegraphics[width=\textwidth, height=1in]{figs/benchmarks/3d-mapping}
        \caption{3D Mapping.}\label{fig:benchmarks:3D-mapping}
    \end{subfigure}
    \hspace{28pt}
    %\hfill
    \begin{subfigure}[t]{1.385in}
        %\centering
        \includegraphics[width=\textwidth, height=1in]{figs/benchmarks/search-and-rescue.jpg}
        
        \caption{Search and Rescue.}\label{fig:benchmarks:search-and-rescue}
    \end{subfigure}
    \caption{MAVBench workloads. Each workload is an end-to-end application targeting both industry and research use cases. All figures are screenshots of a MAV executing a workload within its simulated environment. Fig.~\ref{fig:benchmarks:package-delivery} shows a MAV planning a trajectory to deliver a package. Fig.~\ref{fig:benchmarks:3D-mapping} shows a MAV sampling its environment in search of unexplored areas to map.}
    \label{fig:bench_screenshot}
\end{figure*}

\begin{figure}[t!]
    \centering
    \vspace{-54pt}
    \begin{subfigure}[t]{.725\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figs/data_flow/scanning}
        \vspace{-35pt}
    \caption{Scanning.}
    \label{fig:benchmarks:data-flow:scanning}
    \end{subfigure}
    \begin{subfigure}[t]{.725\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figs/data_flow/aerial_photography}
        \vspace{-25pt}
        \caption{Aerial Photography.}\label{fig:benchmarks:data-flow:aerial_photography}
    \end{subfigure}
    \begin{subfigure}[t]{.725\columnwidth}
    \centering
        \includegraphics[width=\columnwidth] {figs/data_flow/package_delivery}
        \vspace{-20pt}
        \caption{Package Delivery.}\label{fig:benchmarks:data-flow:package_deilvery}
    \end{subfigure}
    \begin{subfigure}[t]{.725\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figs/data_flow/mapping}
        \vspace{-20pt}
        \caption{3D Mapping.}
        \label{fig:benchmarks:data-flow:mapping}
    \end{subfigure}
    \begin{subfigure}[t]{.725\columnwidth}
    \vspace{-5pt}
        \centering
        \includegraphics[width=\columnwidth]{figs/data_flow/sar}
        \vspace{-25pt}
        \caption{Search and Rescue.}\label{fig:benchmarks:data-flow:sar}
    \vspace{1pt}
    \end{subfigure}
    \caption{\footnotesize Application dataflows. Circles and arrows denote nodes and their communications respectively. Subscriber/publisher communication paradigm is denoted with filled black arrows whereas client/server with dotted red ones. Dotted black arrows denote various localization techniques.}
    \label{fig:benchmarks_data_flow}
\end{figure}

\textbf{Scanning:} In this simple though popular use case, a MAV scans an area specified by its width and length while collecting sensory information about conditions on the ground. It is a common agricultural use case. For example, a MAV may fly above a farm to monitor the health of the crops below. To do so, the MAV first uses GPS sensors to determine its location (Perception). Then, it plans an energy efficient ``lawnmower path'' over the desired coverage area, starting from its initial position (Planning). Finally, it closely follows the planned path (Control). While in-flight, the MAV can collect data on ground conditions using onboard sensors, such as cameras or LIDAR. 


%This workloads QOS can be defined as both the mission time and the energy consumption of the mission.

\textbf{Aerial Photography:} Drone aerial photography is an increasingly popular use of MAVs for entertainment, as well as businesses. In this workload, we design the MAV to follow a moving target with the help of computer vision algorithms. The MAV uses a combination of object detection and tracking algorithms to identify its relative distance from a target (Perception). Using a PID controller, it then plans motions to keep the target near the center of the MAV's camera frame (Planning), before executing the planned motions (Control).
%The workload's QOS can be defined as average distance of the target from the center of camera frame. 

\textbf{Package Delivery:} In this workload, a MAV navigates through an obstacle-filled environment to reach some arbitrary destination, deliver a package and come back to its origin. Using a variety of sensors such as RGBD cameras or GPS, the MAV creates an occupancy map of its surroundings (Perception). Given this map and its desired destination coordinate, it plans an efficient collision-free path. To accommodate for the feasibility of maneuvering, the path is further smoothened to avoid high-acceleration movements (Planning), before finally being followed by the MAV (Control). While flying, the MAV continuously updates its internal map of the surroundings to check for new obstacles and re-plans its path if any such obstacles obstruct its planned trajectory.
%QOS for this workload can consider both energy and mission time. 
%Additionally, the MAV is responsible for accurately localizing itself at all times, to determine its distance from its destination. If the MAV is outdoors, then this localization can easily be done using GPS, but in a GPS-denied environment, the MAV must instead rely upon SLAM algorithms such as ORB-SLAM2, which uses stereo or RGBD cameras, or VINS-MONO~\cite{vins-mono}, which uses a monocular camera paired with IMU data.

\textbf{3D Mapping:} With use cases in mining, architecture, and other industries, this workload instructs a MAV to build a 3D map of an unknown polygonal environment specified by its boundaries. To do so, as in package delivery, the MAV builds and continuously updates an internal map of the environment with both ``known'' and ``unknown'' regions (Perception). Then, to maximize the highest area coverage in the shortest time, the map is sampled, and a heuristic is used to select an energy efficient (i.e., short) path with a high exploratory promise (i.e., with many unknown areas along the edges) (Planning). Finally, the MAV follows this path (Control), until the area has been mapped.

%Note that if the MAV is in a GPS-denied environment, it will also have to simultaneously run SLAM algorithms to localize itself and its surrounding obstacles.
%QOS for this workload can be defined as a function of energy and mission time.
%The success of the application is determined by the time in which it can completely map its surroundings and the accuracy of the 3D map it builds.

\textbf{Search and Rescue:} MAVs are promising vehicles for search-and-rescue scenarios where victims must be found in the aftermath of a natural disaster. For example, in a collapsed building due to an earthquake, they can accelerate the search since they are capable of navigating difficult paths by flying over and around obstacles. In this workload, a MAV is required to explore an unknown area while looking for a target such as a human.  For this workload, the \textit{3D Mapping} application is augmented with an object detection machine-learning-based algorithm in the perception stage to constantly explore and monitor its environment until a human target is detected.

\subsection{Benchmark Kernels} \label{sec:kernels}

The workloads incorporate many computational kernels that can be grouped under the three pipeline stages described earlier in Section~\ref{sec:benchmarks}. Table~\ref{kernel_makeup} shows the kernel make up of MAVBench's workloads and their corresponding time profile (measured at 2.2 GHz, 4 cores enabled mode of Jetson TX2). MAVBench is equipped with multiple implementations of each computational kernel. For example, MAVBench comes equipped with both YOLO and HOG detectors that can be used interchangeably in workloads with object detection. The user can determine which implementations to use by setting the appropriate parameters. Furthermore, our workloads are designed with a ``plug-and-play'' architecture that maximizes flexibility and modularity, so the computational kernels described below can easily be replaced with newer implementations designed by researchers in the future.

%\begin{Export}
\renewcommand{\arraystretch}{1.15}
\begin{table*}[]
\centering
\caption{MAVBench applications and their kernel make up time profile in $ms$. The application suite, as a whole, exercises a variety of different computational kernels across the perception, planning and control stages, depending on their use case. Furthermore, within each of the kernel computational domain, applications have the flexibility to choose between different kernel implementations.}
\label{kernel_makeup}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\cline{2-14}
\multirow{3}{*}{}                                                                           & \multicolumn{8}{c|}{\textbf{Perception}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{4}{c|}{\textbf{Planning}}                                                                                                                                                                                                                                                                    & \textbf{Control}                                                                                 \\ \cline{2-14} 
                                                                                            & \multirow{2}{*}{\textit{\begin{tabular}[c]{@{}c@{}}Point Cloud\\ Generation\end{tabular}}} & \multirow{2}{*}{\textit{\begin{tabular}[c]{@{}c@{}}Occupancy Map\\ Generation\end{tabular}}} & \multirow{2}{*}{\textit{\begin{tabular}[c]{@{}c@{}}Collision\\ Check\end{tabular}}} & \multirow{2}{*}{\textit{\begin{tabular}[c]{@{}c@{}}Object\\ Detection\end{tabular}}} & \multicolumn{2}{c|}{\textit{\begin{tabular}[c]{@{}c@{}}Object\\ Tracking\end{tabular}}} & \multicolumn{2}{c|}{\textit{Localization}} & \multirow{2}{*}{\textit{PID}} & \multirow{2}{*}{\textit{\begin{tabular}[c]{@{}c@{}}Smoothened\\ Shortest Path\end{tabular}}} & \multirow{2}{*}{\textit{\begin{tabular}[c]{@{}c@{}}Frontier\\ Exploration\end{tabular}}} & \multirow{2}{*}{\textit{\begin{tabular}[c]{@{}c@{}}Smoothened \\Lawn Mowing\end{tabular}}} & \multirow{2}{*}{\textit{\begin{tabular}[c]{@{}c@{}}Path Tracking/\\ Command Issue\end{tabular}}} \\ \cline{6-9}
                                                                                            &                                                                                            &                                                                                              &                                                                                     &                                                                                      & \textit{Buffered}                          & \textit{Real Time}                         & \textit{GPS}        & \textit{SLAM}        &                               &                                                                                              &                                                                                          &                                                                                 &                                                                                                  \\ \hline
\multicolumn{1}{|c|}{\textbf{Scanning}}                                                     &                                                                                            &                                                                                              &                                                                                     &                                                                                      &                                            &                                            &                     &                      &                               &                                                                                              &                                                                                          & 89                                                                              & 1                                                                                                \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Aerial\\ Photography\end{tabular}}} &                                                                                            &                                                                                              &                                                                                     & 307                                                                                  & 80                                         & 18                                         & 0                   &                      & 0                             &                                                                                              &                                                                                          &                                                                                 & 1                                                                                                \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Package\\ Delivery\end{tabular}}}   & 2                                                                                          & 630                                                                                          & 1                                                                                   &                                                                                      &                                            &                                            & 0                   & 55                   &                               & 182                                                                                          &                                                                                          &                                                                                 & 1                                                                                                \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}3D\\ Mapping\end{tabular}}}         & 2                                                                                          & 482                                                                                          & 1                                                                                   &                                                                                      &                                            &                                            &              0       & 46                   &                               &                                                                                              & 2647                                                                                     &                                                                                 & 1                                                                                                \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Search and\\ Rescue\end{tabular}}}  & 2                                                                                          & 427                                                                                          & 1                                                                                   & 271                                                                                  &                                            &                                            &               0      & 45                   &                               &                                                                                              & 2693                                                                                     &                                                                                 & 1                                                                                                \\ \hline
\end{tabular}
}
\end{table*}
\renewcommand{\arraystretch}{1}

%\end{Export}
%\begin{table*}[t!]
%\centering
%\footnotesize
%\caption{MAVBench applications and their kernel make up time profile in $ms$. The application suite, as a whole, exercises a variety of different computational kernels across the perception, planning and control stages, depending on their use case. Furthermore, within each of the kernel computational domain, applications have the flexibility to choose between different kernel implementations.}
%\label{kernel_makeup}
%% Please add the following required packages to your document preamble:
%% \usepackage{multirow}
%\resizebox{1.01\columnwidth}{!}{
%\setlength{\extrarowheight}{9pt}
%\begin{tabular}{|l||c|c|c|c|c|l|c|c||l|c|c|c||c|}
%\hline
%\multirow{3}{*}{} & \multicolumn{8}{c||}{\textbf{Perception}} & \multicolumn{4}{c||}{\textbf{Planning}} & \textbf{Control} \\ \cline{2-14} 
% & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Point Cloud Generation}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Occupancy Map Generation}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Collision Check}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Object Detection}\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Object} \\\textbf{Tracking}\end{tabular}} & \multicolumn{2}{c||}{\textbf{Localization}} & \multirow{2}{*}{\textbf{PID}} & \multirow{2}{*}{\textbf{Smoothened Shortest Path}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Frontier Exploration}\end{tabular}} & \multirow{2}{*}{\textbf{Lawn Mowing}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Path Tracking/Command} \textbf{Issue} \end{tabular}} \\ \hline\hline
% \cline{6-9}
% &  &  &  &  & \multicolumn{1}{l|}{\textbf{Buffered}} & \textbf{Real Time} & \textbf{GPS} & 
%\textbf{SLAM} &  &  &  &  &  \\ \hline
%\textbf{Scanning} &  &  &  &  &  &  & 0 &  &  &  &  & 89 & 1 \\ \hline
%\begin{tabular}[c]{@{}l@{}}\textbf{Package Delivery}\end{tabular} & 2 & 630 & 1 &  &  &  & 0 & 55 &  & 182 &  &  & 1 \\ \hline
%\textbf{Mapping} & 2 & 482 & 1 &  &  &  & 0 & 46 &  &  & 2647 &  & 1 \\ \hline
%\textbf{Search and Rescue} & 2 & 427 & 1 & 271 &  &  & 0 & 45 &  &  & 2693 &  & 1 \\ \hline
%\textbf{Aerial Photography} &  &  &  & 307 & 80 & 18 & 0 &  & \multicolumn{1}{c|}{0} &  &  &  & 1 \\ \hline
%\end{tabular}
%}
%\end{table*}
%




\begin{comment}

\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|l|c|c||l|c|c|c||c|}
\hline
 & \multicolumn{8}{c||}{Perception} & \multicolumn{4}{c||}{Planning} & Control \\ \hline
 & \begin{tabular}[c]{@{}c@{}}Point Cloud\\  Generation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Occupancy\\ Map\\ Generation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Collision\\ Check\end{tabular} & \begin{tabular}[c]{@{}c@{}}Object\\  Detection\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Object\\ Tracking\end{tabular}} & \multicolumn{2}{c||}{Localization} & PID & Smoothened Shortest Path & \begin{tabular}[c]{@{}c@{}}Frontier\\ Exploration\end{tabular} & Lawn Mowing & \begin{tabular}[c]{@{}c@{}}Path Tracking/Command \\ Issue\end{tabular} \\ \hline
 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Buffered} & Real Time & GPS & SLAM &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l||}{} & \multicolumn{1}{l|}{} \\ \hline
Scanning &  &  &  &  &  &  & 0 &  &  &  &  & 89 & 1 \\ \hline
\begin{tabular}[c]{@{}l@{}}Package \\ Delivery\end{tabular} & 2 & 630 & 1 &  &  &  & 0 & X &  & 182 &  &  & 1 \\ \hline
Mapping & 2 & 482 & 1 &  &  &  & 0 & X &  &  & 2647 &  & 1 \\ \hline
Search and Rescue & 2 & 427 & 1 & 271 &  &  & 0 & X &  &  & 2693 &  & 1 \\ \hline
Aerial Photography &  &  &  & 307 & 80 & 18 & 0 &  & \multicolumn{1}{c|}{0} &  &  &  & 1 \\ \hline
\end{tabular}
}
\end{table*}
\end{comment}
\paragraph{Perception Kernels:} These are the computational kernels that allow a MAV application to interpret its surroundings.

\textit{Object Detection:} Detecting objects is an important kernel in numerous intelligent robotics applications. So, it is part of two MAVBench workloads: \textit{Aerial Photography} and \textit{Search and Rescue}. MAVBench comes pre-packaged with the YOLO~\cite{yolo16} object detector, and the standard OpenCV implementations of the HOG~\cite{hog} and Haar people detectors.

\textit{Tracking:}
%While object detectors attempt to identify all objects of a particular class within an image, 
It attempts to follow an instance of an object as it moves across a scene. 
%Tracking allows the MAV to follow a particular person in a crowd of other people. 
This kernel is used in the \textit{Aerial Photography} workload. MAVBench comes pre-packaged with a C++ implementation~\cite{kcf-c++} of a KCF~\cite{kcf} tracker.

\textit{Localization:} MAVs must determine their position. There are many ways that have been devised to enable localization, using a variety of different sensors, hardware, and algorithmic techniques. MAVBench comes pre-packaged with multiple localization solutions that can be used interchangeably for benchmark applications. Examples include a simulated GPS, visual odometry algorithms such as ORB-SLAM2~\cite{orbslam2}, and VINS-Mono~\cite{vins-mono} and these are accompanied with ground-truth data that can be used when a MAVBench user wants to test an application with perfect localization data.

%Localization may sometimes fail, such as when a SLAM algorithm fails to calculate a MAV's position correctly. To account for such cases, in MAVBench applications we include several SLAM recovery methods. If a SLAM algorithm fails during flight, the MAV will attempt to slowly backtrack over its previous trajectory, until it reaches an area that its SLAM algorithm will recognize. If backtracking is unsuccessful, then the application will simply reset its SLAM map, in a last attempt to regain its localization capabilities. If after a reset, the application is unable to successfully re-initialize its SLAM capabilities, then the application run will end in failure.

\textit{Occupancy Map Generation:} Several MAVBench workloads, like many other robotics applications, model their environments using internal 3D occupancy maps that divide a drone's surroundings into occupied and unoccupied space. Noisy sensors are accounted for by assigning probabilistic values to each unit of space.
%are often noisy and imprecise, MAVBench's occupancy maps also incorporate uncertainty readings to build probabilistic 3D maps that enable them to model surrounding obstacles. 
In MAVBench we use OctoMap~\cite{octomap} as our occupancy map generator since it provides updatable, flexible and compact 3D maps.
%OctoMap also has the advantage of modeling known and unknown space, in addition to occupied and unoccupied space, which makes it suitable for the \textit{Exploration} and \textit{Search and Rescue} workloads.

\paragraph{Planning Kernels:} Our workloads comprise several motion-planning techniques, from simple ``lawnmower" path planning to more sophisticated sampling-based path-planners, such as RRT~\cite{rrt} or PRM~\cite{prm} paired with the A*~\cite{astar} algorithm. We divide MAVBench's path-planning kernels into three categories: \textit{shortest-path planners}, \textit{frontier-exploration planners}, and \textit{lawnmower path planners}. The planned paths are further smoothened using the \textit{path smoothening} kernel. 

%Here, we describe two computationally-significant types of motion planners that are utilized in MAVBench: \textit{collision-free planners} and \textit{lawnmower path planners}.
% Motion-planning is an extremely broad, but extremely important kernel of MAV applications, as a MAV's main utility comes from its ability to fly through environments.

\textit{Shortest Path:} Shortest-path planners find collision-free flight trajectories that minimize the MAV's traveling distance. MAVBench comes pre-packaged with OMPL~\cite{ompl}, the Open Motion Planning Library, consisting of many state-of-the-art sampling-based motion planning algorithms. These algorithms provide collision-free paths from an arbitrary start location to an arbitrary destination. %Our PRM can be paired with either Dijkstra's algorithm or A*, based on user-defined parameters.

\textit{Frontier Exploration:} 
Some applications incorporate collision-free motion-planners that aim to efficiently ``explore'' all accessible regions in an environment, rather than simply moving from a single start location to a single destination as quickly as possible.
For these applications, MAVBench comes equipped with the official implementation of the exploration-based ``next best view planner''~\cite{nbvplanner}.

\textit{Lawnmower:} Some applications do not require complex, collision-checking path planners, e.g., agricultural MAVs fly over farms in a simple, lawnmower pattern, where the high-altitude of the MAV means that obstacles can be assumed to be nonexistent. For such applications, MAVBench comes with a simple path-planner that computes a regular pattern for covering rectangular areas.

\textit{Path Smoothening:} The motion planners discussed earlier return piecewise trajectories that are composed of straight lines with sharp turns. However, sharp turns require high accelerations from a MAV, consuming high amounts of energy (i.e., battery capacity). Thus, we use this kernel to convert these piecewise paths to smooth, polynomial trajectories that are more efficient for a MAV to follow.

\paragraph{Control Kernels:} The control stage of the pipeline enables the MAV to closely follow its planned motion trajectories in an energy-efficient, stable manner. 

\textit{Path Tracking:} MAVBench applications produce trajectories that have specific positions, velocities, and accelerations for the MAV to occupy at any particular point in time. However, due to mechanical constraints, the MAV may drift from its location as it follows a trajectory, due to small but accumulated errors. So, MAVBench includes a computational kernel that guides MAVs to follow trajectories while repeatedly checking and correcting the error in the MAV's position.

\subsection{Quality-of-Flight (QoF) Metrics}
\label{sec:QoF}

Metrics are key for quantitive evaluation and comparison of different systems. In traditional computing systems, we use Quality-of-Service (QoS), Quality-of-Experience (QoE) etc. to evaluate computer system performance for servers and mobile systems, respectively. Similarly, various figures of merits can be used to measure a drone's mission quality. These metrics otherwise called as mission metrics measure mission success and also throughout this paper are used to gauge and quantify compute impact on the drone's behavior. While some of these metrics are universally applicable across applications, others are specific to the application under inquiry. On the one hand, for example, a mission's overall time and energy consumption are almost universally of concern. On the other hand, the discrepancy between a collected and ground truth map or the distance between the target's image and the frame center are specialized metrics for 3D mapping and aerial photography respectively. MAVBench platform collects statistics of both sorts; however, this paper mainly focuses on time and energy due to their universality and applicability to our goal of cyber-physical co-design. 
%As shown in \Tbl{tab:benchmarks}, MAVBench consists of five different applications: scanning, aerial photography, package delivery, exploration, and search and rescue. In the following paragraphs, we describe each of these applications and present each of the applications in order of increasing complexity.
\begin{comment}
\begin{table*}[t]
\centering
\caption{Benchmark suite}
\label{tab:benchmarks}
\begin{tabular}{|l|l|l|}
\hline
\textbf{Benchmarks } & \textbf{Kernels} & \textbf{Evaluation Metrics} \\ \hline \hline
Scanning & lawnmower path planning & Fuel consumption, mission time \\ \hline
Sports photography & object detection, tracking & ``Target-centering'' \\ \hline
Package delivery & \begin{tabular}[c]{@{}l@{}}collision-free planning, obstacle avoidance,\\ localization \end{tabular} & \begin{tabular}[c]{@{}l@{}} Fuel consumption, mission time, \\ final location accuracy \end{tabular} \\ \hline
Exploration & \begin{tabular}[c]{@{}l@{}}collision-free planning (frontier exploration), \\ obstacle avoidance, localization\end{tabular} & \begin{tabular}[c]{@{}l@{}}mission time, fuel consumption, \\ map accuracy\end{tabular} \\ \hline
Search and rescue  & \begin{tabular}[c]{@{}l@{}}collision-free planning (frontier exploration), \\ obstacle avoidance, object detection, localization\end{tabular} & Time to find target \\ \hline
\end{tabular}
\end{table*}
\end{comment}


==> tex/MAV_CIG_and_NewDomain.tex <==
\section{A Cyber-Physical Perspective on MAVs}
\label{sec:MAV_cyber_physical_interaction}

Similar to the cross-compute layer optimization approach widely adopted by computer system designers, robots benefit from cross system (i.e. cross cyber and physical) optimizations and co-designs. To this end, we introduce the Cyber-Physical Interaction Graph (CIG) to better explore and analyze the tight coupling of compute and physical processes in cyber-physical systems. We first familiarizing the reader with the CIG, present the CIG for a MAV, examine the role of compute for MAVs through its CIG, and finally discuss the need for new tools to develop deep insights from the interactions described by CIGs.

\subsection {Cyber-Physical Interaction Graph (CIG)}
\newcommand{\cpg}{Cyber-Physical Interaction Graph}

Figure ~\ref{fig:CIG_general}, shows a generic CIG. There are four types of nodes in a CIG: the subsystems making up the robot complex (denoted using rectangles), the cyber and physical quantities that determine the behavior of the robot (denoted using ellipses), and the quality metrics used to measure the system (denoted using diamonds). The edges in the graph imply the existence and the direction of interactions between nodes. Vertices, filled black circles where two or more edges cross, represent the potentially complex equations that govern the interaction. To fully investigate the interactions between any two nodes, one needs to examine all of the paths along all of the edges in the graph originating from the first node and ending with the second node. We call each one of these paths an ``impact path.''

\begin{figure}[!htb]
\centering
\vspace{10pt}
\includegraphics[trim=0 0 0 0, clip, width=0.6\linewidth]
{figs/genericCIG.png}
%\vspace{-10pt}
\caption{Generic Cyber-Physical Interaction Graph.}
\label{fig:CIG_general}
\end{figure}

\subsection{CIG for MAVs}

\begin{figure}[!t]
\vspace{20pt}
\includegraphics[trim=0 0 0 0, clip, width=.7\linewidth]
{figs/cyber_physical_interaction_graph_example_paths}
\vspace{5pt}
\caption{A CIG for a MAV along with two example impact paths.}
\label{fig:CIG_MAV}
\end{figure}

Figure ~\ref{fig:CIG_MAV} is the CIG for a quadrotor MAV. An MAV has three important subsystems: the sensors, the actuators, and the compute. It also has three important cyber quantities: \textit{Sensory-to-Actuation latency} (Sense-Act Latency in the graph), \textit{Sensory-to-Actuation throughput} (Sense-Act Throughput in the graph), and \textit{Response Time}. Sensory-to-Actuation latency is the time the drone takes to sample sensory data, process the data, and finally issue flight commands. Sensory-to-Actuation throughput is the rate with which the drone can issue flight commands. Response time is the time the drone takes to respond to an event emerging in its surrounding environment (e.g. the emergence of an obstacle in the drone's field of view). An MAV has four important physical quantities: its power consumption, the total mass of the drone, its acceleration, and its velocity. The later three importantly summarize the MAV's dynamics. We focus on two quality metrics: mission time and mission energy. These metrics are chosen since for many applications (e.g., package delivery, search and rescue) a faster mission is a more successful mission. Finally, reduction in energy consumption will enable an MAV to successfully complete longer and more complicated missions. The many edges and vertices in the graph denote and describe the interactions between these quantities. These interaction range from simple addition to sum up the masses of the robot complex (marker 1) to more complex linear functions describing power consumption (marker 2) to complex non-linear relations (marker 3). 

\subsection{Examining the Role of Compute for MAVs}
\label{sec:role_of_comp_intro}
Figure \ref{fig:CIG_MAV}, show that there are \textbf{9} impacts paths originating from compute. In this section we briefly explain two of these paths to give the reader a high-level intuition for how compute affects quality metrics for MAVs. We defer a detailed discussion of these impact paths to Sections ~\ref{sec:comp_mission_time}, ~\ref{sec:comp_mission_energy}, and ~\ref{sec:impact_holistic}. Interestingly, through one path the impact is positive (lowering the energy consumption and hence saving battery) while through the other the impact is negative. In the positive impact path (shown in blue), increased compute capability allows an MAV to reduce a cyber quantity, sensory-to-actuation latency and thus response time. This allows the drone to increase a physical quantity, velocity, while still avoiding obstacles. By flying faster, the drone can reduce its mission time and in many cases also reduce total mission energy by being more efficient with its flight. In the negative impact path (shown in red), we observe that increased compute capability consumes more power and thus can directly increase total mission energy.

% At first in sections ~\ref{sec:comp_mission_time} and ~\ref{sec:comp_mission_energy},
% we investigate them in isolation to gain a better insight into the underlying concepts, and then in section ~\ref{sec:impact_holistic}, we put them all together for a holistic examination. 
% Overall, if studied in isolation, we see that an increase in compute can positively impact (reduce) mission time and energy
% by reducing cyber quantities such as reaction throughput and latency; however,
% an increase in compute can negatively impact the mission time and energy through increasing physical quantities such as quad's mass and power.

\subsection{Analyzing CIGs}
Investigation of the interactions modeled in CIGs requires new sets of tools due to the numerous differences between cyber-physical systems and their more traditional counterparts (e.g., desktops, servers, smartphones). In this paper, we develop tools to overcome two of these major differences. First, cyber-physical systems have continuous interactions with complex and unpredictable surrounding environments. Second, in these systems, the data flows in a (closed) loop starting from the environment, passing through the MAV, and then back to the environment as shown in \Fig{fig:Aerial_agent_data_flow}.

\begin{figure}[ht!]
\centering
\includegraphics[trim=0 0 0 -25, clip, width=0.9\linewidth]{figs/Aerial_agent_3}
\vspace{5pt}
\caption{Closed-loop data flow in a MAV. Information flows from sensors collecting environment data into the MAV's compute system, down into the actuators and back to the environment.}
\label{fig:Aerial_agent_data_flow}
\end{figure}

To enable system design research and development, we provide a simulator (Section~\ref{sec:simulation}) and a benchmark suite (Section ~\ref{sec:mavbench}) to model these types of interactions. Our simulator is able to capture an environment's complexity with high fidelity through the use of a game engine, and the closed-loop data flow is modeled using a hardware in the loop setup. In the next two sections, we discuss each of these tools in details. It is worth noting that although this paper mainly focuses on Micro Aerial Vehicles (MAVs), the generality of our simulation framework allows for the investigation of other autonomous machines (e.g., AirSim now supports cars as well). With this, we hope to systematically bootstrap a collaboration between the robotics and system design community---an opportunity for domain-specific architecture specialization. 

==> tex/MAV_cyber_physical_interactions.tex <==
\section{A Cyber-Physical Perspective on MAVs}
\label{sec:MAV_cyber_physical_interaction}

MAVs are an integration of cyber and physical processes. 
A tight interaction of the two enables compute to control the physical actions of an autonomous MAV. 
%For example, the performance of the onboard compute platform dictates the agility and maneuverability of a MAV. 
Robot designers need to understand how such cyber and physical processes impact one another and ultimately, the robot's end-to-end behavior.
%, and investigate how different subsystems within a robot complex impact the robot's end-to-end behavior through such interactions.
%subsystems within a robot complex the impact robots subsystems investigate their impact on the robot's end-to-end behavior.
Furthermore, similar to cross-compute layer optimization approach widely adopted by the compute system designers,
robot designers can improve the robot's optimality by adopting a robot's cross-system (i.e., cross cyber and physical) optimization methodology and co-design.

To this end, we introduce the \csig, a directed acyclic graph that captures how different subsystems of a robot impact the mission metrics through various cyber and physical quantities.
%which captures interactions that exist between the cyber and physical processes of a robot that impact mission time and energy consumption. 
We familiarize the reader with the graph (using a simple example) and move onto presenting what the graph looks like for a complicated MAV robot. Next, looking through the lens of this graph, we provide a brief example of how a subsystem such as compute can impact a mission metric, and finally discuss the need for new tools to investigate these impacts in details.

\subsection{Cyber-Physical Interaction Graph}

A \csig has four components to it. It has (1) a robot complex, (2) cyber-physical quantities, (3) impact functions, and (4) mission metrics. Subsystems in the robot complex have either cyber and/or physical quantities that impact one another that are captured in the graph, which can ultimately affect mission metrics such as mission time or energy consumption.

Figure ~\ref{fig:CIG_general}a shows a generic \csig. The graph consists of a set of edges and vertices. The subsystems making up the robot complex are denoted using ellipses. The mission
metrics specifying the metrics developers use to measure the mission's success are shown using diamonds. The cyber-physical quantities specifying various quantities that determine the behavior of the
robot are shown using rectangles. The impact functions, capturing the impact of one quantity on another and further on the mission metrics, are shown using contact points (filled black circles when two or more edges cross). The edges in the graph imply the existence and the direction of the impact. 

\begin{figure}[]
\centering
\includegraphics[trim=0 0 0 0, clip, width=1\linewidth]
{figs/cyber_physical_interaction_graph_general}
\caption{Cyber-physical interaction graph. This graph captures how the various subsystems of a robot impact mission metrics through cyber and physical quantities that interact with one another.}
\label{fig:CIG_general}
\end{figure}

To investigate the impact of one vertex on another, such as compute and mission time, 
we need to examine all the paths originating from the first vertex (compute) and ending with the second vertex (mission time). We call each one of these paths ``impact paths.''

We use a toy example of a simple robot arm (Figure ~\ref{fig:CIG_general}b) to familiarize the reader with the graph.  
% ~\footnote{Note that although we grant that such a simplistic robot can not exist, its simplicity is meant to aid the reader with understanding of the data structure rather than getting bugged down
% with the complexity of the robot}$^{,}$
% ~\footnote{Robot Description: This robot is used in a factory pipeline, where it simply picks up a box, rotates 45 degrees, drop it, rotates 45
% degree back to pick-up the next box. Using an open loop controller, the aforementioned set of actions are repeated for a limited number of iterations (and hence boxes)}.
Our robotic arm has two subsystems, namely a compute and an actuation subsystem. These subsystems impact mission time, i.e., the time it takes for the
robot to relocate all the boxes, through a cyber quantity such as control throughput and a physical quantity such as arm's mass.
The green-color/double-sided and blue-color/coarse-grained-dashed paths show two paths that compute impacts mission time.
Intuitively speaking, through the blue-color/coarse-grained-dashed path, compute impacts controller's throughput and hence the robot's rotation speed. This, in return, impacts mission time.
Through the green-color/double-sided path, compute impacts the mass of the robot and hence dictating the speed and ultimately, the mission time. Note that the impact function, shown with the marker F in Figure ~\ref{fig:CIG_general}b, is simply an addition
function since the robot's overall mass is the aggregation of the compute and actuation subsystem mass.


%Quality Metrics of interest for such a robot is mission time, i.e., the time it takes for the
%robot to relocate all the boxes. Cyber and physical quantities of this robot are the control throughput, i.e., the frequency with which the control subsystem sends out action commands, and the arm's
%mass respectively~\footnote{It is worth noting that in general, the choice of cyber and physical quantities are highly robot, domain, and application dependent.}. The filled circle marked with ``F'' shows one of the interaction functions. Robotic arm' mass is simply the addition of the actuator's and the control
%subsystem's mass. Hence, ``F'' is simply an addition function. The green and blue color Paths show two different paths that compute impacts mission time.
%Intuitively speaking, through the blue path, compute impacts the controller's throughput and hence the robot's rotation speed. This in return impact mission time.
%Through the green path, compute impacts the mass of the robot and hence dictating the speed and ultimately the mission time.

%The interaction function vertex (i.e, filled circles) marked with + quantify how these two paths interact. Examples of these functions are extensively discussed in section ~\ref{sec:comp_mission_time}.

\begin{comment}
These vertec
``Subsystem'' vertices (denoted by rectangles) specify the subsystem makeup of the robot such as compute, actuators and sensors.
``System quantity'' vertices (denoted by non-filled circles) specify robot's various quantities, i.e, 1.cyber quantities such as throughput and latency 2. physical quantities such as system's mass, and acceleration, and 3.mission metrics such as mission time and energy. 
``Interaction function'' vertices (denoted by filled circles) specify functions that capture the interactions between adjacent quantities. The edges in the graph, imply the existence and the direction of the interactions. 
To investigate the impact of one quantity on another, we need to examine the paths starting with the first quantity and ending with the second. We call each one of such paths ``impact paths''.

Figure~\ref{fig:CIG_arm} shows the interaction graph for 
such robot. This robot has two subsystems, namely a compute and an actuation subsystem. In our graph, we present one 
relevant cyber and physical quantities, namely control throughput and mass respectively. Finally, for our light discussion, we
focus on mission time (i.e, the time it takes for the robot to relocated all the boxes) as the metric of interest. 
To investigate the interactions between any two vertices, such as compute and mission time, 
we need to examine all the paths originating from the first vertex (compute) and ending with the second vertex (mission time). These paths are shown with green-color/double-sided and
blue-color/coarse-grained-dashed lines.
Compute impacts the controller throughput and hence the rotation speed. This in return impact mission time (blue-color/coarse-grained-dashed path).
Furthermore, compute impacts the mass of the robot and hence dictating the speed and ultimately the mission time (green-color/double-sided path).
The impact function vertex (i.e, filled circles) marked with + quantify how these two paths interact. Examples of these functions are extensively discussed in section ~\ref{sec:comp_mission_time}.
\end{comment}


\subsection{MAV Cyber-Physical Interaction Graph}
\blueDebug{par summary:SIG for our quad. Exemplify two paths with a short description. Explain direct/indirect interactions. outro to case studies}

\begin{figure}[!t]
%\vspace{20pt}
\includegraphics[trim=0 0 0 0, clip, width=.8\linewidth]
{figs/cyber_physical_interaction_graph_example_paths}
\caption{Cyber-physical interaction graph for our quadrotor MAV with some path examples.}
\label{fig:CIG_MAV}
\end{figure}

We apply the \csig to our quadrotor MAV. The quadrotor consists of three subsystems, namely the sensory, actuation, and compute subsystem. Figure ~\ref{fig:CIG_MAV} illustrates the MAV's \csig broken down into the four major subcomponents.

We focus on three cyber quantities, i.e, \textit{sensing-to-actuation latency} (Sensing-Actuation Latency in the graph), \textit{sensing-to-actuation throughput} (Sensing-Actuation Throughput in the
graph), and \textit{Response Time}. Sensing-to-actuation latency is the time the drone takes to sample sensory data and process them to issue flight commands ultimately. 
Sensing-to-actuation throughput is the rate with which the drone can generate the aforementioned (and new) flight commands. Response time is the time the drone takes 
to respond to an event emerging (e.g., the emergence of an obstacle in the drone's field of view) 
in its surrounding environment. %As we show in the later sections, we show the relationship between these three quantieies. 

For the physical quantities, we focus on motion dynamic/kinematic related quantities such as mass, i,e, the total mass of the drone, it's acceleration, and velocity. This is because they impact our mission metrics. For instance, an increase in mass can decrease acceleration, which translates to more power demands from the rotors, and that ultimately increases the overall mission energy consumption. 

For mission metrics, we focus on time and energy. These metrics are chosen due to their importance to the mission success. Reducing mission time is of utmost importance for most applications such as package delivery, search and rescue, scanning, and others. Also, reduction in energy consumption is valuable as a drone that is out of battery is unable to finish its mission. 

The impact functions range from simple addition (marker 1 in Figure~\ref{fig:CIG_MAV}) to more complex linear functions (marker 2) to non-linear relations (marker 3). 

Note that although the MAV \csig presented in this paper does not contain all the possible cyber and physical quantities associated with a MAV, we have included the ones that have the most significant impact on our mission metrics.
%Each one of these interactions of extensively detailed in later sections. 

\subsection{Examining the Role of Compute Using the Cyber-physical Interaction Graph}
\label{sec:role_of_comp_intro}

%Figure \ref{fig:CSIG_combined} on the left shows all paths 
Compute plays a crucial role both in the overall mission time and total energy consumption of a MAV in different ways, which we refer to as impact paths. Figure \ref{fig:CIG_MAV}, highlights two paths that can influence mission energy. We briefly explain these to give the reader an intuition for how compute affects MAV's mission metrics, deferring the details until later for discussion.

Through one path,  the impact is positive (i.e., lowering the energy consumption and hence saving battery) while through the other, the impact is negative (i.e., increasing the energy
consumption). In the positive impact path, i.e., the blue-color/coarse-grained-dashed path, compute can reduce the mission energy. This is because a platform with more compute capability reduces a
cyber quantity, such as sensing-to-actuation latency and response time. This allows the drone to respond to its environment faster and in return, increase a physical quantity like its velocity. By flying faster, the drone finishes its mission faster and so reduces a mission metric such as its total mission energy. 

Looking through the lens of another path, the impact is negative (i.e., energy consumption increases). In the negative impact path, i.e., the red-color/fine-grained-dashed path, a more compute capable platform has a negative impact on the mission energy because it consumes more power. 
%Since the MAV has a finite amount of battery capacity, every joule of energy consumption matters. 

We count a total of nine impacts paths originating with compute and ending with mission time and energy. This paper quantitatively examines all such paths where the cyber and physical quantities
impact one another dictating the drone's behavior. At first in sections ~\ref{sec:comp_mission_time} and ~\ref{sec:comp_mission_energy},
we investigate them in isolation to gain a better insight into the underlying concepts, and then in section ~\ref{sec:impact_holistic}, we put them all together for a holistic examination. 
Overall, we see that an increase in compute can positively impact (reduce) mission time and energy
by improving cyber quantities such as sensing-to-actuation throughput and latency; however,
an increase in compute can negatively impact the mission time and energy through increasing physical quantities such as quad's mass and power.

%Combined all together, we show that such opposite impacts constrains the amount of compute one can deploy onboard. 
%We briefly explain each path leaving the detailed discussion to later sections. 
%In this paper, we examine how the compute subsystem can impact MAV's behavior; however, first, let's us provide a brief overview of CIG in action. Later on in the paper, we aggressively couple CIG with theory, system modeling, and benchmarking to dive into details. 



%The red, blue, and purple edges respectively denote direct,
%indirect, and hybrid interactions compute can have with other variables. 
%For example, the red line between compute and latency shows that compute directly impacts
%latency, whereas the blue line between latency and velocity shows the indirect way (i.e., through latency)  in which compute impacts velocity. We counted a total of  8 number of different paths
%with which compute impacts mission time and energy.  We illustrate two of such paths with dashed lines, each with a 
%different quantity and direction of impact. The coarse grain ("\_\;\;\_") dashes show how compute
%impacts mission's energy by traversing through latency, velocity, and mission time vertices. Through this path, an increase in compute capability, reduces latency, and as a result incre%asing velocity,
%reducing mission time and finally leading to a reduction in mission energy. On the other hand, the fine grain path (denoted with "..") shows this impact through power directly, where an increase in
%compute%
%capability, increases the power consumption and hence increases mission energy (These paths along with others are detailed and quantified in the next 3 sections). 


==> tex/abstract.tex <==
\begin{abstract}
Autonomous and mobile cyber-physical machines are becoming an inevitable part of our future. In particular, unmanned aerial vehicles have seen a resurgence in activity. With multiple use cases, such as surveillance, search and rescue, package delivery, and more, these unmanned aerial systems are on the cusp of demonstrating their full potential. Despite such promises, these systems face many challenges, one of the most prominent of which is their low endurance caused by their limited onboard energy. 
    % For example, many of the off-the-shelf commercial Micro Aerial Vehicles (MAVs) have an endurance of fewer than 20 minutes. 
    Since the success of a mission depends on whether the drone can finish it within such duration and before it runs out of battery,
    improving both the time and energy associated with the mission are of high importance.  
    Such improvements have traditionally arrived at through the use of better algorithms. But our premise is that more powerful and efficient onboard compute can also address the problem. In this paper, we investigate how the compute subsystem, in a cyber-physical mobile machine, such as a Micro Aerial Vehicle (MAV), can impact mission time and energy.
    Specifically, we pose the question as ``\textit{what is the role of computing for cyber-physical mobile robots?}'' 
%mitigate the aforementioned constraints.} 
% To unlock their potential, optimial designs should not only deploy better algorithms but also pay attention to more efficient onboard computers. Toward this goal, we dedicate this paper to
%the investigation of a simple question, i.e,  \textit{what is the role of computing for an autonomous and mobile cyber-physical system such as micro aerial vehicle? In other words, how can compute impact and
%mitigate the afformentioned constraints.} As we show 
We show that compute and motion are tightly intertwined, and as such \texit{a close examination of cyber and physical processes and their impact on one another is necessary.} We show different ``impact paths'' through which compute impacts mission metrics and examine them using a combination
of analytical models, simulation, micro and end-to-end benchmarking. 
To enable similar studies, we open sourced \textit{MAVBench}, our tool-set, which consists of \textbf{(1)} a closed-loop real-time feedback simulator and \textbf{(2)} an end-to-end benchmark suite comprised of
state-of-the-art kernels. By combining MAVBench, analytical modeling, and an understanding of various compute impacts, we show up to 2X and 1.8X improvements for mission time and mission energy for two optimization case studies. 
Our investigations, as well as our optimizations, show that \textit{cyber-physical co-design, a methodology with which both the cyber and physical processes/quantities of the robot are developed with consideration of one another, similar to hardware-software co-design, is necessary for arriving at the design of the optimal robot.}

\end{abstract}


==> tex/analysis.tex <==
\section{Analysis}

In this section we characterize our workloads and determine the components of a drone's subsystem that their performance is most affected by. Thus, we get an accurate picture of exactly what is being tested by each workload.

We see that workload X stresses the parallel processing capability of a drone's companion computer, while workload Y's performance is unaffected by such-and-such component, etc.


==> tex/background.tex <==
\section{Micro Aerial Vehicle Background}
\label{sec:background}


\begin{table}[b!]
\centering
\caption{UAVs by NATO Joint Air Competence Power~\cite{nato-uav-classification}.}
\label{nato-classification-drones}
\resizebox{.6\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
Category                                                              & Weight (kg) & Altitude (ft) & Mission Radius (km) \\ \hline\hline
Micro                                                                 & \textless2                                             & \textless200                                                                    & 5                                                                           \\ \hline
Mini                                                                  & (2-20)                                                 & (200- 3000)                                                                     & 25                                                                          \\ \hline
Small                                                                 & (20-150)                                               & (3000-5000)                                                                    & 50                                                                          \\ \hline
Tactical                                                              & (150-600)                                              & (5000-10000)                                                                    & 2000                                                                        \\ \hline
Combat & \textgreater600                                        & \textgreater10000                                                               & Unlimited                                                                   \\ \hline
\end{tabular}
}
\end{table}


We provide a brief background on Micro Aerial Vehicles (MAVs), the most ubiquitous and growing segment of Unmanned Aerial Vehicles (UAVs). We then describe various subsystems that make up a MAV, and finally present the overall system level constraints facing MAVs.

\subsection{Micro Aerial Vehicles (MAVs)}
\label{sec:mav}

UAVs initially emerged as military weapons for missions in which having a human pilot would be a disadvantage~\cite{rs}. But since then there has been a recent proliferation of various other aerial vehicles for civilian applications including crop surveying, industrial fault detection, mapping, surveillance and aerial photography. There is no single established standard to categorize the wide range of UAVs. But Table~\ref{nato-classification-drones} shows one proposed classification guide provided by NATO. This classification is largely based on the weight of the UAV, and the mission altitude and range. 

In this paper, we focus on MAVs. A UAV is classified as a micro UAV if its weight is less than 2~\si{\kilo\gram}, and it operates within a radius of 5~\si{\kilo\meter}. MAVs' small size increases their accessibility and affordability by shortening their ``development and deployment time,'' and reducing the cost of ``prototyping and manufacturing''~\cite{Zhang2017207}. Also, their small size coupled with their ability to move flexibly empowers them with the agility and maneuverability necessary for these emerging applications.

\begin{comment}
\begin{table}[]
\centering
\caption{Classification based on Size}
\label{my-label}
\begin{tabular}{|l|l|}
\hline
\textbf{Size} & \textbf{Value}  \\ \hline
Very Small    & 30 to 50 cm     \\ \hline
Small         & 50 to 2 m       \\ \hline
Medium        & 5 to 10 m       \\ \hline
Large         & \textgreater10m \\ \hline
\end{tabular}
\end{table}
\begin{table}[]
\centering
\caption{Classification of UAV based on Range and Endurance}
\label{my-label}
\begin{tabular}{|l|l|l|}
\hline
\textbf{Class}   & \textbf{Range} & \textbf{Endurance}    \\ \hline
Very Close Range & 5 Km           & 20-45 min             \\ \hline
Close Range      & 50 Km          & 1 to 6 Hours          \\ \hline
Short Range      & 150 Km         & 8 to 12 Hours         \\ \hline
Mid Range UAV    & 650 Km         & 12 to 36 Hours        \\ \hline
Endurance UAV    & 300 Km         & \textgreater 36 Hours \\ \hline
\end{tabular}
\end{table}
\end{comment}

MAVs come in different shapes and sizes. A key distinction is their wing type, ranging from fixed wing to rotary wing. Fixed wing MAVs, as their names suggest, have fixed winged airframes. Due to the aerodynamics of their wings, they are capable of gliding in the air, which improves their ``endurance'' (how long they last in the air). However, this also results in these MAVs typically requiring (small) runways for taking-off and landing. In contrast, rotor wing MAVs not only can take off and land vertically, but they can also move with more agility than their fixed-wing counterparts. 
They do not require constant forward airflow movement over their wings from external sources since they generate their own thrust using rotors. These capabilities enhance their benefits in constrained environments, especially indoors, where there are many tight spaces and obstacles. For many applications these benefits outweigh the cost of reduced endurance and as such rotor wing MAVs have become the dominant form of MAV. We focus on rotor based MAVs, specifically quadrotors. Nonetheless, the conclusions we draw from our studies apply other UAV categories as well.

% Vertical Take-Off and Landing (VTOL) vehicles represent a hybrid between both designs. These vehicles use rotor wings to take off after which the vehicle transitions to forward flight with a fixed wing formation.


% \begin{comment}
% \subsection{rotor-based Micro Aerial Vehicles: UAV of choice}
% %Among the aforementioned categories, rotor-based Micro aerial vehicle have an outburst of attention in recent years. This section elaborates how their rotor-based flight mechanism and smaller size can explain such a trend.

% \textit{rotor based flight mechanism:} Using their flight mechanism, one can classify UAVs to fixed wing, flapping wing, or rotary wing. Though fixed-wings "simpler structure and more efficient aerodynamics provide the advantage of longer flight"(http://www.uavinsider.com/rotary-wing-vs-fixed-wing-uavs/),  the aircrafts with rotors are capable of "
% %vertically taking off and landing, fixed-point hovering, flying
% at low level altitude, and great stability and maneuverability."~\cite{Development-of-a-Micro-Aerial-Vehicle}. 

% \textit{small size:} MAVS are aircrafts of size less than 15 cm length, width, or height and weigh less than 100 g. Such a small size have increased accessibility and affordibily of such systems by shortening the "development and deployment time", and reducing the cost for "prototyping and manufacturing", ~\cite{Rugged Embedded Systems 1st Edition book}. 
% In addition, the combination of the small size and the hovering capability of the rotors provide these systems with the agility and  maneuverability necessary for various applications such as sports photography, indoor mapping, surveillance and etc.
% \end{comment}

% %Micro-Aerial Vehicles(MAV) comes in different shapes and sizes. On one end of the spectrum, MAV have fixed wing. On the other end, we have rotor based. Both these type of MAV can have electric motors or internal combustion engine as the propulsion system. The choice of propulsion system has a direct impact on the range and endurance of the MAV. There are also hybrid MAVs which uses both electric and internal combustion engine for propulsion. 

% \begin{comment}
% \begin{table}
% \centering
% \resizebox{\columnwidth}{!}{%
% \caption{Drone categories.}
% \label{tab:drones}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% Category          & weight & range(km) & endurance(h) & altitude(h)     \\ \hline\hline
% Micro       \textless2      &  \textless1      &           & 5-30 min     & \textless330 \\ \hline
% Mini              &  \textless1 &           & 1-2          &              \\ \hline
% Small             &    \textless13.5    &           &              &              \\ \hline
% Light/ultra Light &     \textless242   &           &              &              \\ \hline
% Normal            &   \textless4332     &           &              &              \\ \hline
% Large             &     \textless4332   &           &              &              \\ \hline
% \end{tabular}
% }
% \end{table}
% \end{comment}

% \begin{comment}
% \subsection{Drone Platforms}
% \label{ssec:drone-arch}
% \begin{table}[]
% \centering
% \caption{Drone tiers: this table will contain high level ideas about drones from the pure functionality level, i.e. no system design perspective. e.g frame size, flight time, max speed, avg payload, max payload}

% \label{my-label}
% \begin{tabular}{|l|l|}
% \hline
% Drone Type & Frame size {[}mm{]} \\ \hline
% Nano       & 80-100              \\ \hline
% Micro      & 90-180 mm           \\ \hline
% Mini       & 150-300             \\ \hline
% \end{tabular}
% \end{table}
% Table~\ref{tab:drone-platforms}
% \begin{table*}[t!]
% \centering
% \caption{Drone platform characteristics. pick a drone from different tiers and introduce the specs (from system perspective)}
% \label{tab:drone-platforms}
% \begin{tabular}{ |p{3cm}||p{3cm}|p{3cm}|p{3cm}|  }
%  \hline
%  Name     or Area Name& A nano drone name & a micro drone name & a mini drone name \\
%  \hline
% Power   & AF    &AFG&   004\\
% Flight-time &   AX  & ALA   &248\\
% Battery &AL & ALB&  008\\
% FMU    &DZ & DZA&  012\\
% Payload &   AS  & ASM&016\\
% ... & AD  & AND   &020\\
% Companion computer & AO  & AGO&024\\
%  \hline
% \end{tabular}
% \end{table*}
% \end{comment}

% \begin{comment}
% \subsection{System Architecture old}
% \label{ssec:drone-arch}

% \red{in this section we explain the general architecture of a drone, since all the drones generally follow the same subsystem design. this is basically about the system architecture that is used by all the drones. explain the components within and how they interact etc.}

% A typical autonomous MAV is equipped with an onboard computer, a flight controller, a collection of sensors, and a set of mechanical components including propellers and motors.

% \paragraph{On-board Computer} A drone requires an onboard computer for autonomous flight. This onboard computer is responsible for high-level flight control and for computations that are not directly related to flight such as object detection or machine learning.

% \paragraph{Flight controller} The flight controller is a microcontroller that handles a variety of low-level flight-related tasks. For example, it stabilizes the drone during flight, logs flight data, and controls the drone's orientation and speed to move it in the fashion specified by the onboard computer.

% \paragraph{Sensors} Drones have the capability of gathering a rich set of sensory data, and the sensors they are equipped with will vary depending on the application that they are intended for. At minimum, however, a typical autonomous drone will be equipped with a sensor, such as an inertial measurement unit, that detects orientation, a sensor, such as a barometer or ultrasonic sensor, that detects altitude, and a sensor, such as a GPS receiver or optical flow camera, that detects position. There are many other possible sensors that may be attached to drones such as LIDAR sensors for 3-D mapping, cameras for photography, or even multispectral sensors for the purpose of monitoring crop health.

% \paragraph{Other} In addition to sensors and processors, drones are composed of mechanical components such as motors, propellers, and frames.

% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{figs/drone-arch}
% \caption{Architectural overview of our drone platform.}
% \label{fig:dronearch}
% \end{figure}
% \end{comment}


\subsection {MAV Robot Complex}
\label{sec:MAV_subsystems}
MAV's have three main subsystems that make up their robot complex: sensing, actuation, and compute, as shown in \Fig{fig:drone_components}. Similar to other cyber-physical systems, the design and development of MAVs requires an understanding of their composed and intertwined subsystems which we detail in this section. In these cyber-physical systems, the data flows in a (closed) loop, starting from the environment, going through the MAV and back to the environment, as shown in  \Fig{fig:Aerial_agent_data_flow}.

\begin{figure}[t!]
\centering
\includegraphics[trim=0 0 0 -25, clip, width=.6\linewidth]{figs/drone_components.pdf}
\caption{MAV robot complex. The three main subsystems, i.e., compute, sensors and actuators, of an off-the-shelf Intel Aero MAV are shown. All other MAVs have a similar subsystem structure.}
\label{fig:drone_components}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[trim=0 0 0 -25, clip, width=0.7\linewidth]{figs/Aerial_agent_3}
\caption{Closed-loop data flow in a MAV. Information flows from sensors collecting environment data into the MAV's compute system, down into the actuators and back to the environment.}
\label{fig:Aerial_agent_data_flow}
\end{figure}
\paragraph{Sensors:} Sensors are responsible for capturing the state associated with the agent and its surrounding environment. 
To enable intelligent flights, MAVs must be equipped with a rich set of sensors capable of gathering various forms of data such as depth, position, and orientation. For example, \mbox{RGB-D} cameras can be utilized for determining obstacle distances and positions. The number and the type of sensors are highly dependent on the workload requirements and the compute capability of onboard processors which are used to interpret the raw data coming from the sensors.

\paragraph{Flight Controller (Compute):} The flight controller (FC) is an autopilot system responsible for the MAV's stabilization and conversion of high-level to low-level actuation commands. 
While they themselves come with basic sensors, such as gyroscopes and accelerometers, they are also used as a hub for incoming data from other sensors such as GPS and sonar. For command conversions, FCs take high-level flight commands such as``take-off" and lower them to a series of instructions understandable by actuators (e.g., current commands to electric motors powering the rotors). FCs use light-weight processors such as the ARM Cortex-M3 32-bit RISC core for the aforementioned tasks.    
 
\paragraph{Companion Computer (Compute):} The companion computer is a powerful compute unit, compared to the FC, that is responsible for the processing of the high level, computationally intensive tasks (e.g., computer vision). Not all MAVs come equipped with companion computers. Rather, these are typically an add-on option for more processing. NVIDIA's TX2 is a representative example with significantly more compute capability than a standard FC.

\paragraph{Actuators:} Actuators allow agents to react to their surroundings. They range from rather simple electric motors powering rotors to robotic arms capable of grasping and lifting objects. Similar to sensors, their type and number are a function of the workload and processing power on board.



%\red{battery is mising}
%\paragraph{Battery:} MAVs are mobile systems, i.e. they need to be able to finish their mission with the limited energy resources that that they have on board. Choosing batteries is an important step in the design of MAVs since the battery subsystem 1.should be able to provide the current and voltage necessary to spin the rotors with sufficient torque 2. should have a high capacity to elongate MAV's endurance, but 3. it must light enough such that it's added mass would not burden the rotors and take away from the MAV's agility and endurance. Various types of batteries are available for MAVs, but Lithium polymer ones (LiPo) are the most common due to higher capacity, faster rate of discharge, and lighter weights. 


\subsection{MAV Constraints}
\label{sec:constraints}

%\red{I still don't understand why we need this section -- I get that constraints are important but you seem to just give an example of a performance constraint and of an energy constraint it doesn't feel fleshed out enough -- or too much. I just find it a bit awkward -- but I also note that it is a direct pull form MavBench so probably not worth worrying about.}

\begin{figure}[t!]
\centering
    \begin{subfigure}{.47\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=.7\columnwidth]{figs/Battery_Capacity_vs_Endurance_plot}
   \caption{Endurance against battery capacity.}
    \label{fig:battery_capacity_vs_endurance}
    \end{subfigure}
    %\hspace*{5pt}
    \begin{subfigure}{.47\columnwidth}
    \centering    
    \includegraphics[trim=0 0 0 0, clip, width=.7\columnwidth]{figs/Size_vs_Battery_Capacity}
    \caption{Drone size against total battery capacity.}
    \label{fig:battery_capacity_vs_size}
    \end{subfigure}
\caption{MAVs based on battery capacity and size. Endurance is important for MAVs to be useful in the real-world. However, their small size limits the amount of onboard battery capacity.}
\label{fig:tradeoff}
\end{figure}

A MAV's mechanical (propellers, payload, etc.) and electrical subsystems (motors and processors) constrain its operation and endurance, and as such present unique challenges for system architects and engineers. For example, when delivering a package, the payload size (i.e., the size of the package) affects the mechanical subsystem, requiring more thrust from the rotors and this, in turn, affects the electrical subsystem by demanding more energy from the battery source. Comprehending these constraints is crucial to understand how to optimize the system. The biggest of the constraints as they relate to computer system design are performance, energy, and weight.

%At the high level, application (package delivery) requirements (lifting certain payload size for a certain range) turns into mechanical (rotors/motors thrust) and energy source (LIPO battery capacities) constraints. In turn, such constraints manifest themselves as performance and power constraints for architects to deal with. In this section we iterate over such constraints:

% \begin{comment}
% \begin{figure}
%     \centering
%     \begin{minipage}{0.5\textwidth}
%         \centering
%         figure puts here
%         \cpation{figure caption goes here}\label{fig: figure-label}
%     \end{minipage}
%     \begin{minipage}
%         \centering
%         \captionsetup{type=table} %% tell latex to change to table
%         table puts here
%         \caption{table caption goes  here}\label{tab: table-label}
%     \end{minipage}
% \end{figure}
% \end{comment}

\paragraph{Performance Constraints:} MAVs are required to meet various real-time constraints. For example, a drone flying at high speed looking for an object requires fast object detection kernels. Such a task is challenging in nature for large-sized drones that are capable of carrying high-end computing systems, and virtually impossible on smaller sized MAVs. Hence, the stringent real-time requirements dictate the compute engines that can be put on these MAVs.

\paragraph{Energy Constraints:} The amount of battery capacity on board plays an important role in the type of applications MAVs can perform. Battery capacity has a direct correlation with the endurance of these vehicles. To understand this relationship, we show the most popular MAVs available in the market and compare their battery capacity to their endurance. As \Fig{fig:battery_capacity_vs_endurance} shows, higher battery capacity translates to higher endurance. We see a step function trend, i.e., for classes of MAVs that has similar battery capacity, they have similar endurance. On top of this observation, we also see that for the same battery capacity, a fixed wing has longer endurance compared to rotor wing MAVs. For instance, in \Fig{fig:battery_capacity_vs_endurance}, we see that the Disco FPV (''Fixed wing'') has higher endurance compared to the Bebop 2 Power (''Rotor wing'') even though they have a similar amount of battery capacity.
We also note that the size of MAV also has a correlation with battery capacity as shown in \Fig{fig:battery_capacity_vs_size}. 



\begin{comment}
\begin{figure}[t!]
\centering
\tabskip=0pt
    \begin{subfigure}{\columnwidth}
    \centering
    \vspace{0.1in}
    \includegraphics[trim=0 0 0 0, clip, width=.9\columnwidth]{figs/Battery_Capacity_vs_Endurance_plot}
    \caption{Endurance versus battery capacity.}
    \label{fig:battery_capacity_vs_endurance}
    \end{subfigure}
    \begin{subfigure}{\columnwidth}
    \centering
    \vspace{0.1in}
    \includegraphics[trim=0 0 0 0, clip, width=.9\columnwidth]{figs/Size_vs_Battery_Capacity}
    \caption{Size versus battery capacity.}
    \label{fig:battery_capacity_vs_size}
    \end{subfigure}
\caption{MAVs based on battery capacity and size. Endurance is important for MAVs to be useful in the real-world. However, their small size limits the amount of onboard battery capacity.}
\label{fig:tradeoff}
\end{figure}
\end{comment}
%\red{I don't think we need the following two constraints. They are not relavant to architects, or if they are, it's hard to argue. also get rid of the figure that comes with it}
%\paragraph{Size:}The Size of MAV plays an important role in selection of mechanical and electrical subsystem. \Fig{fig:battery_capacity_vs_size} shows the distribution of size of MAVs and the battery capacity. MAVs deployed for aerial photography/surveying have higher battery capacity for their sizes. The racing MAVs are much smaller in size compared to camera MAVs but have more battery capacity for their size. However, racing MAVs typically have lower flight times in the order five to ten minutes because all the energy is spent generating higher thrusts.

%\red{this paragraph is confusing. where are the aerial photography/scanning drones in the figure. Are they camera drones? also it doesn't seem like we are discussing size constraints, but rather the implications of picking a size. also I think we should get rid of this or combine it with weight and imply the }

\paragraph{Weight Constraints:} MAV weight, inclusive of its payload weight, can also have a significant impact on its endurance. Higher payload puts stress on the mechanical subsystems requiring more thrust to be generated by the rotors for hovering and maneuvering. This significantly reduces the endurance of MAVs. For instance, it has been shown that adding a payload of approximately 1.3~\si{\kilo\gram} reduces flight endurance by 4X~\cite{hasan2016sensorcloud}.


%Since most of the above-mentioned constraints either leads to performance bottlenecks in compute or energy consumption, opening up interesting avenues for research in computer architecture.\red{<- wording doesnt make sense. I also see the connection to compute architects.} To address these problems, computer architects need tools that extend beyond traditional simulators. 

%The aforementioned constraints opens up interesting avenues for research in computer architecture. To address these problems, computer architects need tools that extend beyond traditional simulators.



%Weight constraint is essential to the functioning of the aircrafts such as taking-off and stability. However, it has system implications. For example, it can throttle the system's thermal power budget since the added weight associated with introducing a fan might not be a possibility
%As was dicussed , the need to be mobile with high exploratory capacities constraints aerial agents to their amount of energy on board. (possibly cite one platform with flight time). As a result, longer flight time due to lower system performance can cause system to run out of energy and hence fail its mission. Performance improvements such as decreasing the decision making time (while drone hovers\footnote{one can think of this analogous to reduction of processor idle times}), or increasing decisions optimality (e.g. shorter paths to take while navigating) allows such systems to stay within energy budget. 

%\begin{figure}[t!]
%\centering
%\includegraphics[width=0.5\columnwidth]{figs/Size_vs_Battery_Capacity}
%\vspace{-.4ex}
%\caption{ }
%\vspace{-3ex}
%\label{fig:1}
%\end{figure}

%\begin{figure}[t!]
%\centering
%\includegraphics[width=0.5\columnwidth]{figs/Battery_Capacity_vs_Endurance_plot}
%\vspace{-.4ex}
%\caption{ }
%\vspace{-3ex}
%\label{fig:1}
%\end{figure}


\begin{comment}
\red{here we explain the power and performance characteristics of drones from the data that is presented in the table. the goal is to provide intuition about what is going on in terms of power consumption and what is the peak performance of the native platform...}

There are multiple factors that affect drone flight performance. These include energy constraints, maximum payload size, total weight, and computing capability.

\paragraph{Energy Constraints} A drone's energy constraints include its battery lifetime and the power consumption of its components. Battery lifetime is of the utmost relevance to a drone's performance because it limits a drone's maximum lifetime, which in turn restricts the maximum range to which a drone can fly. If battery lifetime is low, then package delivery drones, for example, may not be able to service rural areas that are far from flight stations. Companies may also have to build expensive recharging stations where drones can stop mid-route in order to extend their range.

\paragraph{Payload Size} Drones may be required to carry external payloads during their flights. Package delivery drones are the most obvious example, but search and rescue drones can also carry payloads in order to leave survivors they discover with food, water, and other survival materials before emergency responders can arrive. Although large payloads may be desirable, they can also be disadvantageous to a drone's flight performance. Large payloads will reduce a drone's stability, which may make it difficult for it to fly in anything other can calm weather, and they will increase a drone's weight and thus the total power consumed by motors in flight.

\paragraph{Total Weight} A drone's total weight is heavily correlated with its power consumption, which, as mentioned above, can have a dramatic effect on a drone's performance. The heaviest component of a drone is usually the battery which must be carefully selected so as to find the optimum tradeoff between battery capacity and battery weight. The heavier a drone's battery, the more energy it can provide for flight, but the more power it takes be lifted off the ground.

\paragraph{Compute} For drones to be fully autonomous, they must be able to process data about their surroundings at high frame rates. For computationally intensive operations like object detection, powerful CPUs and GPUs may be required.

\paragraph{Communication} Autonomous drones may communicate with ground stations or other drones while in flight. As long as they are able to maintain communication, they can offload computations or mission tasks to off-board components which can improve their performance. In certain environments, however, communication may be unreliable and so autonomous drones must still be able to complete their tasks when they lose communication with off-board components, even if their performance drops as a result.

\paragraph{Speed} Drones that fly fast must be able to process incoming information much more quickly than those that fly more slowly in order, for example, to avoid collisions. Therefore, fast-flying drones require more powerful onboard computers to achieve safe autonomous flight. They will also require more advanced IMUs and flight controllers in order to maintain stability at high speeds.
\end{comment}



==> tex/case_studies.tex <==
%\section{Compute-driven, Flight-Efficiency Optimization: A Case Study}
 
\label{sec:energy-case-study}
\section{Case Studies}
\label{sec:case-study}


We show how our closed-loop simulation, along with our open-source benchmark suite, can enable (1) performance, (2) energy and (3) reliability studies, both at the architecture and the holistic system-level. MAVBench simulation setup allows for inspection of intra-system, as well as system and environment interactions. Studying the intra-system interactions opens new avenues for hardware and software co-design, which we demonstrate in the form of onboard/edge-only compute versus offloading the compute to the unconstrained cloud. Studying the system and environment interactions can unlock new opportunities for tradeoffs in computational complexity for energy efficiency, which we demonstrate using software-guided, hardware-assisted OctoMap resolution optimizations.

\subsection{A Performance Case Study}


As opposed to the study in Section~\ref{sec:char} where we emulated a fully-on-edge drone (i.e., a drone which all of its computation is done on the drone itself), we examine a cloud/edge drone where the computation is distributed across the edge and the cloud. We compare a fully-on-edge drone equipped with a TX2 versus a fully-in-cloud drone with a powerful cloud support. The ``cloud'' computational horsepower is composed of an Intel i7 4740 @ 4GHz with 32 GB of RAM and a GeForce GTX 1080. For network connectivity we utilize a 1Gbp/s LAN, which mimics a future 5G network~\cite{agyapong2014design, gupta2015survey}.

\begin{figure}[b!]
\centering
    \begin{subfigure}{.608\columnwidth}
    \centering
    \includegraphics[trim=5 0 20 0, clip, width=\columnwidth]{figs/tx2-desktop_performance}
    \caption{Performance.}
    \label{Perforamnce}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.365\columnwidth}
    \centering
    \includegraphics[trim=5 10 0 0, clip, width=\columnwidth]{figs/tx2-desktop_energy}
    \caption{Energy.}
    \label{fig:cloud-edge-energy}
    \end{subfigure}
\caption{Comparing a full-on-edge drone versus a full-on-cloud drone. Our system allows part or portion of the MAVBench workloads to be offloaded to the cloud (or another local co-processing agent).}
\label{fig:cloud_edge}
\end{figure}

We target the planning stage of the PPC pipeline and focus on the 3D Mapping as the application of choice to offload. As we show in \Fig{fig:cloud_edge}, a drone that can enjoy the cloud's extra compute power sees a 3X speed up in planning time. This improves the drone's average velocity due to hover time reduction, and hence reduces the drone's overall mission time by as much as 50\%, effectively doubling its endurance.

\begin{figure*}[!t]
\vspace{-12pt}
    \centering
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[height=1.4in]{figs/garage_sim}%
         \vspace{-20pt}
        \caption{Environment's map.}%
        \label{fig:garage_sim}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[height=1.4in]{figs/garage_rviz__15}%
         \vspace{-20pt}
        \caption{Resolution of 0.15 \emph{(m)}.}%
        \label{fig:rviz__15}
    \end{subfigure}
    \hfill
     \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[height=1.4in]{figs/garage_rviz__5}%
      \vspace{-20pt}
     \caption{Resolution of 0.5 \emph{(m)}.}%
        \label{fig:game:rviz__5}
    \end{subfigure}
       \hfill
   \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[height=1.4in]{figs/garage_rviz_1}%
        \vspace{-20pt}
        \caption{Resolution of 0.80 \emph{(m)}.}%
        \label{fig:game:rviz_1}
    \end{subfigure}
    \hfill\\[15pt]
   \vspace{-25pt}
   \caption{For the environment in \emph{(a)}, OctoMap's resolution impact on the drone's perception of its environment is shown in \emph{(b)}, \emph{(c)}, \emph{(d)}.}
    \label{fig:octomap_perception}
\end{figure*}

\begin{figure}[t]
\vspace{0pt}
\centering
\includegraphics[trim=0 0 30 0, clip, width=\columnwidth]
%\includegraphics[trim=0 0 0 0, clip, width=1.0
%\linewidth]%
{figs/octomap_resolution_case_study}
%{figs/octomap_resolution_with_boxes}
%\vspace{-50pt}
\vspace{-23pt}
\caption{Reduction in OctoMap resolution (accuracy) can be traded off with processing time. Increasing the $x$-axis means larger voxels to represent the space more coarsely (less accurately). A 6.5X reduction in resolution results in a 4.5X improvement in processing time.}
%\vspace{15pt}
\label{fig:octrest}
\end{figure}


\subsection{An Energy Case Study} 

Focusing on energy efficiency, we conduct a kernel/environment sensitivity analysis using the OctoMap node~\cite{octomap}, which is a major bottleneck in three of our end to end applications, namely package delivery, 3D mapping and search and rescue. OctoMap is used for the modeling of various environments without prior assumptions. The map of the environment is maintained in an efficient tree-like data structure while keeping track of the free, occupied and unknown areas. Both planning and collision avoidance kernels use OctoMap to make safe flight possible, via costly compute cycles, by only allowing navigation through free space. Due to its implementation efficiency, OctoMap is widely adopted in the robotics community. Its broad adoption and impact in two out of three stages (Perception and Planning) makes this kernel highly general and important for optimization.

The size of the voxels in OctoMap, i.e. the map's resolution, introduces accuracy versus flight-time/energy tradeoff. By lowering the resolution, i.e. increasing \emph{voxel} sizes, obstacle boundaries get inflated, hence the drone's perception of the environment and the objects within it becomes inaccurate. We illustrate the impact of OctoMap resolution on the drone's perception using \Fig{fig:octomap_perception}. \Fig{fig:garage_sim} {shows the environment and  Figures~\ref{fig:rviz__15}, \ref{fig:game:rviz__5}, \ref{fig:game:rviz_1} show the drone's perception of the environment as a function of OctoMap resolution. When the resolution is lowered, the voxels size increases to the point that the drone fails to recognize the openings as possible passageways to plan through (Figure~\ref{fig:game:rviz_1}). This results in mission time inefficiency and failures depending on the environment.

To examine the accuracy versus performance trade off, we measured OctoMap kernel's processing time (running in isolation) while varying its resolution knob. \Fig{fig:octrest} shows that as planning resolution increases (i.e., voxels are larger so space is represented more coarsely and hence less accurately), performance improves dramatically because less compute is needed. Going from one extreme to another, when planning resolution goes from less than 0.2~m to 1.0~m ($x$-axis), OctoMap's processing time (or update rate) goes from more than 0.4~seconds to less than 0.1~seconds ($y$-axis). In other words, a 6.5X reduction in accuracy results in a 4.5X improvement in processing time.


\begin{figure}[t]
%\vspace{-5pt}
\centering
\includegraphics[trim=0 0 0 0, clip, width=\columnwidth]
%\includegraphics[trim=0 0 -5 -25, clip, width=0.9\linewidth]
%\includegraphics[height=5cm,keepaspectratio]
%\includegraphics[width=\columnwidth]%
%\includegraphics[trim={0 0 0 5cm}, clip, width=\columnwidth]%
{figs/energy-case-study}
\vspace{-23pt}
%\vspace{-15pt}
\caption{Switching between OctoMap resolutions dynamically leads to successfully finishing the mission compared to 0.80~m. It also leads to battery life improvement compared to 0.15~m. The $y$-axis in the top graph is the battery left on the drone upon mission completion.}
%\vspace{15pt}
\label{fig:dual-res}
\end{figure}



\begin{comment}
\begin{table}[t]
\vspace*{20pt}
\centering
\vspace{-14pt}
\caption{Switching between OctoMap resolutions dynamically leads to mission success compared to 0.8~m, and compared to 0.15~m we consume less energy and thus retain more battery.}
\label{tbl:octopt}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l|l|l|l|}
\cline{2-4}
\textbf{Resolution {(m)}}       & \textbf{Mission Status} & \textbf{Battery  (\%)} \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Package Delivery}}} & \textit{0.8}              & \cellcolor{red!25}Fail                    &   0           \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{0.15}             & Pass                    &    81.00          \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{Chameleon (0.8, 0.15)} & Pass                    &   \cellcolor{green!25}86.00           \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Mapping}}}          & \textit{0.8}              & \cellcolor{red!25}Fail                    & 0           \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{0.15}             & Pass                    & 39.03        \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{Chameleon (0.8, 0.15)} & Pass                    & \cellcolor{green!25}53.83        \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Search and Rescue}}}              & \textit{0.8}              & \cellcolor{red!25}Fail                    & 0         \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{0.15}             & Pass                    & 24.21        \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{Chameleon (0.8, 0.15)} & Pass                    & \cellcolor{green!25}57.87        \\ \hline
\end{tabular}
}
\end{table}
\end{comment}


Certain aspects like obstacle density in the environment determine the ``ideal'' OctoMap resolution. In low-density environments, where the drone has many obstacle-free paths to take, a low resolution can suffice. In dense environments, low resolutions can deprive the drone of viable obstacle-free paths because the drone perceives the obstacles to be larger than they are in the real world, and so plans to avoid them. Since the drone's environment constantly changes, a dynamic approach where a runtime sets the resolution is ideally desirable.

We study two environments during the mission, namely outdoors (low obstacle density) and indoors (high obstacle density). \Fig{fig:dual-res} shows the result of two static (predetermined) resolutions, 0.15~m and 0.80~m, and our dynamic approach that multiplexes between the two appropriately.\footnote{Resolutions are based on the environment like the door width size. A 0.15~m resolution is chosen to ensure that the drone (diagonal width of 0.65~m) considers an average door (width of 0.82~m) as an opening for planning.} The dynamic approach allows improvement of battery consumption by up to 1.8X. 
%life for up to 43\%. To compute this improvement, we calculate the difference between the dynamic and static battery consumption and divide it by the static value. For example, for SAR, $\frac{(76\%- 43\%)}{76\%}$ leads to a 43\% improvement. 
Intuitively, as compute reduces, OctoMap bottleneck eases, and therefore the drone completes its mission faster. The figure also highlights another interesting relationship that statically choosing the 0.80~m resolution to optimize for compute (only) causes the drone to fail its mission since it is unable to plan paths through narrow openings in the indoor environments. Instead, by switching between the two resolutions according to the environment's obstacle density, the dynamic approach is able to balance OctoMap computation with mission feasibility and energy, holistically. Therefore, in all cases, the dynamic approach uses less energy and retains more battery life at mission end time.


% Please add the following required packages to your document preamble:
% \usepackage{multirow}


\subsection{A Reliability Case Study}

Reliability is an especially important topic in the context of autonomous vehicles~\cite{reli-1, reli-2, reli-3, reli-4}. Traditionally, it is common to study the susceptibility of execution to errors that manifest in programs and the architecture. In autonomous vehicles, errors or ``noise'' in the data can arise from sensor inputs. 

We investigate the impact of sensor noise on the performance of our package delivery application, specifically its perception stage. The data is summarized in Table~\ref{tbl:noise-data}. We inject Gaussian noise with a range of standard deviations (0 to 1.5~m) into the depth readings of the drone's RGBD camera. The sensory noise distorts the drone's perception of the obstacles in its environment, and we found such noise \emph{inflates} obstacles, making them appear larger than they are in reality. This causes the drone to re-plan its trajectories more often, as it assumes that its planned path will collide into objects that are actually further away than they seem. The more the drone re-plans its paths, the longer it takes to reach its destination, which increases it mission time by up to 90\%. It is also important to note that when noise values reach greater than a certain value, it causes the drone to fail in its mission altogether, e.g. noise with the standard deviation of 1.5~m results the drone to fail reaching its delivery destination in 10\% of its total runs. 

In addition to injecting noise in the sensor subsystem, we can also inject errors directly into the compute subsystem to ``simulate'' soft errors and transient bit flips in logic. Such a capability can be used to conduct vulnerability analysis~\cite{mukherjee2005soft}.


==> tex/characterization.tex <==
\begin{comment}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{figs/slam-speed-energy.png}
\caption{relationship between drone's speed compute power}
\label{sec:powerbreakdown}
\end{figure}
\end{comment}
\begin{comment}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{figs/desktop_vs_tx2_mapping.png}
\caption{relationship between motion planning performance and compute power}
\label{microbenchmark_1}
\end{figure}
\end{comment}
\section{The Role of Compute in MAVs}
\label{sec:char}

In this section, we discuss how compute affects MAV systems. At /the high level, compute plays a crucial role both in the overall mission time and total energy consumption of such systems. First, we discuss each effect by providing relevant  theoretical background and supplement the discussion with a microbenchmark. Then, we analyze MAVBench as a set of representative applications in which such effects can manifest.   %Figure~\ref{fig:benchmarks_data_flow} and our benchmark suits and  discuss the high level insights into aerial agents bottlenecks and their corresponding implications. 


%thout the loss of generality we use our benchmark suit to conduct studies. The results and the flow presented in section blah to explain the corresponding  the by a discussion of  total system, i.e. locomotion and compute energy consumption, and its distribution. Then, we provide case studies showing that more compute can result in an improvement in the overall system's energy consumption. Finally we delve into our application benchmark suit to discuss how such a role can effect them.

%\subsection{Compute and Accuracy Relationship}
%explain slam and present the microbenchmark

\subsection{Compute and Flight Time Relationship}

Compute can play an important role in reducing the drone's mission time by increasing the mission's average velocity. To attain a high average velocity, the drone needs to maintain a high velocity throughout its mission. In order to do this, the drone needs to 1.have a high maximum velocity to traverse the trajectory with 2.maintain this high velocity and reduce deviation from it. 



This requires have a high maximum velocity  we identify that the reduction in hover time and the increase in maximum allowed velocity are the two major ways with which more compute can contribute to a higher average velocity. Here, we shed light on these different ways.
\being{comment}
\paragraph{Hover Time Reduction:} Hover time and the average velocity have an inverse relationship, namely, the more drone spends time on hovering, the lower its average velocity. Similar to an idling CPU, a hovering drone is unfavorable since it is not working toward its mission, but yet wasting its limited energy. A hovering drone typically is waiting for its mission planning stage to make a decision (e.g. deciding on a path to follow). \emph{More compute power can help reduce hovering (e.g by reducing the decision making time),} hence decreasing the negative effect hovering has on the average velocity. 
\end{comment}
\begin{figure}[t!]
\centering
    \begin{subfigure}{.49\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/fig_13}
    \caption{Theoretical max velocity.}
    \label{fig:process-time-velocity}
    \end{subfigure}
    \begin{subfigure}{.49\columnwidth}
    \centering
   \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/slam_fps_velocity_energy}
    \caption{Measured max velocity.}
    \label{fig:slam-velocity-energy}
    \end{subfigure}
\vspace{-5pt}
%\setlength{\belowcaptionskip}{-4ex}
\caption{\emph{(a)} Theoretical relationship between processing time and maximum velocity. \emph{(b}) Relationship between SLAM throughput (FPS) and maximum velocity and energy of UAVs.}
%\label{SOLO_power_breakdown}
\end{figure}

\paragraph{Max Velocity Increase, Collision Avoidance Effect:} The maximum velocity of the drone is not only mechanically bounded, but also compute bounded. For a given flight velocity, a collision-free flight is only possible if the drone can process its surrounding fast enough to react to it. Therefore, \emph{a higher velocity requires a faster processing capability}. The collision avoidance task can be rather compute intensive exercising various stages of the pipeline starting from the pixel processing in the perception stage and ending with the command issue in control. In order to guarantee collision avoidance, a  drone's maximum velocity is determined based on the aforementioned pixel to response time.
Equation~\ref{eq:runtime-compute-bound} specifies the components involved in setting this velocity where $\delta_{t}$, d, $a_{max}$ and v denote process time, required stopping distance, maximum acceleration limit of the drone and maximum velocity~\cite{high-speed-nav}. 
In order to understand this, consider a drone that periodically takes a snap shot of its environment (using its sensors), generates a trajectory and then follows it. In doing so, at any point if the drone realizes that there is an obstacle on its path, it attempts to plan around it. However, if the motion planner fails to converge, the drone needs to decelerate immediately to avoid running into the obstacle. Figure blah shows this scenario in action.  
\begin{equation}
\label{eq:runtime-compute-bound}
v_{max} = a_{max}(~\sqrt[]{4*\delta{t}^2 + 2\frac{d}{a_{max}}} - 2*\delta{t})
\end{equation}
\setlength{\belowcaptionskip}{-1ex}

\begin{equation}
\label{eq:latency}
\delta{t}_{sensor_to_actuation} = \delta{t}_{perception} + \delta{t}_{planning} + \delta{t}_{control}
\end{equation}

\begin{equation}
\label{eq:throughput}
\tau_{sensor_to_actuation} = \frac{1}/\Delta = Min(\frac{1}{\delta{t}_{perception}},  \frac{1}{\delta{t}_{planning}}, \frac{1}{\delta{t}_{control}})
\end{equation}

\begin{equation}
\label{eq:obstacle-distance}
obstacle\;distance= d - v_{max}*\delta_{t} - v_{max}*\delta_{t}
\end{equation}

\begin{equation}
\label{eq:stop-distance}
stopping\;distance= v^2/2*a_{max} 
\end{equation}

\begin{figure}[t]
\includegraphics[width=\columnwidth]{figs/vmax_seq.pdf}
\caption{stopping distance in a sequential design}
\label{sec:vel_proc_relationship_figure}
\end{figure}

\begin{figure}[t]
\includegraphics[width=\columnwidth]{figs/vmax_pipe.pdf}
\caption{stopping distance in a sequential design}
\label{sec:vel_proc_relationship_figure}
\end{figure}

\textit{Sequential Design:}
At point $Snap_{0}$, the drones takes a snap shot of the world, and spends $\delta_{t}$ to digest (perception), generate a trajectory (planning )  and following (control) within its visible distance (d). \ref{eq:latency} shows this time where $\delta$ denotes latency. In a naive approach, while the drone is going through one iteration of the PPC pipeline, no new snap shot is taken. This results in the drone to be blind ($t_{blind}$) for the entirety of the PPC pipeline, i.e. $t_{blind}$ = $\delta_{t}$ and causing a momentarily blind space ($sp_{blind})$ until the next snap shot. In the worse case scenario, an obstacle can be hiding within the blind space (point O)  d - $v_{max}$*$\delta_{t}$ away from the drone. Point $snap_{1}$ marks the second snap shot when the drone starts digesting the new information and realizing that it needs to plan around the obstacle. This demands another pass through the PPC pipeline hence spending another $\delta_{t}$. At this point, if the drone fails to converge on a plan, it needs to slam on its breaks and hope to stop within distance shown in \ref{eq:obstacle-distance}.
Equation \ref{eq:stop-distance} shows the distance that it takes for a moving body to come to a complete stop. Setting \ref{eq:obstacle-distance} and \ref{eq:stop-distance} equal to one another and solving for v results in \ref{eq:runtime-compute-bound}, i.e. the absolute maximum velocity with which the drone is allowed to fly in while guaranteeing a collision free mission. 
 
\textit{Taking advantage of pipeline:}
By overlapping perception, planning and control, we can reduce the blind time ($t_{blind}$) and space ($sp_{blind}$) as shown in figure blah. In doing so, blind time quals to the inverse of system throughput. Note that since each stage takes different amount of time, worse case throughput needs to be considered as shown in \ref{eq:throughput} where \tou denotes throughput, and \Delt is the its inverse. This approach reduces the velocity to \ref{eq:runtime-pipe}. 

\begin{equation}
\label{eq:runtime-pipe}
v_{max} = a_{max}(~\sqrt[]{(\delta{t} + \Delta{t})^2 + 2\frac{d}{a_{max}}} - (\delta{t} + \Delta{t})
\end{equation}
\setlength{\belowcaptionskip}{-1ex}

As \Fig{fig:process-time-velocity} shows, our simulated drone, in theory, is bounded by the max velocity anywhere between 8.83 to 1.57 m/s given a pixel to response time of the range 0 to 4~seconds. 



\begin{comment}
\begin{figure}[t]
\includegraphics[width=\columnwidth]{figs/fig_13}
\caption{Theoretical relationship between process time and max velocity}
\label{sec:vel_proc_relationship_figure}
\end{figure}
\end{comment}



\paragraph{Max Velocity Increase, Localization Failure Effect:} The faster the speed of the drone, the higher the likelihood of its localization failure because the environment changes rapidly around a fast drone. Kernels such as SLAM which help localize the drone by tracking a set of points/features through successive camera frames struggle to keep up with the rate of these changes. It is important to note that localization failures can have catastrophic effects such as permanent loss or spending of extra time (for example by backtracking) for re-localization. 

Minimizing or avoiding localization related failure scenarios is highly favorable, if not necessary. To examine the relationship between the compute, maximum velocity and localization failure, we devised a micro-benchmark in which the drone was tasked to follow a predetermined circular path of the radius 25~meters. For the localization kernel, we used ORB-SLAM2 and to emulate different compute powers, we inserted a sleep in the kernel. We swept different velocities and sleep times and bounded the failure rate to 20\%. As \Fig{fig:slam-velocity-energy} shows, higher FPS values, i.e. more compute, allows for a higher maximum velocity for a bounded failure rate. 

%\begin{figure}[h]
%\includegraphics[]{figs/blank.pdf}
%\caption{Measurement set up to collect power data for 3DR Solo.}
%\label{sec:powerbreakdown}
%\end{figure}
\begin{figure}[!t]
\centering
    \begin{subfigure}{.49\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/power_break_down_tx2}
    \caption{Measured power breakdown.}
    \label{fig:SOLO-power-breakdown}
    \end{subfigure}
    \begin{subfigure}{.49\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/drone-power-time-series}
    \caption{Measured mission power.}
    \label{fig:drone-power-time-series}
    \end{subfigure}
\caption{\emph{(a)} Measured power consumption of a flying 3DR Solo. \emph{(b)} Total measured power consumption while the drone is "Flying" at two different steady-state velocities. The power consumption is severely dominated by the quad rotors by 20X.}
\label{SOLO_power_breakdown}
\end{figure}

\paragraph{Maintaining Max Velocity}
As was discussed before, in order to reduce the mission time, it's not enough to have a high bound on v (v_max), but we need to reach v_max and maintain it along the flight. In other words, once v_max is reached, the drone should attempts at reducing deviation from it. This means that trajectories of low curvature are desired. 

\subsection{Compute and Energy Relationship}
The compute subsystem can also have a significant role in reducing total MAV energy consumption. To understand this, first we present the power distribution associated with \solo~\cite{solo3DR}, a popular off-the-shelf MAV. To measure power, we attach a wattmeter known as Eagle~Tree Systems eLogger~V4~\cite{eLoggerV4} to the \solo's battery during flight. The wattmeter allows us to collect data over time at 50~Hz while the drone flies. We command the drone to fly for fifty seconds and pull the data off of the wattmeter after the drone lands.

% The wattmeter gave us the total power consumed by the drone, without a deeper breakdown. To estimate the portion of the instantaneous power that would typically be consumed by a MAV's processor, we subtracted the idle power consumption of the \solo's default onboard computer and added to it the power consumed by the TX2 during typical workloads.

As \Fig{SOLO_power_breakdown} shows, the majority of the power consumption is dedicated to rotors (locomotion) and the compute only occupies a small portion of the entire pie and its role seemingly trivial. Although small in quantity, compute can have a grand effect on the system's power. This is because by reducing the mission time (as explained in the previous section), more compute power can, in fact, reduce the bigger portion of the pie, namely rotors energy consumption (due to a shorter flight). Note that although more compute can lead to more energy consumption of the compute subsystem, the reduction in rotor's energy can easily outweigh such an increase.  
% \setlength{\belowcaptionskip}{-2ex}


We profiled the mission time and the energy associated with the aforementioned microbenchmark. As the bottom plot in \Fig{fig:slam-velocity-energy} shows, higher compute capability results in increased SLAM FPS and hence a reduction in mission time by allowing for faster velocity. The reduced mission results in reduced total system energy, as the top plot in \Fig{fig:slam-velocity-energy} shows. By increasing processing speed by 5X, we were able to reduce the drone's energy consumption by close to 4X.


\subsection{MAVBench Workloads Compute vs. Flight Time vs. Energy}
\label{sec:operating-spoints}
We use our benchmark suite as a representative set of applications to examine the effect of compute on MAV systems. To analyze this effect, we conducted sensitivity analysis to core and frequency scaling of the TX2 board. TX2 has two sets of cores, namely a \textit{HMP Dual Denver cores} and a \textit{Quad ARM A57}. We turned off the Denver cores so that the indeterminism caused by process to core mapping variations across runs would not affect our results.
Average velocity, mission, and energy values of various operating points are profiled and presented as heat maps (\Fig{fig:benchmarks:OPA:scanning}---\Fig{fig:benchmarks:OPA:ap}) for a DJI Matrice 100 drone. \emph{In general, compute can improve mission time and lower energy consumption by as much as 5X.}

\paragraph{Scanning:}
We observe trivial differences for velocity, endurance and energy across all three operating points (\Fig{fig:benchmarks:OPA:scanning:velocity}, \Fig{fig:benchmarks:OPA:scanning:time}, and \Fig{fig:benchmarks:OPA:scanning:energy}). This is despite seeing a 3X boost in the motion planning kernel, i.e. lawn mower planning, which is its bottleneck (\Fig{fig:kernel-breakdown}). The trivial effect of compute on this application is because planning is done once at the beginning of the mission and its overhead is amortized over the rest of the mission time. For example the overhead of planning for a 5 minute flight is less than .001\%.  
%\vspace{2pt}

%We present our understanding and takeaways regarding the computational bottlenecks and the effect of compute on them.


%Each application and its associated nodes are time profiled (table~\ref{kernel_makeup}).  We use this table along with the data flow presented in figure    \label{fig:benchmarks} to dissect and understand various compute bottlenecks. 

%At the high level, each application contains a node called mission planner responsible for high level decision making and arbitrating flight command issuance. When needed, this nodes place a service call to the motion planning kernel, setting out drones next set of moves. Some of our applications have the collision avoidance capability. This node exercises all stages of the pipeline starting from the perception stage, i.e. point cloud generation, OctoMap, collision check, to planning, mission planner/motion planner and ending with control, i.e. path tracking/command issue. 

 
%and their kernel makeup is provided. This will help us to understand the bottle-necks and opportunities for improvements.

%It would be wise to note that this application is intentionally design minimally without an involved perception and planning because ~\red{ask vijay. He knows very well how to justify this}.

\paragraph{Package Delivery}:  As compute scales with the number of cores and/or frequency values, we observe a reduction of up to 84\% and 82\% for the mission time and energy consumption, respectively (\Fig{fig:benchmarks:OPA:pd:time}, and \Fig{fig:benchmarks:OPA:pd:energy}). The sequential bottlenecks i.e. motion planning and OctoMap generation kernel are sped up by frequency scaling to enable the observed improvements. There does not seem to be a clear trend with core scaling, concretely between 3 and 4 cores. We conducted investigation and determine that such anomalies are caused by the non-real-time aspects of ROS, AirSim and the TCP/IP protocol used for the communication between the companion computer and the host. We achieve up to 2.9X improvement in OctoMap generation and that leads to maximum velocity improvement. It is important to note that although we also gain up to 9.2X improvements for the motion planning kernel, the low number of re-plannings and its short computation time relative to the entire mission time render its impact trivial. Overall the aforementioned improvements translate to up to 4.8X improvement in the average velocity. Therefore, mission time and the MAV's total energy consumption are reduced.

%OctoMap generation is a major computationally intensive kernel in this application. This kernels performance OctoMap is of utmost importance since it is on the collision avoidance path. As shown in the data flow, this path starts with depth images and flows through point cloud generation, OctoMap generation, collision check and finally ends in the control.  OctoMap is responsible for 99\% of the pixel to response time determined by this path. Figure blah shows how OctoMap kernel scales with different number of cores and frequencies. 

%Motion planner is another computationally intensive kernel for this application. Although at first glance, its optimization can improve the mission time, the low number of re-plannings and its short computation time relative to the entire mission time render its impact trivial. For example, if we re-plan 20 times during the coarse of 5 minutes of the mission time, planning time would only consume .01\% of the entire flight.  
 
\begin{comment}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{figs/velocity_process_time_relationship}
\caption{Theoretical relationship between process time and max velocity}
\label{sec:vel_proc_relationship}
\end{figure}
\end{comment}

%lowering the process time, results in a higher velocity and in turn, lowering the mission time and energy. 
%Explain collision avoidance path and policty and then discuss how octomap and planning comprise most of the it and the rest is ros runtime overhead. 
%Our pixel to response time is equal to 1.2 seconds most of which is dedicated to octomap and planning as is showing in the table.   

%As opposed to the surveying benchmark, package delivery's trajectory is determined at the mission time.  perception of the obstacles surrounding the drone at any moment and also on the way to the destination is required. To do so, a map of once visible and visited environment is created and maintained within an octomap structure \ref{blah}. Arriving at such a map requires converting image depth information to point clouds (point cloud generation node) and integrating them to the map (octomap server). It is important to note the dynamic obstacles are intentional not captured within the octomap. Motion planner, attempts to find the shortest path to the destination with the knowledge of such map and only remap on demand. 
  
%As the drone follow its trajectory, new trajectory can be demanded due to environmental triggers. These environmental triggers can be static obstacles unaccounted for at the time of planning (since they were not in the sensor's visibility range). Dynamic obstacles not present at the time of planning can also trigger replannings. 

%These triggers are identified using the panic and the future collision node. The future collision node identifies whether an obstacle (mainly static ones) is on the trajectory planned and alarm the mission planner node to request a re-plan. Since future collision operates on octomap, dynamic obstacles can not be spotted to be reacted to. This is an intentional decision since dynamic obstacles can move out of the path.
%Panic node, alarms the drone of any obstacles that enters a virtual halo surrounding the drone by processing the point cloud. By equipping the drone with a forward and backward camera, we can avoid most obstacles\footnote{since each camera only has a FOV of 120 degree, there are blind spots for our drone. To fix this, more sensors are required. We address this issue in the limitation section}  This node is our solution to dynamic obstacles. In addition to dynamic obstacles, this node can save the drone from crashing in any obstacle if the control node (follow trajectory) allows for a drift from it's supposed trajectory. 

%Due to small number of replannings, the hover time associated with the planning stage has a minor affect on the mission time. In addition, small time associated with real time threads such as panic and future collision does not demand more attention. Hence, compute's role on this application is minor.

{
\begin{figure}[t!]
    	\centering
    	\begin{subfigure}[t!]{.3\columnwidth}
    	\centering
    		\includegraphics[width=\columnwidth]{figs/scanning_velocity_operating_point}
    		\caption{Velocity (m/s)}
            \label{fig:benchmarks:OPA:scanning:velocity}
    	\end{subfigure}
        \begin{subfigure}[t!]{.3\columnwidth}
    	\centering 
    \includegraphics[width=\columnwidth]{figs/scanning_flight_time_operating_point}
    \caption{Mission Time (s)}
    \label{fig:benchmarks:OPA:scanning:time}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/scanning_energy_operating_point}
    \caption{Energy (kJ)}
    \label{fig:benchmarks:OPA:scanning:energy}
    \end{subfigure}
    \caption{Scanning.}
    \label{fig:benchmarks:OPA:scanning}
    \end{figure}%
   \begin{figure}[t!]
    \centering
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/pd_velocity_operating_point}
    \caption{Velocity (m/s)}
     \label{fig:benchmarks:OPA:pd:velocity}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/pd_flight_time_operating_point}
    \caption{Mission Time (s)}
    \label{fig:benchmarks:OPA:pd:time}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/pd_energy_operating_point}
    \caption{Energy (kJ)}
     \label{fig:benchmarks:OPA:pd:energy}
    \end{subfigure}
    \caption{Package Delivery.}
    \label{fig:benchmarks:OPA:pd}
    \end{figure}%
    \begin{figure}[t!]
    \centering
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/mapping_velocity_operating_point}
    \caption{Velocity (m/s)}
     \label{fig:benchmarks:OPA:mapping:velocity}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/mapping_flight_time_operating_point}
    \caption{Mission Time (s)}
    \label{fig:benchmarks:OPA:mapping:time}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/mapping_energy_operating_point}
    \caption{Energy (kJ)}
     \label{fig:benchmarks:OPA:mapping:energy}
    \end{subfigure}
    \caption{Mapping.}
    \label{fig:benchmarks:OPA:mapping}
    \end{figure}%
    \begin{figure}[t!]
    \centering
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/SAR_velocity_operating_point}
    \caption{Velocity (m/s)}
     \label{fig:benchmarks:OPA:sar:velocity}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/SAR_flight_time_operating_point}
    \caption{Mission Time (s)}
    \label{fig:benchmarks:OPA:sar:time}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/SAR_energy_operating_point}
    \caption{Energy (kJ)}
     \label{fig:benchmarks:OPA:sar:energy}
    \end{subfigure}
    \caption{Search and Rescue.}
    \label{fig:benchmarks:OPA:sar}
    \end{figure}
    \begin{figure}[t!]
    \centering
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/aerial_photography_error_operating_point}
    \caption{Error Rate(m/s)}
     \label{fig:benchmarks:OPA:ap:velocity}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/aerial_photography_flight_time_operating_point}
    \caption{Mission Time(s)}
    \label{fig:benchmarks:OPA:ap:time}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/aerial_photography_energy_operating_point}
    \caption{Energy (kJ)}
     \label{fig:benchmarks:OPA:ap:energy}
    \end{subfigure}
    \caption{Aerial Photography.}
    \label{fig:benchmarks:OPA:ap}
\end{figure}
}


\paragraph{Mapping:} We observe a reduction of up to 86\% and 83\% for the mission time and energy consumption, respectively, as compute scales with the number of cores and/or frequency values (\Fig{fig:benchmarks:OPA:mapping:velocity}, \Fig{fig:benchmarks:OPA:mapping:time}, and \Fig{fig:benchmarks:OPA:mapping:energy}). The concurrency present in this application (all nodes denoted by circles with a filled arrow connection or none at all in \Fig{fig:benchmarks:data-flow:mapping} run in parallel) justifies the performance boost from core scaling. The sequential bottlenecks, i.e. motion planning and OctoMap generation explains the frequency scaling improvements. We achieve up to 6.3X improvement in motion planning (\Fig{fig:kernel-breakdown}) and that leads to hover time reduction. We achieve a 6X improvement in OctoMap generation and that leads to maximum velocity improvement. The improvements translate to a 5.3X improvement in average velocity. Since mission time is reduced, total energy consumption reduces.


\paragraph{Search and Rescue:} We see a reduction of up to 67\% and 57\% for the mission time and the energy, respectively, as compute scales (\Fig{fig:benchmarks:OPA:sar:velocity}, \Fig{fig:benchmarks:OPA:sar:time}, and \Fig{fig:benchmarks:OPA:sar:energy}). Similar to mapping, more compute allows for the reduction of hover time and an increase in maximum velocity which contribute to the overall reduction in mission time and energy. In addition, a faster object detection kernel prevents the drone from missing sampled frames during any motion. We achieve up to 1.8X, 6.8X, and 6.6X speedup for the object detection, motion planning and OctoMap generation kernels, respectively. In aggregate, these improvements translate to 2.2X improvement in the MAV's average velocity.

\begin{comment}
\begin{figure}[!t]
\centering
\includegraphics[trim=0 0 0 -25, clip, width=0.9\linewidth]{figs/tx2-desktop}
\vspace{-12pt}
\caption{Comparing a full-on-edge drone versus a full-on-cloud drone. Our system allows part or portion of the MAVBench workloads to be offloaded to the cloud (or another local co-processing agent).}
\label{fig:cloud_edge}
\end{figure}
\end{comment}

\paragraph{Aerial Photography:} We observe an improvement of up to 53\% and 267\% for \emph{error} and mission time, respectively (\Fig{fig:benchmarks:OPA:ap:velocity}, \Fig{fig:benchmarks:OPA:ap:time}, and  \Fig{fig:benchmarks:OPA:ap:energy}). In aerial photography, as compared to other applications, higher mission time is more desirable than a lower mission time. The drone only flies while it can track the person, hence a longer mission time means that the target has been tracked for a longer duration. In addition to maximizing the mission time, error minimization is also desirable for this application. We define error as the distance between the person's bounding box (provided by the detection kernel) center to the image frame center.  Clock and frequency improvements translate to 2.49X and 10X speedup for the detection and tracking kernels and that allows for longer tracking with a lower error. No significant trend is observed in the energy data because energy depends on both the mission time and the velocity, and as opposed to the other applications, there is no need for the drone to minimize its velocity. Instead, it needs to successfully track the person.


\begin{figure*}[!t]
\centering
\includegraphics[width=\columnwidth]{figs/kernel-breakdown_2}
\vspace{-18pt}
\caption{Kernel breakdown for MAVBench. The abbreviations are as follows: \emph{OD-}Object detection, \emph{MP-}Motion Planning, \emph{OMG-}OctoMap Generation for kernels and \emph{SC-}Scanning, \emph{PD-}Package Delivery,  \emph{MAP-}3D Mapping, \emph{SAR-}Search and Rescue, and \emph{AP-}Aerial Photography for applications. The $x$-axis lists the kernel-application names and $y$-Axis represents the runtime in seconds. Each bar graph represents one of the configurations used in the hardware. The cores are varied from 2 to 4 and the frequency goes from from 0.8 GHz , 1.5 GHz or 2.2 GHz.}
\label{fig:kernel-breakdown}
\end{figure*}

%\begin{minipage}[!]{0.99\columnwidth}
   
%\end{minipage}


%In the perception stage of this application, a person is detected, and the bounding box associated with the person is tracked. The tracking stage consists of two nodes itself. The first node (buffer then track) buffers the images while detection is running and then track the buffered once the person is detected. The second node (track continuously) tracks the previous bounding box while the new one is calculated. Buffer then track node is necessary, since otherwise, image difference between the image detection sampled and tracking is large enough that increases the false positive tracking. PID node calculates the difference between the targets place and where it should be in the frame and sends small trajectories to the drone. Similar to other applications, these trajectories are followed in the follow trajectory node.

%Compute's effect on this application is on its accuracy and the duration in which drone can follow the target. In other words, faster compute can affect how closely and for how long the target is tracked. 
%\subsection{Understanding the Compute to Endurance Relationship}
%in this section, we demonstrate the relationship between compute on the drone and the drone's mission time (i.e., endurance). We start by showing that looking naively indicates that compute consumes an insignificant amount of power, and that much of the power is spent on keeping the drone afloat using its rotors. Therefore, this leads to a shortsighted conclusion that compute does not play a dominant role in autonomous flight for dron

%\subsection{Micro architectural characterization}
%To understand the reason behind the aforementioned bottlenecks, we provide micro-architectural characterization of them. This will help the designers to design for the future MAV systems while alleviating such bottlenecks. Our analysis show that the bottle necks mainly exists in the perception and the planning stage. Hence, we turn our focus solely to these two stages.  
%
%characterize OctoMap, slam and nbvPlanner. 

\begin{comment}
%\subsubsection{Algorithmic Choices}
%Algorithms at some point will be general enough to cover all the environments, hence we shouldn't 
%be highlighting our algorithmic sensitivity to environment (which in this argument is considered in a flaw)
 
\subsection{explanation of each apps inter kernel interactions}
\textbf{Scanning:} This application involves only a single ROS node. All the code runs on a CPU, with no parallelization. The main computational kernel is the simple path-planning since no collision-checking is involved. This is because the \textit{Scanning} benchmark is meant for outdoors environments, high aboveground where obstacles are not to be found. Because the benchmark is meant for outdoors environments, localization is accomplished through the use of GPS sensors, which incur negligible computational overhead.

\textbf{Aerial Photography}
This application involves three ROS nodes running concurrently. One node is responsible for running object detection algorithms to locate the human target. However, object detection is normally a very computationally-intensive task that can take up to several seconds to complete. Therefore, another node runs much faster tracking algorithms such as KCF which estimate the position of the target in the interval between completions of the object detection algorithm. Another node controls the motion of the MAV based on the position of the target. All nodes run on the CPU except for the object detection node which runs on a GPU.

\textbf{Package delivery:}
This application involves 4 ROS nodes, which all run on CPU cores. One node plans collision-free trajectories using the path-planning algorithms described in the previous section. Another node waits for paths to be planned and then controls the motion of the MAV to follow them. However, as the MAV follows these trajectories, it may uncover new obstacles in its environment that had been out of range of its sensors when the path was initially planned. Therefore, an additional node must constantly run to check whether any newly uncovered obstacle causes a collision upon the planned trajectory, so that the path can be re-planned if necessary. Finally one final node must provide localization capabilities, either through GPS or SLAM, to enable the MAV to follow its planned trajectory accurately.

\textbf{Mapping}
This application involves 3 ROS nodes which all run on CPU cores. One node samples its environment and finds points on the boundary of previously explored space where the MAV can be expected to maximize the amount of unknown space that it uncovers. Once these points are found, the node then plans a path towards them along an RRT tree. A second node controls the motion of the MAV, following the trajectories generated by the first node. Finally, a third node must provide localization, such as through SLAM. This localization must be accurate, because the MAV updates its internal map based upon the position it believes it is in. If the MAV relies upon an inaccurate SLAM algorithm, the map it generates may not be completely accurate.


\textbf{Exploration:}
Computationally, this application includes the same nodes as the \textit{Exploration} benchmark, as well as another node that constantly runs object detection algorithms to search for human victims as it explores unknown environments. The object detection node here runs on a GPU. The object detection algorithm must run fast, in order to allow the MAV to sweep a large area quickly, but they must also be highly accurate, to prevent the MAV from missing a victim due to a false negative.


\label{sec:characterization}
 possibly the bottlenecks, and a table with kernel times and their distribution.
 
 possibly the requirements compute wise and which platforms are suitable for them (refer back to the HIL and how we can conduct these conclusive studies)

\subsection{Environment and it's effects}
indoor/outdoor,
obstacle density, dynamic obstacle speed
\subsection{}

\end{comment}

 


==> tex/compute_system_interdependence.tex <==
\section {Compute Robot Interactions}
\label{sec:char}
Cyber-physical systems are a compilation of many intertwined components; Hence, the development of optimal compute subsystems require an understanding of the interaction across such subsystems (i.e., compute, mechanical (actuators),  battery, etc). 
Furthermore, similar to cross-compute layer optimization widely adopted by the compute system designers,
robot's cross-system considerations and optimizations are highly desirable.

To this end, in this section first we introduce a directed acyclic graph as a general tool to capture the robot's inter-dependencies; Then, we examine how such graph looks like for
our robot, i.e., a micro aerial quad. Furthermore, we provide high-level intuitive reasoning behind some interaction instances within this graph and leave the detailed quantification to the next section. Finally,
we propose a semantic clustering that guides us through experimentation and discussions.


\subsection{Cross-system Interaction Graph}
\blueDebug{par summary:explain graph:edges and nodes. define impact paths and do a graphical example}

Cyber-physical machines are a compilation of a different set of systems and sub-components all working together toward a specific mission. 
An optimal design, not only should consider the individual components in isolation, but also investigate the interactions and furthermore take advantage of the opportunities across different systems. 
Designers need to understand various ways in which these subsystems impact one another and the overall robot's behavior. 
We introduce the cross-system interaction DAG (CSIG) as a tool for such considerations (Figure \ref{fig:CSIG_general}). 
The graph consists of three types of vertices: 1. sub-system vertices 2. system variable vertices 3. interaction functions vertices.
``Sub-system'' vertices (denoted by rectangles) specify the subsystem makeup of the robot such as compute, actuators, sensors, and battery. 
``System variables and metrics'' vertices (denoted by non-filled circles) specify robot's internal variables such as
compute's throughput, system's mass, and acceleration. 
``Interaction function'' vertices (denoted by filled circles) specify functions that capture the nature and quantity of the interaction between adjacent variables. The edges in the graph, imply the existence and the direction of the interactions. 
To investigate the impact of one variable on another, we need to examine the paths starting with the first variable and ending with the second. We call each one of such paths ``impact paths''.
Figure \ref{fig:CSIG_general} shows two of such paths 
from $subsystem_{0}$ to $var_2$ each denoted with a different dashed pattern (i.e ".." and "\_\;\_"). To examine the total impact of $subsystem_0$ on $var_2$, each one of these paths needs to be considered and finally combined. Note that the combination function is determined by the immediate interaction function before the second vertex (marked with +).

\begin{figure}[t]
%\vspace{-5pt}
\centering
\includegraphics[trim=0 0 0 0, clip, width=.5\columnwidth]
{figs/cross_system_interaction_graph_general.pdf}
%\vspace{-23pt}
%\vspace{-15pt}
\caption{cross system interaction DAG (CSIG) captures the inter-dependencies between robot's subsystems.}
\vspace{5pt}
\label{fig:CSIG_general}
\end{figure}



\subsection{MAV's Cross-system Interaction Graph}
\blueDebug{par summary:SIG for our quad. exemplify two paths with short description. explain direct/indirect interactions. outro to case studies}
Figure \ref{fig:CSIG_combined} on the left, shows the CSIG graph for our quad robot. This section lists and discusses this graph's vertices in details.

\textbf{Subsystems Vertices:} As we have extensively detailed, our quadrotor consists of four subsystems, namely sensory, actuation, battery and compute subsystem. 

\textbf{System Variables and Metrics Vertices:} To capture our robot's intelligence and mobility 
and further probe into their interactions, we have equipped our CSIG with relevant system variables.
For example, we have included compute's performance variables such as throughput and latency and also motion dynamic/kinematic related variables such as mass, acceleration, and velocity. Furthermore, for system metrics, 
we focus on two mission metrics, i.e., mission time and mission energy. The choice of these metrics was due to their general significance across applications (package delivery, search and rescue, ...), robotics domains (robotics in Hazardous applications, 
robotics in construction, robotics in agriculture), and even robotic platforms with different constraints (flying, ground, or underwater robots).
It is worth noting that in general, the choice of system variables and metrics are highly robot, domain and application dependent.

\textbf{Interaction Function Vertices:} For our quadrotor, the interaction functions range from simple addition (marked by 1) to more complex linear functions (marked with 2) to non-linear relations (marked with 3). 


%Figure \ref{fig:CSIG_combined} on the left shows all paths 
In this paper, we turn our focus on the interactions between the compute subsystem and mission time and energy. 
Figure \ref{fig:CSIG_combined} on the right, highlights all such interactions. The red, blue, and purple edges respectively denote direct,
indirect, and hybrid interactions compute can have with other variables. 
For example, the red line between compute and latency shows that compute directly impacts
latency, whereas the blue line between latency and velocity shows the indirect way (i.e., through latency)  in which compute impacts velocity. We counted a total of  8 number of different paths
with which compute impacts mission time and energy.  We illustrate two of such paths with dashed lines, each with a 
different quantity and direction of impact. The coarse grain ("\_\;\;\_") dashes show how compute
impacts mission's energy by traversing through latency, velocity, and mission time vertices. Through this path, an increase in compute capability, reduces latency, and as a result increasing velocity,
reducing mission time and finally leading to a reduction in mission energy. On the other hand, the fine grain path (denoted with "..") shows this impact through power directly, where an increase in compute
capability, increases the power consumption and hence increases mission energy (These paths along with others are detailed and quantified in the next 3 section). 
\begin{figure*}[!t]
%\vspace{-5pt}
\centering
\includegraphics[trim=0 0 0 0, clip, width=\linewidth]
%{figs/blah_}
{figs/cross_system_interaction_graph_combined}
%\vspace{-23pt}
%\vspace{-15pt}
\caption{cross system interaction DAG captures the inter-dependencies between the robot's subsystems. left: all interactions right: compute interactions (direct/indirect)}

\label{fig:CSIG_combined}
\end{figure*}
\begin{comment}
In the previous section, the concept of compute-system interdependence was introduced 
through a data structure called CSIG in which edges denote dependence/interactions. 
We can identify the interactions between two vertices (e.g., compute sub-system and mission time), 
by traversing and combining each of paths (from now on called impact paths) that starts from one and end with the other one. 
In this (and the following two) section(s), we
detail the reasoning behind each impact path shown in \red{figure blah}. Furthermore, 
through theory, system modeling, and experimentation, we quantify the direction and magnitude of each impact path.
Without the loss of generality, in this paper, we specifically focus on the interactions (and hence the impact paths) between the compute subsystem and two mission metrics, i.e., mission time and mission energy. The choice of these metrics was due to their general significance across applications (package delivery, search and rescue, ...), robotics domains (robotics in Hazardous applications, 
robotics in construction, robotics in agriculture), and even robotic platforms with different constraints  (flying, ground, or underwater robots).
\end{comment}

To investigate the impact of compute subsystem on mission time and energy, we bin the impact paths 
(that start from compute and end with mission energy or mission time) into 3 clusters: 
    1. impact paths that originate from compute's performance (i.e., through latency and throughput)
    2. impact paths that originate from compute's mass.
    3. impact paths that originate from compute's power.

In the next section, through theory, system modeling, and experimentation, we quantify the direction and magnitude of each of the aforementioned
clusters and their corresponding impact paths.



==> tex/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% MAVs have seen an outburst of attention recently, specifically in the area with a demand for autonomy. Despite their ample use cases, e.g., package delivery, and high constraints, e.g., power and performance, these systems have seen a modest examination from the software and hardware architects. 
We show that a tight interaction between
the cyber and physical processes dictates autonomous mobile machines' behavior. Hence, a robot design methodology needs to consider such interactions for optimal results. Furthermore, this consideration
can uncover co-design (cyber-physical co-design)
opportunities, similar to hardware-software co-design, to be taken advantage of. This paper sets its goal as to probe and investigates the cyber and physical interactions of Micro Aerial Vehicles (MAVs) as examples of complex
robots. We frame this goal as a simple question: \textit{what is role of compute in the operation of autonomous MAVs?}
To answer this question, we combine analytical models, benchmarks and simulations showing how \textit{fundamentals of compute and motion are interconnected}.
For our analytical models, we use detailed physics, capturing compute's impact on various mission metrics. For our simulator and benchmarks, we address the lack of systematic benchmarks and
infrastructure for research by developing MAVBench, a first of its kind platform for the holistic evaluation of aerial agents, involving a closed-loop simulation framework and a benchmark suite. Using
our tool sets, we provide two optimization case studies through which we improve mission time and energy. 
As a concluding remark, while we focus on autonomous drones, the lessons learned about the role of computing, and the simulation methodology (i.e., closed/hardware in the loop) readily extend to other autonomous machines and robots.
By open sourcing our tool-sets, we hope to \textbf{(1)} help raising the
understanding of compute subsystem (system) designers of cyber-physical machines, \textbf{(2)} enable the cyber-physical co-design paradigm, and \textbf{(3)} start a closer discussion/collaboration between the robotics and
system design communities. 

%MAVBench facilitates the integrated study of performance and energy efficiency of not only the compute subsystem in isolation but also the compute subsystem's dynamic and runtime interactions with the simulated MAV. 




%MAVBench is a tool including a closed-loop simulation platform and a benchmark suite to probe and understand the intra-system (application data flow) and inter-system (system and environment) interactions of MAVs. This enables us to pinpoint bottlenecks and identify opportunities for hardware and software co-design and optimization. Using our setup and benchmark suite, we uncover a hidden compute to total system energy relationship where faster computers can allow drones to finish missions quickly, and hence save energy. This is because most of the drone's energy is consumed by the rotors, hence, faster compute can cut down on mission time (by increasing the max velocity and reducing the hovering time) and energy accordingly. Our insight allows us to improve MAV's battery consumption by up to 1.8X
%life by up to 43\% 
%for our OctoMap case study. 

\section*{Acknowledgements}

This material is based upon work supported by the NSF under Grant No. 1528045 and funding from Intel and Google.


\begin{comment}
On large drones, power goes mainly to motors, no matter how performant a processor is used. On smaller drones, the power consumed by processors becomes much more significant.

Faster computers can allow drones to finish missions faster, saving energy.

Such-and-such applications perform best with computers with such-and-such architectures. For example, such-and-such applications require faster parallel computers, while other applications depend upon fast serial performance.

We introduce a benchmark suite that can be used to test drone performance.
\end{comment}


==> tex/diff.tex <==
%DIF < \section{Compute-driven, Flight-Efficiency Optimization: A Case Study}
\section{\DIFaddbegin \DIFadd{Compute-driven, Flight-Efficiency Optimization: A }\DIFaddend Case \DIFdelbegin \DIFdel{Studies}\DIFdelend \DIFaddbegin \DIFadd{Study}\DIFaddend }
\label{sec:case-study}

Our closed-loop simulation platform, together with our plug and play benchmarks, enables a holistic inspection of intra-system and system/environment interactions. Studying of the former open doors for hardware/software co-design studies. Such studies starts with the profiling and sensitivity analysis as exemplified in the previous section. The latter enables environment focused considerations and designs such \DIFdelbegin \DIFdel{as reliability studies%DIF < , i.e. the effect of various localization kernels and collision avoidance algorithms on the system. 
}\DIFdelend \DIFaddbegin \DIFadd{reliability studies, i.e. the effect of various localization kernels and collision avoidance algorithms on the system. }\DIFaddend In this section \DIFdelbegin \DIFdel{, we conduct performance, energy and reliability case studies  highlighting the insights architects can take advantage of by using our platform.   
}%DIFDELCMD < \red{\subsection{Sensor-cloud: A Performance Case-Study}
%DIFDELCMD < As opposed to the studies provided in the previous section where our setup emulated a fully-on-edge drone (i.e. a drone which all of its computation is done on the drone itself), our setup can further examine a cloud/edge drone where the computation is distributed across the edge and the cloud. To examine the impact of cloud computing for MAVs, we compare a fully-on-edge drone equipped with a TX2 versus a fully-in-cloud drone with only a minimal computer on board (i.e. a flight controller) but a powerful cloud support (mention the x86 platform we used). This case study targets Mapping as the application of choice. As can be seen in Fig.\ref{fig:edge_cloud}, a drone that can enjoy the cloud's extra compute power sees a 3X speed up in planning time. This improves the average velocity of the drone due to the reduction in hover time and hence reduces the overall mission time almost to half.
%DIFDELCMD < }
%DIFDELCMD < \begin{figure}[t!]
%DIFDELCMD < \centering
%DIFDELCMD < \includegraphics[trim=0 0 0 -25, clip, width=0.9\linewidth]{figs/tx2-desktop}
%DIFDELCMD < %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{Comparing a full-on-edge drone vs a full-on-cloud drone.}}
%DIFAUXCMD
%DIFDELCMD < \label{fig:cloud_edge}
%DIFDELCMD < \end{figure}
%DIFDELCMD < %%%
\subsection{\DIFdel{Environment Aware Design: An Energy Case-Study}}  
%DIFAUXCMD
\addtocounter{subsection}{-1}%DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{we consider an example of the latter.   
}

\DIFaddend We conduct a kernel/environment sensitivity analysis using the OctoMap node~\cite{octomap}, which is a major bottleneck in \DIFdelbegin \DIFdel{3 of our end to  applications, namely package package delivery, mapping and search and rescue}\DIFdelend \DIFaddbegin \DIFadd{our benchmark suite}\DIFaddend . OctoMap is used for modeling of various environments without prior assumptions. In order to do so, the map of the environment is maintained in an efficient tree-like data structure while keeping track of the free, occupied and unknown areas. Both planning and collision avoidance kernels utilize this data structure to make safe flights possible by only allowing the drone to navigate through free spaces.  

\DIFdelbegin %DIFDELCMD < \begin{figure}[b]
%DIFDELCMD < \centering
%DIFDELCMD < \includegraphics[trim=0 0 0 -25, clip, width=\columnwidth]{figs/octomap_resolution_with_boxes}
%DIFDELCMD < %%%
%DIF < \vspace{-30pt}
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{OctoMap accuracy (resolution) versus performance.}}
%DIFAUXCMD
%DIFDELCMD < \label{fig:octrest}
%DIFDELCMD < \end{figure}
%DIFDELCMD < 

%DIFDELCMD < \begin{figure*}[t!]
%DIFDELCMD <     \centering
%DIFDELCMD <     \begin{subfigure}{.23\linewidth}
%DIFDELCMD <         \centering
%DIFDELCMD <         \includegraphics[trim=0 -10 0 -10, clip, width=\textwidth]{figs/garage_sim}
%DIFDELCMD <        \vspace{-30pt}
%DIFDELCMD <         %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{Environment's Map}}%DIFAUXCMD
%DIF < Level-1 Evaluation}
         %DIFDELCMD < 

%DIFDELCMD <         %DIFDELCMD < \label{fig:game:level-1}%%%
%DIFDELCMD <     \end{subfigure}
%DIFDELCMD <     \hfill
%DIFDELCMD <     \begin{subfigure}{.23\linewidth}
%DIFDELCMD <         \centering
%DIFDELCMD <         \includegraphics[trim=0 -10 0 -10, clip, width=\textwidth]{figs/garage_rviz__15}
%DIFDELCMD <        \vspace{-30pt}
%DIFDELCMD <        %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{resolution of .15 }\emph{\DIFdelFL{(m)}}%DIFAUXCMD
}
        %DIFAUXCMD
%DIFDELCMD < \label{fig:rviz__15}
%DIFDELCMD <     \end{subfigure}
%DIFDELCMD <     \hfill
%DIFDELCMD <      \begin{subfigure}{.23\linewidth}
%DIFDELCMD <         \centering
%DIFDELCMD <         \includegraphics[trim=0 -10 0 -10, clip, width=\textwidth]{figs/garage_rviz__5}
%DIFDELCMD <        \vspace{-30pt}
%DIFDELCMD <        %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{resolution of .5 }\emph{\DIFdelFL{(m)}}%DIFAUXCMD
}
        %DIFAUXCMD
%DIFDELCMD < \label{fig:game:rviz__5}
%DIFDELCMD <     \end{subfigure}
%DIFDELCMD <        \hfill
%DIFDELCMD <    \begin{subfigure}{.23\linewidth}
%DIFDELCMD <         \centering
%DIFDELCMD <         \includegraphics[trim=0 -10 0 -10, clip, width=\textwidth]{figs/garage_rviz_1}
%DIFDELCMD <         \vspace{-30pt}
%DIFDELCMD <         %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{resolution of .8 }\emph{\DIFdelFL{(m)}}%DIFAUXCMD
}%DIFAUXCMD
%DIF < Level-3 Evaluation}
        %DIFDELCMD < \label{fig:game:rviz_1}
%DIFDELCMD <     \end{subfigure}
%DIFDELCMD <     \hfill
%DIFDELCMD <    \vspace{+30pt}
%DIFDELCMD <    %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
%DIFDELCMD < \small %%%
\DIFdelFL{Drone's environement }\emph{\DIFdelFL{(a)}} %DIFAUXCMD
\DIFdelFL{and its perception of it with various OctoMap resolutions (}\emph{\DIFdelFL{(b)}}%DIFAUXCMD
\DIFdelFL{, }\emph{\DIFdelFL{c}}%DIFAUXCMD
\DIFdelFL{, emph}%DIFDELCMD < {%%%
\DIFdelFL{d}%DIFDELCMD < }%%%
\DIFdelFL{).}}
    %DIFAUXCMD
%DIFDELCMD < \label{fig:octomap_perception}
%DIFDELCMD < \end{figure*}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend % Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\vspace*{7pt}
\centering
\caption{Switching between OctoMap resolutions dynamically leads to mission success compared to 0.8~cm, and compared to 0.15~cm we consume less energy and thus retain more battery.}
\label{tbl:octopt}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l|l|l|l|}
\cline{2-4}
                                                                 & \textbf{Resolution {(cm)}}       & \textbf{Mission Status} & \textbf{Battery  (\%)} \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Package Delivery}}} & \textit{0.8}              & \cellcolor{red!25}Fail                    &   0           \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{0.15}             & Pass                    &    81.00          \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{Chameleon (0.8, 0.15)} & Pass                    &   \cellcolor{green!25}86.00           \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Mapping}}}          & \textit{0.8}              & \cellcolor{red!25}Fail                    & 0           \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{0.15}             & Pass                    & 39.03        \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{Chameleon (0.8, 0.15)} & Pass                    & \cellcolor{green!25}53.83        \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Search and Rescue}}}              & \textit{0.8}              & \cellcolor{red!25}Fail                    & 0         \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{0.15}             & Pass                    & 24.21        \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{Chameleon (0.8, 0.15)} & Pass                    & \cellcolor{green!25}57.87        \\ \hline
\end{tabular}
}
\end{table}

Size of the voxels, i.e. the map's resolution, trades off accuracy and flight-time/energy. By lowering the resolution, i.e. increasing voxel sizes, obstacle boundaries get inflated, hence the drones perception of the environment and the objects within it becomes inaccurate. However, doing so improves the performance of the OctoMap node and eventually leads to a faster flight time. To examine the trade off, we ran OctoMap with various resolutions.
\DIFdelbegin %DIFDELCMD < \Fig{fig:octrest} %%%
\DIFdel{shows 4.5X speed up in the OctoMap's update rate for 6.5X reduction in accuracy. 
%DIF < \begin{comment}
}%DIFDELCMD < 

%DIFDELCMD < %%%
%DIF < \end{comment}
\DIFdelend %DIF > \Fig{fig:octrest} shows 4.5X speed up in the OctoMap's update rate for 6.5X reduction in accuracy. 
\DIFaddbegin \begin{comment}
\begin{figure}[b]
\centering
\includegraphics[trim=0 0 0 -25, clip, width=\columnwidth]{figs/octomap_resolution_case_study}
\caption{OctoMap accuracy (resolution) versus performance.}
\label{fig:octrest}
\end{figure}
\end{comment}
\DIFaddend Certain aspects of the environment such as obstacle density determine the OctoMap resolution. In low density environments, where the drone has ample opportunities for paths to take, a low resolution can suffice. However, in dense environments, low resolutions can deprive the drone from path opportunities present since the drone perceive the obstacles bigger than they are. \DIFdelbegin %DIFDELCMD < \red{The impact of OctoMap resolution on the drone's perception can be easily seen in figure blah, where figure blah-1 shows the environment and the figure blah-2 through 4 show the drone's perception of the environment. As observed, when the resolution is lowered, the voxel sizes increase to the point that the drone can fail to recognize openings as possible passage ways to plan through. This in turn can result in a mission inefficiency and possible failures depending on the environment}%%%
\DIFdel{.
}\DIFdelend Since the environment around the drone changes, a dynamic approach where the resolution is set on the runtime is desirable. We study two environments during the mission, namely outdoors (low obstacle density) and indoors (high obstacle density). 

Table~\ref{tbl:octopt} shows the result of two static (predetermined) resolutions, 15~cm and 80~cm, and our proposed dynamic approach (Chameleon) that multiplexes between the two appropriately. The dynamic approach allows for up to 2.3X improvement in endurance. As compute reduces, OctoMap bottleneck eases, and therefore the drone completes its mission faster. 

The table also highlights another interesting relationship. Statically choosing the 80~cm resolution to optimize for compute (only) causes the drone to fail its mission since it is unable to plan paths through narrow openings in the indoor environments. By switching between two resolutions according to the environments obstacle density, Chameleon is able to balance OctoMap computation with mission feasibility and energy, holistically. Therefore, in all cases, Chameleon uses less energy and retains more battery charge. \DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < \red{\subsection{Depth Sensor Noise: A Reliability Case-Study}}
%DIFDELCMD < \red{Vijay could you add the information flow introduction you mentioned.}
%DIFDELCMD < 

%DIFDELCMD < \red{In this case study we examined the impact of sensor noise on the performance of our package delivery application. We injected Gaussian noise with a range of standard deviations into the depth readings of the drone's RGBD camera. Sensory noise distorts the drone's perception of the obstacles in its environment, and we found that Gaussian noise in particular \emph{inflates} obstacles, making them appear larger than they actually are. This causes the drone to re-plan its trajectories more often, as it assumes that its planned path will collide into objects that are actually further away than they seem, as shown in figure blah. The more the drone re-plans its paths, the longer it takes to reach its destination, increasing mission time by blah percent.
%DIFDELCMD < }
%DIFDELCMD <  %%%
\DIFdelend

==> tex/evaluation.tex <==
\section{Evaluation Setup}
\label{sec:evaluation}

We want to study how for a cyber-physical mobile machine such as a MAV, \textit{the fundamentals of compute relate to the fundamentals of motion}. To this end, we combine theory, system modeling, and micro and end-to-end benchmarking using MAVBench. The next three sections detail our experimental evaluation and in-depth studies. We deploy our \csig to investigate paths that start from compute and end with mission time or energy. To assist the reader in the semantic understanding of the various impacts, we bin the impact paths into three clusters:
\begin{enumerate}
\item Performance impact cluster: Impact paths that originate from compute performance (i.e., sensing-to-actuation latency and throughput) which are shown in blue-color/coarse-grained-dashed lines in Figure~\ref{fig:CIG_performance_paths}.

\item Mass impact cluster: Impact paths that originate from compute mass which are shown in green-color/double-sided lines in Figure~\ref{fig:CIG_mass_paths}.

\item Power impact cluster: Impact paths that originate from compute power which are shown in red-color/fine-grained-dashed lines in Figure~\ref{fig:CIG_power_paths}.
\end{enumerate}

At first, we study the impact of each cluster on mission time (Section ~\ref{sec:comp_mission_time}) and energy (Section ~\ref{sec:comp_mission_energy}) separately. This allows us to isolate their effect in order to gain better insights into their inner workings. Then we combine all clusters together and study them holistically in order to understand their aggregate impact (Section~\ref{sec:impact_holistic}). 

\begin{figure}[t!]
\vspace{-12pt}
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0 0 0 0, clip, width=.46\columnwidth]
{figs/cyber_physical_interaction_graph_performance_paths.pdf}
\caption{Performance cluster. Impact paths influencing mission-time/energy through latency/throughput.}
\label{fig:CIG_performance_paths}
\end{subfigure}
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0 0 0 0, clip, width=.46\columnwidth]
{figs/cyber_physical_interaction_graph_mass_paths.pdf}
\caption{Mass cluster. Impact paths influencing mission time and energy through compute mass.}
\label{fig:CIG_mass_paths}
\end{subfigure}
\begin{subfigure}{\linewidth}
\centering
\includegraphics[trim=0 0 0 0, clip, width=.46\columnwidth]
{figs/cyber_physical_interaction_graph_power_paths.pdf}
\caption{Power cluster. Impact paths influencing mission time and energy through compute power.}
\label{fig:CIG_power_paths}
\end{subfigure}
\caption{Three impact clusters, performance, mass, and power,  impacting mission time and energy. Each cluster with all the paths contained in it are shown with a different color. Having the
cyber-physical interaction graph with different clusters enables the cyber-physical co-design advocated in this paper.}
\label{fig:CIG_all}
\end{figure}

% Using this clustering, we guide illustrate how through different impact paths, compute influences mission time and energy.
% Our discussions involve a combination of theoretical physics followed by micro and end-to-end benchmarking. 
% In this manner, first, through theory, we
% familiarize the reader with the fundamentals of motion ranging from 
% drone's dynamics and kinematics to drone's  power and energy. 
% We continue on the theory path illustrating how \textit{fundamentals of compute 
% relate to the fundamentals of motion}. Then, we provide simple microbenchmarks
% to isolate and verify the theory; Finally, we use our developed tool sets, i.e, our simulator 
% and benchmark suite, to conduct extensive end-to-end investigations.

In the \textbf{compute performance and power studies}, we conduct a series of sensitivity analysis using core and frequency scaling on an NVIDIA TX2. The TX2 has two sets of cores, a \textit{Dual-Core NVIDIA Denver 2}
and a \textit{Quad-Core ARM Cortex-A57}. We turned off the Denver cores during our experiments to ensure that the indeterminism caused by process to core mapping variations across runs would not affect our results. We profile and present the average velocity, mission, and energy values of various operating points for our end-to-end applications. 
%%To mainly focus on the impact of compute perforamnce and power (not mass), for these studies we 
%keep the compute platform (and hence its mass) the same.

In the \textbf{compute mass and holistic studies}, we use four different compute platforms with different compute capabilities and mass ranging from a lower-power TX2 to high-performance, power-hungry
Intel Core-i9. These studies model a mission where the drone is required to traverse a \SI{1}{\km} path to deliver a package. We collect sensing-to-actuation latency and throughput values by running a package delivery application as a micro benchmark for 30 times on each platform. Mission time is calculated using the velocity and the path length while the power and energy are calculated using our experimentally verified models provided in Section~\ref{sec:energy}. 
%Finally, maximum to average velocity conversion are calculated based on the environment congestion. 
%For compute mass studies in isolation, we have zeroed out latency and throughput
%alues to cut out their effect. However, in holistic studies (section~\ref{sec:impact_holistic}), 
%we bring back these values investigating their impacts.


==> tex/intro.tex <==
 %\section{Aerial Computing: Dream of an intelligent sky}
\section{Introduction}
Unmanned aerial vehicles (UAVs), or drones, are rapidly increasing in number. Between 2015, when the U.S. Federal Aviation Administration (FAA) first required every owner to register their drone, and
2018, the number of drones has grown by over 100\%. The FAA indicates that there are over a million drones in the FAA drone registry database (Figure~\ref{fig:faa-registrations}). Due in large part to an increasing set of use cases, including sports photography~\cite{drone-sports1}, surveillance~\cite{drone-surveillance}, disaster management, search and rescue~\cite{disaster-drone,nepal-earthquake-drone}, transportation and package delivery~\cite{Amazondel:online,CSD-Amazon-Drone-patents,drone-package-delivery-google}, %these unmanned aerial vehicles are on the cusp of demonstrating their full potential. and 
FAA predicts that this number will only increase over the next 5 years as indicated by the projections shown in Figure~\ref{fig:faa-prediction}.

% Such an optimistic upward trend can be explained by the new opportunities that unmanned aerial vehicles are enabling. With myriad use cases, such as in sports photography~\cite{drone-sports1}, surveillance~\cite{drone-surveillance}, disaster management, search and rescue~\cite{disaster-drone,nepal-earthquake-drone}, transportation and package delivery~\cite{Amazondel:online,CSD-Amazon-Drone-patents,drone-package-delivery-google}, and more, these unmanned aerial vehicles are on the cusp of demonstrating their full potential. 

% For example, by replacing the traditional forms of data collection from farming to project management on the construction site, drones have been reported to increase the time saving by 5-20X and hence reducing the costs up to 5X~\cite{dronedeploy:online}.

\begin{figure}[t!]
\centering
    \begin{subfigure}{.45\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/faa_results}
    \caption{Registered UAVs in the FAA database.}
    \label{fig:faa-registrations}
    \end{subfigure}
    \hspace{5pt}
    \begin{subfigure}{.52\columnwidth}
   \centering
    \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/Graph_FAA_Data}
    \caption{Predicted number of UAVs by the FAA.}
    \label{fig:faa-prediction}
    \end{subfigure}
       \caption{Currently and predicted number of registered UAVs according to FAA~\cite{FAA:online}. A visible growth indicates the significance of these vehicles which demands system designers attention.}
      \label{fig:current_predicated_UAVs}
\end{figure}


The growth and significance of this emerging new domain %involving autonomous agents 
calls for \emph{cyber-physical co-design} involving computer and system architects. Traditionally, the robotics domain has mostly been left to experts in mechanical engineering and controls. However, as we show in this paper, drones are challenged by limited battery capacity and therefore low endurance (how long the drone can last in the air). For example, most off-the-shelf drones have an endurance of less than 20 minutes ~\cite{CSD-Amazon-Drone-patents}. This need for greater endurance demands the attention of hardware and system architects. 
%and small battery capacities which lead to limited range of drones require hardware and system architects' attention. The limited onboard energy budget manifests itself in the limited endurance and range of drones. 

\newcommand{\csig}{cyber-physical interaction graph\xspace}

In this paper, we investigate how the compute subsystem in a cyber-physical mobile machine, such as a Micro UAV (MAV), can impact the mission time and energy and consequently the MAV's endurance. 
We illustrate that \textit{fundamentals
of compute and motion are tightly intertwined}. Hence, an efficient compute subsystem can directly impact mission time and energy. 
We use a directed acyclic graph, which we call the ``\csig", to capture the different ways (paths in the graph or ``impact paths'') through which compute can affect mission time and energy. %Each path within this map shows a particular way with which a subsystem such as compute can impact a mission metric. 
By analyzing the impact paths, one can observe the effect that each subsystem has on each mission metric. Furthermore, we can find out through which cyber and physical quantities (e.g., response time and compute mass) this impact occurs. 
%We semantically split the paths into three impact clusters, i.e., power, mass, and performance. We name each cluster after the cyber or physical quantity from which the compute impact originates.  We investigate these clusters first in isolation and then holistically. 

To study the different impact paths, we use a mixture of analytical models, benchmarks, and simulations. For our analytical models, we use detailed physics to show how compute impacts cyber and physical quantities and ultimately mission metrics such as mission time and energy. For example, through
derivation, we show how compute impacts response time, a cyber quantity, which impacts velocity, a physical quantity, which in turn impacts mission time. For our simulator and benchmarks, we address the lack of systematic benchmarks and infrastructure for research by developing MAVBench, a first of its kind platform for the holistic evaluation of aerial agents, involving a closed-loop simulation framework and a benchmark suite. MAVBench facilitates the integrated study of performance and energy efficiency of not only the compute subsystem in isolation but also the compute subsystem's dynamic and runtime interactions with the simulated MAV. 

% Our investigations use analytical models. We detail theoretical physics equations and show how cyber and physical quantities influenced by compute impact the entire MAV complex. For example, through
% derivation, we show how compute impacts mission time through a cyber quantity such as response time which itself impacts a physical quantity such as velocity. By understanding these relationships, the designers can design optimal MAVs.

% Our investigations also use benchmarks and simulations. To enable research, the foremost challenge to address is the lack of systematic benchmarks and infrastructure for research. To address this shortcoming, we introduce MAVBench, the first of its kind, a platform for the holistic evaluation of aerial agents, involving a closed-loop simulation framework and a benchmark suite. MAVBench facilitates the integrated study of performance and energy efficiency of not only the compute subsystem in isolation but also the compute subsystem's dynamic and runtime interactions with the simulated micro-aerial vehicle (MAV) as a whole.

%\red{Either remove the last sentence of the previous paragraph or the next three paragraphs. I think you can chose to remove the next three paragraphs because all of that info is in detail in sections 4 and 5 and really isn't needed here (I don't think).}

MAVBench, which is a framework that is built on top of AirSim~\cite{Airsim_paper}, faithfully captures all of the interactions a real MAV encounters and ensures reproducible runs across experiments, starting from the software layers down to the hardware layers. Our simulation setup uses a hardware-in-the-loop configuration that can enable hardware and software architects to perform co-design studies to optimize system performance by considering the entire vertical application stack, including the Robotics Operating System (ROS). Our setup reports a variety of quality-of-flight (QoF) metrics, such as the performance, power consumption, and trajectory statistics of the MAV.

MAVBench includes an application suite covering a variety of popular applications of micro aerial vehicles: %. We constructed five distinct and widely used applications:
\bench{Scanning}, \bench{Package Delivery}, \bench{Aerial Photography}, \bench{3D Mapping} and \bench{Search and Rescue.} MAVBench applications are comprised of holistic end-to-end application dataflows found in a typical real-world drone application. These applications' dataflows are comprised of several state-of-the-art computational kernels, such as object detection~\cite{yolo16,hog}, occupancy map generation~\cite{octomap}, motion planning~\cite{ompl}, localization~\cite{orbslam2,vins-mono}, which we integrated together to create complete applications. 

% The MAVBench environment has the ability to ``plug and play'' different computational kernels to study tradeoffs for the same task.


MAVBench enables us to understand and quantify the energy and performance demands of typical MAV applications from the underlying compute subsystem perspective. More specifically, it allows us to study how compute impacts cyber and physical quantities along with the downstream effects of those impacts on mission metrics. It helps designers optimize MAV designs by answering the fundamental question of \emph{what is the role of compute in the operation of autonomous MAVs?}

Using the analytical models, benchmarks, and simulations, we quantitatively show that compute has a significant impact on MAV's mission time and energy. We bin the various impact paths mentioned above to three clusters and study them separately and then simultaneously (holistically). First, by studying each cluster independently, we isolate its effect to gain a better insight into its impact, as well as its progress along the impact path. Second, by studying them simultaneously, we illustrate the clusters aggregate impacts. The latter approach is especially valuable when the clusters have opposite impacts, and hence understanding compute's overall impact requires a holistic outlook.

%In scenarios in which the clusters have opposite impacts, such holistic studies provides insights into which one of the competing clusters impacts,  drawing accurate conclusions in order to arrive at optimal design.


%Studying eaching clu When studying impact clusters in isolation, we observe a 5X, and 2X improvement in mission time through the performance and mass clusters, respectively, and a 5.8X, 2.7X, and 1.3X improvement in mission energy through performance, mass, and power clusters, respectively. The holistic examination uncovers a 1.8X and 1.5X difference in mission time and energy due to different compute subsystems. %\red{make sure this is all up to date}

%An off-the-shelf MAV, such as the DJI~Matrice~\cite{dji-matrice} or \solo~\cite{solo3DR}, consumes between 300~W to 400~W for its rotors, as much power as a typical data center server, with an average endurance that is typically less than 20 minutes. Compute on average consumes less than 5\% of that total system power.  A state-of-the-art compute platform like the Nvidia TX2 consumes about 10~W on average. However, the compute performed onboard by the TX2 can affect flight mission time by as much as 2X. We conduct frequency and core scaling experiments on the TX2 to demonstrate how the \emph{compute performance affects the drone's velocity, which in turns impacts its mission time, and consequentially the drone's total system energy consumption.}

Finally, we present two optimization case studies showing how our tool-sets combined with an understanding of the compute impact on the robot can be used to improve mission time and energy. In the first case study, we examine a sensor-cloud architecture for drones where the computation is distributed across the edge and the cloud to improve both mission time and energy. Such an architecture shows a reduction in the drone's overall mission time and energy by as much as 2X and 1.3X respectively when the cloud support is enabled. The second case study targets Octomap~\cite{octomap}, a computationally intensive kernel that is at the heart of many of the MAVBench applications, and demonstrates how a runtime dynamic knob tuning can reduce overall mission time and energy consumption to improve battery consumption by as much as 1.8X.

In summary, we make the following contributions:

\begin{itemize}
    \item We introduce an acyclic directed graph called the \csig to capture various impact paths that originate from compute in cyber-physical systems.
    \item We present various analytical models demonstrating these impacts for MAVs. 
    \item We provide an open-source, closed-loop simulation framework to capture these impacts. This enables hardware and software architects to perform performance and energy optimization studies that are relevant to compute subsystem design and architecture.
    \item We introduce an end-to-end benchmark suite, comprised of several workloads and their corresponding state-of-the-art kernels. These workloads represent popular real-world use cases of MAVs further aiding designers in their end-to-end studies.
    \item Combining our tool-sets and analytical models, we demonstrate the role of compute and its relationship with mission time and energy for unmanned MAVs.
    \item We use our framework to present optimization case studies that exploit compute's impact on performance and energy of MAV systems.
\end{itemize}

The rest of the paper is organized as follows. 
%\Sec{sec:background} gives background on UAVs and MAVs that is relevant to this paper. 
~\Sec{sec:background} provides a basic background about Micro Aerial Vehicles, the reasons for their prominence, and the challenges MAV system designers face.
\Sec{sec:MAV_cyber_physical_interaction} demonstrates the tight interaction between the cyber and physical processes of a MAV and introduces the ``cyber-physical interaction graph'' to capture how these two processes impact one another.
Architects simulators and benchmarks need to be updated to model such impacts. To this end, \Sec{sec:simulation} describes the MAVBench closed-loop simulation platform, and \Sec{sec:mavbench} introduces
the MAVBench benchmark suite and describes the computational kernels and full-system stack it implements.  \Sec{sec:evaluation} then describes our evaluation setup, and \Sec{sec:comp_mission_time},
\Sec{sec:comp_mission_energy}, and \Sec{sec:impact_holistic} use a combination of our analytical models, simulator, and benchmarks to dissect the impact of compute on MAVs. 
\Sec{sec:optimizations} presents two case studies exemplifying optimizations of the sort that system designers can exploit to improve mission time and energy, \Sec{sec:related} presents the related work, and finally, \Sec{sec:conclusion} summarizes and concludes the paper.


==> tex/new_domain.tex <==
% \subsection{Cyber-physical Domain, A New Domain with New Characteristics Demanding New Toolsets} 

Investigating the cyber and physical interactions of the sorts mentioned above requires new tools. This is due to the numerous differences between cyber-physical systems and their more traditional counterparts (i.e., desktops, servers, smartphones, etc.).
Such differences need to be appreciated, and the architects' tool sets need to be adjusted accordingly. In this paper, we mainly focus on two major difference, namely (1) continuous interaction of the system with its complex and unpredictable surrounding environment, an aspect that is void in traditional systems, and (2) a closed-loop data-flow. 

To enable various system design research and development, we provide a simulator (Section~\ref{sec:simulation}) and a benchmark suite (Section ~\ref{sec:mavbench}) to model the MAV-environment close interactions. Furthermore, the environments' complexity is captured with high fidelity using a game engine. And finally, the closed-loop data flow nature of these systems are modeled using hardware in the loop simulator. 
In the next two sections, we discuss each of these tools in detail. It is worth noting that although this paper mainly focuses on Micro Aerial Vehicles (MAVs), the generality of our simulation framework allows for the investigation of other autonomous machines (e.g., AirSim now supports cars as well). With this, we hope to systematically bootstrap a collaboration between the robotics and system design community---an opportunity for domain-specific architecture specialization. 



==> tex/optimization.tex <==
\section{Context-Sensitive Optimization}
\label{sec:optimization}

As was shown in the previous section, the OctoMap generation node plays a crucial role in performance and energy consumption of drones.
This node is used for modeling of various environment without prior assumptions. In order to do so, the map of the environment is maintained in an efficient tree-like data structure while keeping track of free, occupied and unknown areas. Both planning and collision avoidance kernels utilize this data structure to make safe flights possible by only allowing the drone to navigate through free spaces.  

size of the voxels, i.e. the map's resolution, trades off accuracy and flight-time/energy. By lowering the resolution, i.e. increasing voxel sizes, obstacle boundaries get inflated, hence drones perception of the environment and the objects within it becomes inaccurate. However, doing so improves the performance of the OctoMap generation node and eventually leads to a faster flight time.  As figure blah shows blahx speed up in the update rate of OctoMap is achievable for a sacrifice of blahx in resolution. 

To study the effect of this knob on our applications we conducted a study where the drone will conduct some part of its mission in less dense environment such as outdoors and part of it in more dense environment such as indoors. We 



the  the flight time and the energy consumption of the drone. This node is responsible for providing the 


==> tex/optimizations.tex <==
\section{Compute Optimization Impact on Mission Time and Energy}
\label{sec:optimizations}
We use our benchmark suite, simulation environment, and the knowledge we acquired through examining compute's impact paths toward conducting two system optimization case-studies. We focus on the first and the third cluster (\Fig{fig:CIG_all}), i.e., optimizations exploiting the impacts through performance and power while leaving the second cluster for future work. The first case study examines the performance/power impact through a hybrid cloud-edge MAV complex, and the second one explores the performance/energy improvements through a runtime optimization. 




\subsection{A ``Cloud-Edge Offloading Optimization'' Case Study}
We examine a cloud/edge drone where the computation is distributed across the edge and cloud endpoints. We compare a fully-onboard compute drone equipped with a TX2 versus a fully-in-cloud drone with a powerful cloud support. The ``cloud'' computational horsepower is composed of an Intel i7 4740 @ 4GHz with 32 GB of RAM and a GeForce GTX 1080. For network connectivity, we utilize a 1Gbp/s LAN, which mimics a future 5G network~\cite{agyapong2014design, gupta2015survey}.

\begin{figure}[t!]
\centering
    \begin{subfigure}{.5\columnwidth}
    \centering
    \includegraphics[trim=5 0 20 0, clip, height=1.3in]{figs/tx2-desktop_performance}
    \caption{Performance.}
    \label{Perforamnce}
    \end{subfigure}
    %\hfill
    \begin{subfigure}{.4\columnwidth}
    \centering
    \includegraphics[trim=5 10 0 0, clip, height=1.3in]{figs/tx2-desktop_energy}
    \caption{Energy.}
    \label{fig:cloud-edge-energy}
    \end{subfigure}
\caption{Comparing a fully-onboard compute drone versus a fully-on-cloud drone. Our system allows part or portion of the MAVBench workloads to be offloaded to the cloud.}
\label{fig:cloud_edge}
\end{figure}

We target the planning stage of the PPC pipeline and focus on the 3D Mapping as the application of choice to offload. As we show in \Fig{fig:cloud_edge}, a drone that can enjoy the cloud's extra compute power sees a 3X speed up in planning time. This improves the drone's average velocity due to hover time reduction, and hence reduces the drone's overall mission time by as much as 50\% (impact through compute performance). Reduction in mission time decreases the total system's energy consumption (Impact through performance). In addition, by offloading the computation to the cloud, and hence avoid embedding a powerful i7 machine on edge, drone's power and therefore total energy consumption is reduced (impact through power). The overall reduction in energy is 1.3X for a cloud-edge hybrid system vs. a full-on edge drone.  
%mission energy is effectively doubling its endurance. Note that by offloading the computation to the cloud, the power that would be consumed by the powerful i7 machine is also  





\begin{comment}
\begin{figure}[t]
\vspace{0pt}
\centering
\includegraphics[trim=0 0 30 0, clip, width=.5\columnwidth]{figs/octomap_resolution_case_study}
%{figs/octomap_resolution_with_boxes}
\caption{Reduction in OctoMap resolution (accuracy) can be traded off with processing time. Increasing the $x$-axis means larger voxels to represent the space more coarsely (less accurately). A 6.5X reduction in resolution results in a 4.5X improvement in processing time.}
%\vspace{15pt}
\label{fig:octrest}
\end{figure}
\end{comment}

\subsection{A ``Context-Aware Runtime System'' Case Study} 
Focusing on energy efficiency, we conduct a kernel/environment sensitivity analysis using the OctoMap node~\cite{octomap}, which is a major bottleneck in three of our end to end applications, namely package delivery, 3D mapping and search and rescue. OctoMap is used for the modeling of various environments without prior assumptions. The map of the environment is maintained in an efficient tree-like data structure while keeping track of the free, occupied and unknown areas. Both planning and collision avoidance kernels use OctoMap to make safe flight possible, via costly compute cycles, by only allowing navigation through free space. Due to its implementation efficiency, OctoMap is widely adopted in the robotics community. Its broad adoption and impact in two out of three stages (Perception and Planning) make this kernel highly general and important for optimization.
\begin{figure*}[!t]
    \centering
    \begin{subfigure}[t]{.43\linewidth}
        \centering
        \includegraphics[width=2.2in]{figs/garage_sim}
         %\vspace{-20pt}
        \caption{Environment's map.}%
        \label{fig:garage_sim}
    \end{subfigure}
   \hspace{20pt}
    \begin{subfigure}[t]{.43\linewidth}
        \centering
        \includegraphics[width=2.2in]{figs/garage_rviz__15}
         %\vspace{-20pt}
        \caption{0.15~\emph{m} resolution.}
        \label{fig:rviz__15}
    \end{subfigure}
       
     \begin{subfigure}[t]{.43\linewidth}
        \vspace{5pt}
        \centering
        \includegraphics[width=2.2in]{figs/garage_rviz__5}
     % \vspace{-20pt}
     \caption{0.5~\emph{m} resolution.}
        \label{fig:game:rviz__5}
    \end{subfigure}
       %\hfill
   \hspace{20pt}
   \begin{subfigure}[t]{.43\linewidth}
          \vspace{5pt}
        \centering
        \includegraphics[width=2.2in]{figs/garage_rviz__1.pdf}
        %\vspace{-20pt}
        \caption{0.80~\emph{m} resolution.}
        \label{fig:game:rviz_1}
    \end{subfigure}
    %\hfill\\[15pt]
   \caption{For the environment in \emph{(a)}, OctoMap's resolution impact on the drone's perception of its environment is shown in \emph{(b)}, \emph{(c)}, \emph{(d)}. Large resolution means larger voxel size (lower is better).}
    \label{fig:octomap_perception}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \begin{subfigure}[t]{.49\linewidth}
        \centering
        \includegraphics[trim=0 0 30 0, clip, width=1\columnwidth]{figs/octomap_resolution_case_study}
        \caption{Octomap resolution Vs. performance time.}%
        \label{fig:octres}
    \end{subfigure}
  % \hspace{20pt}
    \begin{subfigure}[t]{.49\linewidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=1\columnwidth]{figs/energy-case-study}
        \caption{Context-aware Octomap resolution tuning.}
        \label{fig:dual-res}
    \end{subfigure}
\caption{\emph{(a)} Reduction in OctoMap resolution (accuracy) can be traded off with processing time. Increasing the $x$-axis means larger voxels to represent the space more coarsely (less accurately). A 6.5X reduction in resolution results in a 4.5X improvement in processing time. \emph{(b)} Switching between OctoMap resolutions dynamically leads to successfully finishing the mission compared to 0.80~m. It also leads to battery life improvement compared to 0.15~m. The $y$-axis in the top graph is the battery left on the drone upon mission completion.}
\end{figure*}

The voxel size in OctoMap, i.e., the map's resolution, introduces accuracy versus flight-time/energy tradeoff. By lowering the resolution, i.e., increasing \emph{voxel} sizes, obstacle boundaries get inflated; hence, the drone's perception of the environment and the objects within it becomes inaccurate. We illustrate the impact of OctoMap resolution on the drone's perception using \Fig{fig:octomap_perception}. \Fig{fig:garage_sim} {shows the environment and  Figures~\ref{fig:rviz__15}, \ref{fig:game:rviz__5}, \ref{fig:game:rviz_1} show the drone's perception of the environment as a function of OctoMap resolution. When the resolution is lowered, the voxels size increases to the point that the drone fails to recognize the openings as possible passageways to plan through (Figure~\ref{fig:game:rviz_1}). This results in mission time inefficiency and failures depending on the environment. In some cases, if the resolution is too large, the drone can't find a path to complete its mission.

To examine the accuracy versus performance tradeoff, we measured OctoMap kernel's processing time (running in isolation) while varying its resolution knob. \Fig{fig:octres} shows that as planning resolution increases (i.e., voxels are larger so space is represented more coarsely and hence less accurately), performance improves dramatically because less compute is needed. Going from one extreme to another, when the planning resolution goes from less than 0.2~m to 1.0~m ($x$-axis), OctoMap's processing time (or update rate) goes from more than 0.4~seconds to less than 0.1~seconds ($y$-axis). A 6.5X reduction in accuracy results in a 4.5X improvement in processing time.

\begin{comment}
\begin{figure}[t]
%\vspace{-5pt}
\centering
\includegraphics[trim=0 0 0 0, clip, width=.7\columnwidth]
%\includegraphics[trim=0 0 -5 -25, clip, width=0.9\linewidth]
%\includegraphics[height=5cm,keepaspectratio]
%\includegraphics[width=\columnwidth]%
%\includegraphics[trim={0 0 0 5cm}, clip, width=\columnwidth]%
{figs/energy-case-study}
\vspace{-15pt}
\caption{Switching between OctoMap resolutions dynamically leads to successfully finishing the mission compared to 0.80~m. It also leads to battery life improvement compared to 0.15~m. The $y$-axis in the top graph is the battery left on the drone upon mission completion.}
%\vspace{15pt}
\label{fig:dual-res}
\end{figure}
\end{comment}


\begin{comment}
\begin{table}[t]
\vspace*{20pt}
\centering
\vspace{-14pt}
\caption{Switching between OctoMap resolutions dynamically leads to mission success compared to 0.8~m, and compared to 0.15~m we consume less energy and thus retain more battery.}
\label{tbl:octopt}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l|l|l|l|}
\cline{2-4}
\textbf{Resolution {(m)}}       & \textbf{Mission Status} & \textbf{Battery  (\%)} \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Package Delivery}}} & \textit{0.8}              & \cellcolor{red!25}Fail                    &   0           \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{0.15}             & Pass                    &    81.00          \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{Chameleon (0.8, 0.15)} & Pass                    &   \cellcolor{green!25}86.00           \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Mapping}}}          & \textit{0.8}              & \cellcolor{red!25}Fail                    & 0           \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{0.15}             & Pass                    & 39.03        \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{Chameleon (0.8, 0.15)} & Pass                    & \cellcolor{green!25}53.83        \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Search and Rescue}}}              & \textit{0.8}              & \cellcolor{red!25}Fail                    & 0         \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{0.15}             & Pass                    & 24.21        \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{Chameleon (0.8, 0.15)} & Pass                    & \cellcolor{green!25}57.87        \\ \hline
\end{tabular}
}
\end{table}
\end{comment}


Certain aspects like obstacle density in the environment determine the ``ideal'' OctoMap resolution. In low-density environments, where the drone has many obstacle-free paths to take, a low resolution can suffice. In dense environments, low resolutions can deprive the drone of viable obstacle-free paths because the drone perceives the obstacles to be larger than they are in the real world, and so plans to avoid them. Since the drone's environment constantly changes, a dynamic approach where a runtime sets the resolution is ideally desirable.

We study two environments during the mission, namely outdoors (low obstacle density) and indoors (high obstacle density). \Fig{fig:dual-res} shows the result of two static (predetermined) resolutions, 0.15~m and 0.80~m, and our dynamic approach that multiplexes between the two appropriately.\footnote{Resolutions are based on the environment like the door width size. A 0.15~m resolution is chosen to ensure that the drone (diagonal width of 0.65~m) considers an average door (width of 0.82~m) as an opening for planning.} The dynamic approach allows improvement of battery consumption by up to 1.8X. 
%life for up to 43\%. To compute this improvement, we calculate the difference between the dynamic and static battery consumption and divide it by the static value. For example, for SAR, $\frac{(76\%- 43\%)}{76\%}$ leads to a 43\% improvement. 
Intuitively, as compute reduces, OctoMap bottleneck eases, and therefore, the drone completes its mission faster (impact through performance). The figure also highlights another interesting relationship that statically choosing the 0.80~m resolution to optimize for compute (only) causes the drone to fail its mission since it is unable to plan paths through narrow openings in the indoor environments. Instead, by switching between the two resolutions according to the environment's obstacle density, the dynamic approach is able to balance OctoMap computation with mission feasibility and energy, holistically. In all cases, the dynamic approach uses less energy and retains more battery at mission end time.






==> tex/performance.tex <==
\section{Performance Characterization}

% Characterizations of each of our micro- and macro-benchmarks. We describe which drone applications require parallel computer architectures, which ones require computers with fast serial performance, and which ones would benefit from parallel architectures but run fast enough on serial computers.

We plot the performance breakdowns of our micro-benchmarks in Fig~\ref{fig:micro-perf}. We found that computer vision kernels such as \textit{object detection} achieve high performance only on computers with highly parallel  architectures such as the TX1. We found that SLAM micro-benchmarks require such-and-such architecture to achieve high performance. We found that the path-finding micro-benchmarks achieve high performance on all our processors, but they achieve even higher performance on computers with such-and-such architecture.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/micro-perf}
\caption{Performance of computational micro-benchmarks on various companion computers.}
\label{fig:micro-perf}
\end{figure}

We plot the performance breakdowns of our macro-benchmarks when running in simulated environments designed for AirSim, as seen in Fig.~\ref{fig:perf-breakdown}. We find, in general, that computer vision tasks act as our applications' bottlenecks.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/perf-breakdown}
\caption{Performance breakdown of \textit{Person Tracking} benchmark on AirSim with various companion computers.}
\label{fig:perf-breakdown}
\end{figure}


==> tex/power.tex <==
\section{Power Characterization}

We characterized the power consumption of drones when executing simple flight maneuvers as well as when executing macro-benchmarks person-tracking.

As a drone's size increases, its motors become responsible for a larger and larger portion of its power consumption, until the motors consume nearly all the power generated by a drone. Fig.~\ref{fig:power-hover-solo} illustrates the power distribution on a large MAV such as the 3DR Solo, while Fig.~\ref{fig:power-hover-nano} illustrates the power distribution of a much lighter and smaller nano-aerial vehicle such as the Hummingbird.

\begin{figure}[h]
\centering

  \subfloat[Large micro-aerial vehicle.]
  {\includegraphics[width=.9\linewidth]{figs/power-hover-solo}
  \label{fig:power-hover-solo}}

  \subfloat[Small nano-aerial vehicle.]
  {\includegraphics[width=.9\linewidth]{figs/power-hover-nano}
  \label{fig:power-hover-nano}}

\caption{Resolution vs performance on the drone.}
\label{fig:power-distribution}
\end{figure}

Thus, as a drone's size falls, it's flight time increasingly depends upon the power consumed by its companion computer, as well as the power required to lift its computer into the air. In Fig.~\ref{fig:flight-time-tracking-tx1}, we plot the flight time of our drones when executing the \textit{Person Tracking} benchmark. The drones are equipped with a TX1 giving them 20 FPS performance.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/flight-time-tracking-tx1}
\caption{Flight time of drones when executing \textit{Person Tracking} benchmark with TX1.}
\label{fig:flight-time-tracking-tx1}
\end{figure}

In Fig.~\ref{fig:perf-tracking-10min}, on the other hand, we plot the performance of the \textit{Person Tracking} application when running on various drones equipped with the most performant computer that will allow them to achieve 10 minutes of flight time.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/perf-tracking-10min}
\caption{Performance of drones when executing \textit{Person Tracking} benchmark with 10 minutes of flight time.}
\label{fig:perf-tracking-10min}
\end{figure}

In Fig.~\ref{fig:energy-search-and-rescue}, we plot the total energy spent by our simulated AirSim drone when completing the \textit{Search-and-Rescue} macrobenchmark with various companion computers. As more powerful computers are used, our simulated drone is able to fly faster without missing potential targets and is thus able to complete its mission faster with less total energy expenditure.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/energy-search-and-rescue}
\caption{Energy expended by AirSim drone when executing \textit{Person Tracking} benchmark with various companion computers.}
\label{fig:energy-search-and-rescue}
\end{figure}


==> tex/related.tex <==
\section{Related Work}
\label{sec:related}
There is prior work that focuses on building analytical models, simulators and benchmark suites to aid the development of autonomous MAVs. We address some shortcomings of previous approaches by
providing a more detailed, integrated, end-to-end solution.

\paragraph{Analytical Models} There are numerous work such as ~\cite{quad_dynamics, quad_dynm2, quad_survey, energyaware} that model the MAV's physical quantities' impact on one another and ultimately MAV's
behavior. These works do not consider cyber quantities and their influence. There are a few works such as ~\cite{high-speed-nav, embedded_img_proc, how_fast_too_fast} that brush the surface of cyber quantities' impact on physical quantities and mission metrics. However, none,
take a detailed and holistic compute subsystem design perspective. For example, ~\cite{high-speed-nav} and ~\cite{how_fast_too_fast} only consider the relationship between response time and velocity whereas
~\cite{embedded_img_proc} does not consider acceleration, velocity or system throughput. 
In addition ~\cite{embedded_img_proc} and ~\cite{how_fast_too_fast} only examine one stage of the pipeline, i.e., the perception stage, whereas our applications enjoy the end-to-end characteristics. 

%difference with embedded_img_proc: 

%      - they don't use end-to-end apps (only image processing)
%      - they don't take into account system latency and response time(only through put)
%      - they don't take into account drone's velocity (and hence their flight time is just basically endurance)


\paragraph{Simulators} Simulators are essential to the study of aerial and robotic agents. Our simulation platform is built upon Microsoft's AirSim \cite{Airsim_paper}, a UAV simulator that uses the Unreal Game Engine to provide accurate physics models and photo-realistic environments. MAVBench uses the AirSim core and extends it with performance, power and battery models that are suited for architectural research, as well as with a gimbal, and dynamic and static obstacle creation capabilities that are not inherently part of AirSim. Another very popular simulator used in the robotics community for MAVs is Gazebo~\cite{gazebo}. However, Gazebo simulations lack photo-realism, while our work, with the help of AirSim and the Unreal Game Engine, enables more accurate visual modeling.

There are also numerous simulators widely used in industry and academia for studying autonomous agents such as ~\cite{boss-cmu,talos-mit,odin-vtech,uber-simulator, uav_benchmark_simulator, mujoco}. However, they either do not provide MAV models or does not consider the architectural insights.

%For instance, one such simulator, CARLA~\cite{carla} also uses the Unreal engine for photo-realistic representations of the environment. However, CARLA lacks models for MAVs, rotor dynamics and their interaction with the environment. For MAVs, there has been prior work~\cite{uav_benchmark_simulator} using simulators built on the Unreal game engine. However, unlike ours, their work mainly focuses on object tracking and does not go into the evaluation of the hardware platform and system architecture. 

A recent work FlightGoggles~\cite{flight-goggles}, creates virtual reality environments for drones using the images streamed from the Unity3D game engine. However, for maximum realism, FlightGoggles requires a fully functioning drone that must fly during tests, with its sensory data being streamed in from the game engine. MAVBench, on the other hand, does not have this constraint. Our users may provide real processors for hardware-in-the-loop simulation, but they are not required to fly the MAVs physically in the real world.

\paragraph{Benchmarks} Most robot benchmark suites target individual computational kernels, such as odometry or motion-planning, rather than characterizing end-to-end applications composed of many
different kernels. For example SLAMBench~\cite{slambench} and CommonRoad~\cite{common-road} solely focus on the perception and the planning stage respectively. However, our benchmarks allow for
holistic studies by providing end-to-end applications. 

\paragraph{Simulator + Benchmarks:} RoboBench~\cite{robobench} provides a common platform around simulators and benchmarks using software containers to combat software compatibility
problems across groups. This work is complementary to ours. 



%For example, there are numerous robotic vision datasets, such as KITTI~\cite{kitti}, and the EuRoC~\cite{euroc} MAV dataset, but these focus exclusively on the perception stage of a robot's computational pipeline. Others such as SLAMBench~\cite{slambench} and CommonRoad~\cite{common-road} lack 
%a software framework that characterizes the accuracy, performance, and energy consumption of RGB-D SLAM algorithms, and goes far deeper into its analysis of the SLAM computational kernel than we do in MAVBench. However, these tools do not provide insights into how SLAM interacts with other kernels in an end-to-end application. CommonRoad~\cite{common-road} is another benchmarking tool that characterizes motion-planning algorithms for autonomous cars, but computational kernels such as mapping and localization, that are necessary for an end-to-end characterization, are outside its scope.




==> tex/role_of_comp_hollistic.tex <==
\section{Role of Compute, a Holistic Outlook}
\label{sec:impact_holistic}
\blueDebug{
    section flow:
    - hollistic look at instead of in isolation (why)
    - explain the experiment very briefly
    - describe the data
    - motivate exhaustive DSE
    - explain data generation
        - explain how we arrive at this data 
        - explain bounderis
    - explain the results
}

The impact of compute clusters needs to be studied not only in isolation, as we have done so far to gain an in-depth understanding, but also simultaneously. The latter sheds light on the aggregate impact of all clusters together. Such a holistic outlook is especially valuable when the clusters have opposite impacts, i.e., one with a positive and the other with a negative impact on a mission metric. 

To this end, in this section, we study the simultaneous effect of all three clusters, performance, mass, and power, on mission time and energy. %These studies are necessary to arrive at an optimal design. 
Our studies, similar to Section~\ref{sec:comp_mass_impact_on_mission_time}, deploy a combination of benchmarking and analysis for a package delivery application.
First, we uncover various impacts by performing holistic analysis using the four platforms in Table~\ref{compute_platform_data}. Subsequently, we expand the design space to its boundaries, %as defined by the MAV's constraints. By looking at the entire design space, 
allowing designers to determine which impact clusters, and hence which design techniques,
are the most beneficial.

%For example, the upper limit of compute's induced mass
%is determined by the maximum payload drone can carry and still lift off the ground.

%we compare 4 different drones each equipped with a different compute platform. The experiment mimics a package delivery application travelling for a distance of \SI{1}{\km}. \red{are there any obstacles? What does the environment look like? which platform?}



\subsection{Compute Impact on Four Platforms}
\label{sec:eval_4_platforms}
Compute mass, power and performance, holistically, impact acceleration, velocity, mission time and energy. We use a combination of simulation and analysis to examine the various impacts collectively on a DJI Matrice 100 drone equipped with the four platforms mentioned previously in Table~\ref{compute_platform_data}. 
 
We find that increasing onboard compute capability impacts acceleration negatively. Figure ~\ref{fig:vel_acc_full_impact} shows this impact where we see an acceleration of \SI{9.8}{\meter/\second\squared} vs. \SI{2.3}{\meter/\second\squared}, i.e., a 4.4X decrease, when our MAV swaps the lightest (TX2) with the heaviest (i9) platform.
% \begin{comment}
% In contrast, an increase in compute has both a negative and positive impact on velocity. The positive impact is caused by the reduction in response time (i.e., sensing-to-actuation throughput and latency) whereas the negative impact is caused by the reduction in maximum acceleration which itself is caused by an increase in mass (see Equation~\ref{eq:runtime-compute_seq}). When combined, we see that a middle ground compute platform, i7, has the highest maximum velocity, i.e., \SI{5.8}{\meter/\second}. 
% But on the other hand, our least compute capable platform, TX2, has the least velocity, i.e., \SI{5}{\meter/\second}. This means that compute causes a 1.2X difference between our slowest and fastest MAVs. A DJI MAV with an i7 is faster than a DJI MAV with either the TX2 or Xavier due to the reduction in response time caused by more compute capability. However, increasing the compute capability to i9 does not improve the velocity due to the negative impact of the added mass outweighs the benefits of the response time reduction for this compute platform. 
% \end{comment}
In contrast, an increase in compute has both a negative and positive impact on velocity. 
Through the positive path, i.e., the performance cluster as we showed in Section~\ref{sec:comp_perf_impact_on_mission_time}, more compute reduces response time, and hence increases velocity. Consequently, robot designers should deploy more compute. On the other hand, through the negative path, i.e., the mass cluster as was described in Section ~\ref{sec:comp_mass_impact_on_mission_time}, more compute increases mass, and hence reduces acceleration and velocity. Consequently, robot designers should deploy less compute. A holistic study however enables us to weigh these competing impacts simultaneously. 

For our four platforms, when paths are examined in combination, we see that not the least nor the most compute capable system, but a middle ground compute platform, i7, has the highest maximum velocity, i.e., \SI{5.8}{\meter/\second}. Our most compute capable platform, i9, has the least velocity, i.e., \SI{4.9}{\meter/\second}. Compute causes a 1.2X difference between our slowest and fastest MAVs. A DJI MAV with an i7 is faster than a DJI MAV with either the TX2 or Xavier due to the reduction in response time caused by more compute capability. However, increasing the compute capability to i9 does not improve the velocity due to the negative impact of the added mass, which outweighs the benefits of the response time reduction for this compute platform. 


%Note that difference betwen the conclusion darwn in the holistic approach and the in isolation approach. In the in isolation approach, for mass we concluded that more compute results in a slower 

%outlook allows us to overcome the myopic conclusions drawn in section blah an blah.  

%At the same time, reducing compute will also reduce velocity as the increased response time will outweigh the benefits of the reduced mass. 

\begin{figure}[t!]
\centering
    \begin{subfigure}[b]{.52\textwidth}
   
    \centering 
   
   \includegraphics[height=1.5in]{figs/compute_holistic/a_v_holistic_cat.pdf}
   \caption{Velocity and acceleration.}
   \label{fig:vel_acc_full_impact}
   \end{subfigure} 
   \begin{subfigure}[b]{0.47\textwidth}
    \centering
    \includegraphics[height=1.5in]{figs/compute_holistic/mission_time_holistic_cat.pdf}
    \caption{Mission time.}
    \label{fig:comp_mt_full_impact}
    \end{subfigure}
    
    \vskip\baselineskip
   \begin{subfigure}[b]{.49\textwidth}
    \centering
   \includegraphics[height=1.5in]{figs/compute_holistic/power_holistic_cat.pdf}
    \caption{Mission power.}
    \label{fig:comp_power_energy_full_impact}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, height=1.5in]{figs/compute_holistic/mission_energy_holistic_cat.pdf}
    \caption{Mission energy.}
    \label{fig:comp_me_full_impact}
    \end{subfigure}
    \caption{Holistic impact of compute on mission metrics. The data enables cyber-physical co-design  where the designers consider the impact of compute's cyber quantities on the robot's physical quantities and further their ultimate impact on robot's end-to-end behavior and mission success. When all impacts are considered together, there is no obvious best design choice. For instance, the i7 has the best (shortest) mission time (highlighted in green) but the Xavier has the lowest mission energy (highlighted in red).}
      \label{fig:full impact}
\end{figure}
A similar trend to velocity, where the least nor the most compute capable system is ideal, is observed with mission time. Figure ~\ref{fig:comp_mt_full_impact} shows this impact where our fastest MAV with i7 has the shortest mission time, i.e., \SI{686}{\second}, comparing to our slowest MAV with i9 which has the longest mission time, i.e., \SI{809}{\second}. Between the two, i7 shows 15\% improvement. Slow down factor (SDR) expands the gap between the best (\SI{62}{\s}) and the worst (\SI{124}{\s}) mission time difference. This again reminds us that for higher congested spaces, more efficient design has a bigger impact.

% This again is a reminder of the need for extra attention under challenging environments.

More compute negatively impacts mission power consumption (Figure~\ref{fig:comp_power_energy_full_impact}). This is due to the high impact of mass on power as discussed in Section~\ref{sec:comp_perf_impact_on_mission_energy}. As such, our most compute capable and hence heaviest platform, i9, consumes the most power, i.e., \SI{770}{\watt}, comparing to the least compute capable and hence lightest platform, TX2, which consumes \SI{521}{\watt} power.
Note that the slow down ratio has a minor impact on power since the velocity (which gets impacted by SDR) has a minor effect on power, as discussed in Section~\ref{sec:comp_perf_impact_on_mission_energy}.  


%\red{I'd like to say something about the total of paths that impact mission time and energy}

In the case of mission energy, there are two competing clusters with opposite impacts. Through the positive path, i.e., performance cluster as we showed in Section ~\ref{sec:comp_perf_impact_on_mission_energy}, more compute results in less energy consumption due to the reduction of mission time. Hence, more compute is desirable. On the other hand,
through the negative path, i.e., the mass cluster as we showed in Section ~\ref{sec:comp_mass_impact_on_mission_energy}, more compute results in more energy consumption. Hence, robot designers should deploy less compute. However, when combined, we see that not the most nor the least compute capable platforms, but another middle ground platform, Xavier performs the best. Xavier burns only \SI{407}{\kilo \joule}, comparing to the least energy efficient design, i.e., i9, which burns \SI{623}{\kilo \joule} (Figure~\ref{fig:comp_me_full_impact}).
Higher slow down factor (SDR) expands the gap between the best and worst design which
reminds us that for higher congested spaces, more efficient design has a bigger impact.


In summary, the MAV with the best mission time is not necessarily the most energy efficient design or vice versa. For instance, in our example, the MAV with the best mission time which carries an i7 is not the most energy efficient design which carries an Xavier. This is because, with i7, the negative impact of higher power consumption outweighs the benefit of lower mission time. The choice between the Xavier and the i7 depends on whether mission time or energy has more significance for the task at hand. %It is also worth noting that for the congestion factor with SDR of 4, although the i7 seems to be superior from a mission time perspective, in reality, the MAV's energy consumption exceeds the total available battery energy that is available onboard (shown with a red line). Hence, the MAV would never actually finish the mission, leaving the Xavier as the most optimal design, for this level of congestion, for both mission time and energy. 

% \begin{comment}
% To better understand this, one should consider the implications of adding more compute to a system. Table \ref{tab:compute_impact} shows the elementary impacts of adding more compute. That is, these are the most pronounced and direct impacts, reality is much more complicated as can be observed in Sections \ref{sec:comp_mission_time} and \ref{sec:comp_mission_energy}.

% \begin{table}[!htb]
% \begin{tabular}{l|l|l}
% Compute Change          & Symptoms                       & System Impact                            \\ \hline
% More mass       & Slower $V_{max}$ and $a_{max}$                 & Worse mission time and energy          \\
% More power      & Higher total power consumption & Worse mission energy                   \\
% Shorter response time & Higher vmax                    & Better mission energy and mission time
% \end{tabular}
% \vspace{10pt}
% \caption{Elementary impact for adding more compute}
% \label{tab:compute_impact}
% \end{table}

% This table shows the impact of adding more compute to design, breaking it down to added mass, power and improved latency respectively. For mission time, there's a tradeoff between mass and improved latency, disregarding a possible overshoot of the maximum battery capacity. For mission time, however, power has a far more significant influence and is a major part of the tradeoff. In other words, adding more compute quickly becomes expensive energy wise, which means that the optimum for total mission energy often diverges from the compute platform most optimal for mission time. 

% Figure \ref{fig:comp_power_energy_full_impact} shows all compute's impact paths on mission energy.
% Since power is a combination of two factors, i.e., power and mission time, where one increases and the other decreases,
% a combining effect shows that mission energy consumption is reduced for some platforms and not all.
% This is very important since mission energy consumption can be a determining factor in mission's failure. If the 
% energy consumption goes above the total energy available in the battery, the mission can not be completed.

% \red{can we propose a new metric ppm and use that to measure the merit of our system}
% \red{can we show what power, performance and mass ideally should the designers look for if they want to keep
% reducing the mission energy}

% \end{comment}

\subsection{Expanding the Design Space}
\label{sec:eval_all_inclusive_DSE}
Understanding the compute subsystem's design space for a MAV, from both the cyber and physical perspective, can help guide the design process.
This section goes beyond the four platforms from Table~\ref{compute_platform_data} and provides an example of, and the insights gathered from, a full design space investigation. Concretely, we examine how the entire design space changes as a function of three compute subsystem quantities and clusters, i.e., compute mass, compute power and performance. 

%We design space boundaries and also the way it morphs along each axis (impact cluster) are studies for our DJI drone.

Our evaluation employs the same analytical and simulation-based models discussed in the previous subsection.
We assume that the quantities can be modified independently. 
%We do not make any assumptions about the relationship between the quantities, i.e.,
For example, we assume that we can increase or decrease mass without effecting response-time or power. MAV's constraints determine the bounds for each quantity.  The maximum payload that the drone can
carry and still lift off the ground determines the compute mass upper bound. The total available energy on board determines the response time and power upper bounds. If the compute
power causes the battery to drain fast enough, or the response time to be long enough (and hence the MAV's speed low enough) that the MAV becomes unable to complete its mission before it runs out of
battery, we discard this design point. For power, we also take into account the upper current limit the battery can provide.\footnote{Although we assume no relationship between the three quantities, in reality since compute impacts
all three simultaneously, there is an indirect relationship between them all. This narrows the design space beyond the constraints we have already put into place. %, but we suspect that depending on emerging technologies, such relationships can vary. Therefore, high-level insights are valuable. 
We are aware that sharpening such constraints and replacing our high-level models with more accurate ones will improve the insight details, nevertheless, 
we believe that lower resolution models have an essential role in the initial stages of the iterative design and development process.
We welcome the community's assistance in both refining and replacing the models and constraints while considering the accuracy-performance tradeoffs of such changes.}
%\red{DOES THIS BELONG HERE OR EARLIER? ISN'T THIS A CRITIQUE OF ALL OF YOUR ANALYSIS?}}

Our results are shown in Figure~\ref{fig:DS}, where we illustrate the mission time (Figure~\ref{fig:mt_ds}) and energy (Figure~\ref{fig:me_ds}) for a DJI Matrice 100 drone. Each point within the space corresponds to a DJI with a compute subsystem of a different mass, response time, and power. % (corresponding to our impact clusters).
Mission metrics are shown as heat maps on the fourth dimension. Hotter colors are higher and hence, less optimal.
To aid the visualization and further understand the internals of the design space, we slice the space with horizontal cuts, concretely five slices for each mission metric. 
Furthermore, for selected slices, we show the gradient plots (i.e., plots of the rate of change in the most optimal direction) to demonstrate various trends. We spend the rest of this section detailing some essential takeaways from this analysis.

\begin{comment}
In other words:

\begin{equation}
    \begin{split}
        mission\_time = f(m,P,\delta_{r\_latency}) \\
        mission\_energy = f(m,P,\delta_{r\_latency})
    \end{split}
\end{equation}

\end{comment}

%where the arrows denote the direction of the fastest slope.
%Semantically, fastest slope is the the direction that provide the most design improvement.


\begin{figure}[t!]
\centering
    \begin{subfigure}{.51\columnwidth}
   \includegraphics[width=\columnwidth]{figs/compute_holistic/design_space_time.png}
   \caption{Mission time design space.}
   \label{fig:mt_ds}
    \end{subfigure} 
    \begin{subfigure}{.48\columnwidth}
   \includegraphics[width=\columnwidth]{figs/compute_holistic/design_space_energy.png}
    \caption{Mission energy design space.}
    \label{fig:me_ds}
    \end{subfigure}
    \caption{Mission metrics design space with respect to different clusters. Mission metrics are shown as heatmaps where hotter is less optimal. The design space is sliced and only a selected set of slices are shown for the ease of visualization.}
    \label{fig:DS}
\end{figure}

%

%Figures \ref{fig:4D_time} and \ref{fig:4D_energy}
%show the heat map for mission time and energy. As seen, a simple walk toward the lowest 

First, as one quantity becomes less optimal, it shrinks the design space of the other two. This can be seen by looking at the reduction in the area of the slices for both mission metrics shown in Figure~\ref{fig:DS}. For example, for mission time (Figure~\ref{fig:mt_ds}), as the power consumption increases (moving up the $z$-axis), the design space slices see a reduction in area for mass and response time. For example, for a 4X increase in power quantity, i.e., from \SI{615}{\watt} to \SI{2415}{\watt}, we see a 5X reduction in the area associated with the mission time's design space. Similar trends are observed for mission energy. Note that such a reduction in the area leaves designers with less space (area) to explore and design within. 

Second, some quantities exhibit diminishing returns, where moving towards more optimal (in this case smaller) values of that quantity results in lower gains. We demonstrate this by showing the gradient plots corresponding to one selected slice from Figure~\ref{fig:mt_ds} and Figure~\ref{fig:me_ds}. The other slices follow the same trend. The slice data are shown in Figures~\ref{fig:mt_gradient_mass}, and ~\ref{fig:mt_gradient_response_time} for Figure~\ref{fig:mt_ds} and in 
Figures~\ref{fig:me_gradient_mass} and ~\ref{fig:me_gradient_power} for Figure~\ref{fig:me_ds}. In these plots, gradient magnitude, i.e., mission metrics' rate of change, is shown by the size of the arrows overlaid on the figure. A change in the size of these arrows when moving along the $y$-axis or the $x$-axis indicates a change in the gradient magnitude. 
%Reduction in the gradient magnitude which is shown with the reduction in arrow sizes indicates a smaller change in the mission metric of interest and hence a lower gain. 
\begin{figure}[t!]
\centering
    \begin{subfigure}{.48\columnwidth}
     \includegraphics[width=\columnwidth]{figs/compute_holistic/contour_field_time_mass.png}
     \caption{Mission time-mass gradient.}
     \label{fig:mt_gradient_mass}
    \end{subfigure}
   \begin{subfigure}{.48\columnwidth}
    \includegraphics[width=\columnwidth]{figs/compute_holistic/contour_field_time_response_time.png}
    \caption{Mission time-response time gradient.}
    \label{fig:mt_gradient_response_time}
    \end{subfigure}
    
    \vspace{2pt}
    \begin{subfigure}{.48\columnwidth}
     \includegraphics[width=\columnwidth]{figs/compute_holistic/contour_field_energy_mass.png}
     \caption{Mission energy-mass gradient.}
     \label{fig:me_gradient_mass}
    \end{subfigure}
   \begin{subfigure}{.48\columnwidth}
    \includegraphics[width=\columnwidth]{figs/compute_holistic/contour_field_energy_power.png}
    \caption{Mission energy-power gradient.}
    \label{fig:me_gradient_power}
    \end{subfigure}
     \caption{Mission metrics' gradient, the rate of change in the most optimal direction, and their components. Change in the gradient magnitude, shown in the arrow size, for a walk toward the center indicates diminishing return in (a), (b), and (c). However, in (d), gradient values stay the same since this gradient is equal to mission time which is not a function of power.}
         \label{fig:gradient}
\end{figure}

For mission time, lowering the mass reduces the gradient magnitude, indicating a smaller change in the mission time.
Figure~\ref{fig:mt_gradient_mass} shows that the size of the arrows shrinks as we lower the mass, i.e., as we move from top to bottom on the $y$-axis. 
Similarly, lowering the response time reduces the gradient magnitude of the mission time. Figure~\ref{fig:mt_gradient_response_time} shows that the size of the arrows shrinks as we lower the response time, i.e.,
as we move left along the $x$-axis.

For mission energy, a similar trend with respect to mass is observed (Figure~\ref{fig:me_gradient_mass}). However, such a trend is not universal across all quantities. For example, lowering power does not impact mission energy's gradient with respect to power. Figure~\ref{fig:me_gradient_power} shows that the size of the arrows stay the same as we lower the power, i.e., as we move left along the $x$-axis. This is because simply put, this gradient is equal to mission time which is not a function of power.
Hence, a change in power would not impact mission time, in other words, the gradient, and hence, the size of the arrows would not change.




Finally, different quantities have different impacts on mission time and energy. To demonstrate this, we use sensitivity analysis by comparing a mission metric's percentage change with respect to the quantities' percentage change. Table~\ref{tab:ds_sensitivity} shows the mean and variance for the sensitively values of different quantities throughout the entire design space. Mission time is most sensitive to the response time since the mean response time, i.e., 0.4, is the highest among the three quantities. In other words, improving the response time on average results in the mission time improvement the most. This means that if the drone's main objective is mission time optimality, system designers should focus their efforts on reducing the response time. On the other hand, mission energy shows equal sensitivity to all three quantities since the mean of all quantities are approximately the same, i.e., 0.4. This means that the designers who are focused on mission energy optimality should target the quantity whose improvement costs the least. It is worth noting power consumption does not have an impact on mission time, hence, the mean and variance are equal to 0. The lack of relationship is also shown in the cyber-physical interaction graph since there is no edge from power to mission time.
\renewcommand{\arraystretch}{1.5}
\begin{table}[t!]
\caption{Design space sensitivity to different compute related quantities. Higher mean means a higher sensitivity and hence a higher gain if the quantity is optimized.
The sensitivity analysis is done by comparing a mission metric's percentage change with respect to the quantities' percentage change.}
\footnotesize
\begin{tabular}{|l|c|c|c||c|c|c|}
\hline
     & \multicolumn{3}{c||}{\emph{Mission Time}} & \multicolumn{3}{c|}{\emph{Mission Energy}} \\ \hline
     & Response Time   & Mass   & Power  & Response time    & Mass   & Power   \\ \hline
Mean & .40             & .31    & 0      & .40               & .40     & .37     \\ \hline
Std  & .25             & .70    & 0      & .24              & .72    & .19     \\ \hline
\end{tabular}
\label{tab:ds_sensitivity}
\end{table}
\renewcommand{\arraystretch}{1}


%of each mission metric with respect to each cluster is calcualted throughout the Table blah shows the sensitivity of our mission metrics to each cluster. sensitiin other words, the sensitivity of the mission time and energy is different for each axis. This can be seen with the different rate with which colors change 
%with a walk along different axis. To assist the reader to see the change, we also show the gradient graph for two of the axis (as an example), where the gradient vector points at the direction of the most change. \red{have percent impact}. Table \ref{tab:gradients} shows the mean and standard deviations of these gradients for different axis. The same order of magnitude is visible for mass and response time, while power shows a much small gradients. In other words, changing the mass or response time is far more effective than changing the power consumption of compute in most cases. Note that since the gradient shows the direction of the most change, it can show the designers the optimal direction to walk along in order to gain the most amount of design improvements.
%space velocity discussion


% space acceleration discussion



%The difference between slice area for the highest and lowest slices associated with the response time difference of 2.41 is 
%mass and power design space are  22X smaller than a lower cut (i.e, response time of 0.41 seconds). 
% boundary argument

%Between these two planes, we see that the lower plane has a surface area \~ 22 times greater than the highest plane. 

%Figures \ref{fig:4D_energy} targets mission energy. Overall trends discussed in mission time hold for mission energy 
%as well. In addition, there's a significant impact of power on mission energy.

%Looking at Figures \ref{fig:4D_time} and \ref{fig:4D_energy}, one can see that the colour gradient is different in various directions. With this, the improvement in mission time and mission energy is most pronounced in a specific direction, for each point in the design space.
%acceleration argument
\\
%If a designer would want to improve MAV performance from a certain initial design point, one or more of the three properties power, mass and latency can be altered. It is of great use to know which parameters are most sensitive; what parameters cause the greatest improvement in mission performance. To further analyze this property of the design space, a slice of it with constant latency is shown in Figures \ref{fig:flow_field_time} and \ref{fig:flow_field_energy}. The arrows denote in which direction mission time and performance respectively improve fastest. For a certain design point, the arrows denote in which direction the design should move to improve mission characteristics in an efficient manner. Also notice the difference between both plots, where mission energy shows significant dependency on power while mission time does not show large changes for altering power.l





% %\subsubsection{Study Limitations}
% \begin{comment}
% \label{subsec:lims}
% To evaluate the validity of the insights obtained, assumptions have to be taken into account. 

% \begin{itemize}
%     \item Simulation is done on a single task
%     \item Simulation lacks fidelity compared to reality
%     \item A limited amount of slow-down factors is taken into account
%     \item The equations from Section \ref{sec:comp_mission_time} are non-ideal
% \end{itemize}
% \end{comment}

% \begin{comment}
% \subsection{Cyber-physical co-design}
% As shown throughout the paper, cyber and physical components of a robot interacts closely. This means that an optimal design needs to consider such interactions. The point here is that the optimization of either mission time or mission energy should be done strategically. Decreasing power, mass or latency will be beneficial for performance, but they have different implications. For certain design points it would be most effective to decrease mass, while for others lowering power would lead to the best results.
% \end{comment}


==> tex/role_of_comp_intro.tex <==
\begin{comment}
In the previous section, the concept of compute-system interdependence was introduced 
through a data structure called CSIG in which edges denote dependence/interactions. 
We can identify the interactions between two vertices (e.g., compute sub-system and mission time), 
by traversing and combining each of paths (from now on called impact paths) that starts from one and end with the other one. 
In this (and the following two) section(s), we
detail the reasoning behind each impact path shown in \red{figure blah}. Furthermore, 
through theory, system modeling, and experimentation, we quantify the direction and magnitude of each impact path.
Without the loss of generality, in this paper, we specifically focus on the interactions (and hence the impact paths) between the compute subsystem and two mission metrics, i.e., mission time and mission energy. The choice of these metrics was due to their general significance across applications (package delivery, search, and rescue, ...), robotics domains (robotics in Hazardous applications, 
robotics in construction, robotics in agriculture), and even robotic platforms with different constraints  (flying, ground, or underwater robots).
\end{comment}

\begin{comment}
To study the impact of compute subsystem on mission time and energy, we bin the impact paths 
(that start from compute and end with mission energy or mission time) into 3 clusters: 
    1. impact paths that originate from compute's performance (i.e., through latency and throughput)
    2. impact paths that originate from compute's mass.
    3. impact paths that originate from compute's power.

In the next 3 sections, through theory, system modeling, and micro benchmarking, we quantify the direction and magnitude of each of the aforementioned
clusters and their corresponding impact paths.
\end{comment}


==> tex/role_of_comp_mass.tex <==

\section{Compute's Mass Impact}
This section investigates the paths within the second cluster in detail. These are the paths with which the compute subsystem's mass impacts mission time and energy. 
The compute mass that needs to be carried by the quad consists of the board, the SOC and a cooling system. 
As the amount of compute on board increases, it escalates the Thermal design power (TDP). To battle the rise in TDP, a more robust and hence heavier cooling solution is required. 
In other words, an increase in the onboard compute capability exacerbate the weight that the quad needs to carry. Table ~\ref{compute_platform_data} illustrates 
the mass associated with 4 different SOCs
each with a different compute capability. 
As we observe, the overall compute subsystem's weight can experience a 7.5X 
increase contributing to a 1.5X increase in the entire drone's mass. 
%\renewcommand{\arraystretch}{.5}
\begin{table*}[]
\caption{characteristics of various platforms used for our experiments}
\resizebox{\columnwidth}{!}{

\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{3}{|c|}{Compute Platform}                                                                                                       & \multicolumn{3}{c|}{Performance}                                                                                                                                                                                                                   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Thermal\\  Power \\ (W)\end{tabular}} & \multicolumn{3}{c|}{Mass}                                                                                                                                                                                                                                 \\ \cline{1-6} \cline{8-10} 
Name          & \multicolumn{1}{l|}{Number of Core} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}CPU \\ Frequency\\  (GHz)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Latency \\     (s)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Throughput\\      (Hz)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Total\\   (s)\end{tabular}} &                                                                                  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Board and\\  processor\\  (g)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Heat \\ Sink \\ (g)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Total \\ (g)\end{tabular}} \\ \hline
i9-9940X      & 14                                  & 1.2                                                                                    & .243                                                                            & 13.3                                                                                & .318                                                                       & 165                                                                              & 453                                                                                        & 603                                                                              & 1056                                                                      \\ \hline
i7-4790K      & 7                                   & 2                                                                                      & .426                                                                            & 4.46                                                                                & .65                                                                        & 88                                                                               & 453                                                                                        & 285                                                                              & 738                                                                       \\ \hline
Jetson Xavier & 8                                   &                                                                                        & .586                                                                            & 3.25                                                                                & .894                                                                       & 30                                                                               & 280                                                                                        & 80                                                                               & 360                                                                       \\ \hline
Jetson Tx2    & 6                                   &                                                                                        & .717                                                                            & 2.49                                                                                & 1.119                                                                      & 15                                                                               & 85                                                                                         & 59                                                                               & 144                                                                       \\ \hline
\end{tabular}
}
\vspace{2pt}

\label{compute_platform_data}
\end{table*}
%\renewcommand{\arraystretch}{1}

Throughout this section, we use these four platforms to study the impact paths that originate with mass.
Our studies model a mission where the drone is required to traverse a 
\red{500} meter paths to deliver a package. Sensory to actuation latency and throughput values are collected by running the a simplified package delivery application as a micro benchmark for 30 times
on each platform \footnote{our Benchmarks are extensively discussed in section~\ref{sec:mavbench}}. Mission time is calculated using the velocity and the path length while the power and energy
are calculated using our experimentally verified models provided in sections ~\ref{sec:energy} and ~\ref{sec:impact_through_power}. 
Finally, maximum to average velocity models are extracted from the extensive experimentation illustrated in section ~\ref{sec:operating-spoints}. 
To examine the impact of compute mass on our metrics in isolation, we have zeroed out latency and throughput
values to cut out their effect. However, note that in section~\ref{sec:impact_holistic}, 
we bring back these values and holistically look at all impact paths all at once.


\begin{figure}[t]
\includegraphics[width=.3\columnwidth]{figs/quad_forces.pdf}
\caption{Forces acting on a quad.}
\label{fig:quad_forces}
\end{figure}

\subsection{Impact on Mission Time}
\textit{\;\;\;\;Impact Path: Compute Subsystem -> Mass-> Acceleration-> Velocity-> Mission Time}
%return float(math.sqrt(maximum_thrust**2 - hover_thrust**2))/self.total_mass

As shown in figure ~\ref{fig:quad_forces}, two forces enable the drone's movements: ``lift'' and ``thrust''.
Lift is the upward force that fights gravity to keep the drone
in the air. A heaver drone needs to generate more lift.
Thrust is the forward force that fights air drag to push the drone forward. A faster drone needs to generate more thrust.
Given the limited amount of force that the motor-propeller combination can generate and distribute among lift and thrust,
adding more mass to the drone demands a higher portion of the generated force to be dedicated to lift (to keep the drone in the air). This, in turn,
takes away from its thrust leading to lower acceleration and velocity and finally longer mission time and energy. 
Equation ~\ref{eq:mass_acceleration} captures the relationship between mass and acceleration where g denotes the gravity
constant. 
\begin{equation}
\label{eq:mass_acceleration}
    a_{max} = \frac{~\sqrt[]{(Maximum\;thrust)^2 - (drone\;mass*g)^2}}{g}
\end{equation}
\setlength{\belowcaptionskip}{-1ex}
Using this equation, we can illustrate the impact of compute's added mass on velocity and acceleration 
for our DJI platform that can be equipped with any of the platforms provided in table ~\ref{compute_platform_data}.
As is seen in Figure ~\ref{fig:vel_acc_mass_impact}, a
\red{blahX} and \red{blahX} reduction in velocity and acceleration can be experienced between intel i9 and tx2. 
A heaver drone results in a longer mission time  (\red{blahX}) as shown in figure ~\ref{fig:comp_mt_mass_impact}. 
Lighter weight solution, in turn lower TDP designs are required to battle this increase.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}



\subsection{Impact on Quad's Power}
    \textit{\;\;\;\;Impact Paths:}
    
        \textit{\;\;\;\;\;\;\;Compute Subsystem -> Mass -> Acceleration -> Velocity -> Power} 
    
        \textit{\;\;\;\;\;\;\;Compute Subsystem -> Mass -> Acceleration -> Power}
    
        \textit{\;\;\;\;\;\;\;Compute Subsystem -> Mass -> Power}

    

        
    Equation~\ref{eq:DJI_power}, shows the mechanical power model used for our quad. As seen, mass, acceleration, and velocity determine the motor-propeller power consumption.
    As shown in the previous section, since, mass impacts velocity and acceleration, it both directly and indirectly, impacts power. Figure \ref{fig:comp_power_energy_mass_impact} shows 
    the combination of all these impact paths for our drone as the mass increases for our four systems mentioned above.
    A mass increase of \red{blah}\% results in a \red{blah}\% increase in power.
\begin{equation}
    \begin{aligned}
    P = \begin{bmatrix}
            -1.526 \\
            3.934 \\
            0.968
        \end{bmatrix}^{T}
        \begin{bmatrix}
            \norm{\vec{v}_{xy}} \\
            \norm{\vec{a}_{xy}} \\
            \norm{\vec{v}_{xy}}\norm{\vec{a}_{xy}}
        \end{bmatrix}
        +
        \begin{bmatrix}
            18.125 \\
            96.613 \\
            -1.085
        \end{bmatrix}^{T}
        \begin{bmatrix}
            \norm{\vec{v}_{z}} \\
            \norm{\vec{a}_{z}} \\
            \norm{\vec{v}_{z}}\norm{\vec{a}_{z}}
        \end{bmatrix}
        \\
        +
        \begin{bmatrix}
            .22\\
            1.332\\
            433.9
        \end{bmatrix}^{T}
        \begin{bmatrix}
            m \\
            \vec{v}_{xy} \cdot \vec{w}_{xy} \\
            1
        \end{bmatrix}
    \end{aligned}
    \label{eq:DJI_power}
    \end{equation}


\begin{figure}[t!]
\centering
     \begin{subfigure}{.3\linewidth}
   \includegraphics[width=\linewidth]{figs/mass_impact/mass_acc_vel.png}
   \caption{mass impact on velocity and acceleration}
   \label{fig:vel_acc_mass_impact}
    \end{subfigure} 
    \begin{subfigure}{.3\linewidth}
   \includegraphics[width=\linewidth]{figs/mass_impact/mass_mission_time.png}
    \caption{mass impact on mission time}
    \label{fig:comp_mt_mass_impact}
    \end{subfigure}
    \begin{subfigure}{.3\linewidth}
      \includegraphics[width=\linewidth]{figs/mass_impact/mass_power_energy.png}
   \caption{mass impact on energy and power}
    \label{fig:comp_power_energy_mass_impact}
    \end{subfigure}
   \caption{mass impact}
      \label{fig:comp_stop_distance}
\end{figure}


\subsection{Impact on Mission Energy}

\textit{\;\;\;\;Impact Path: Compute Subsystem -> Mass-> Acceleration-> Velocity -> Mission Time-> Mission Energy}

By increasing both the mission time and power, compute's
mass increases the overall systems' energy consumption. Figure \ref{fig:comp_power_energy_mass_impact} shows the relationship between 
different compute platforms and mission energy. An increase of \red{blah}\% is observed between the most and least compute capable system.
This increase demands designs with lower TDP, and hence lighter weight.


\begin{comment}
\begin{comment}
    # impact paths (vectors) 
    #-- missiontime //possibly use the same graph for the following
    compute->mass->acceleration->velocity->missiontime (through theory(finding max acceleration), and models for v max and v average)
    
    #-- power //possibly use the same graph for the following
    compute->mass->acceleration->velocity->power (through our models)
    compute->mass->power (through our power models)
    compute->mass->acceleration->power (through power models)
    
    #-- energy 
    compute->mass->acceleration->velocity->missiontime->missionenergy
\end{comement}

\blueDebug{section summary: explain different ways in which compute through math impacts 
                    mission time and energy.
           section flow: 
                 - name the impact paths.
                 - impact paths contributing to mission time //subsection
                    - graph quantifying magnitude and direction each impact path
                 - impact paths contributing to mission energy //subsection
                    - graph quantifying magnitude and direction each impact path
          }
\end{comment}


==> tex/role_of_comp_on_mission_energy.tex <==
\section{Compute Impact on Mission Energy}
\label{sec:comp_mission_energy}
Compute can impact mission energy through its performance, added power and mass.
We dive deep into such impacts and study each impact cluster separately to isolate their effect so that we gain better insights into their inner working. First, we explain the impact paths in the power cluster (Figure~\ref{fig:CIG_power_paths}, red-color/fine-grained-dashed paths). These are the paths originate with compute power. 
Then,
we explain performance cluster impacts paths (Figure~\ref{fig:CIG_performance_paths}, blue-color/coarse-grained-dashed paths). These  paths originate with compute performance quantities such as
sensing-to-actuation latency and throughput. Finally, we discuss the effect of mass cluster impact paths (Figure~\ref{fig:CIG_mass_paths}, green-color/double-sided paths). These paths originate with compute mass.



\subsection{Compute Power Impact on Mission Energy}
\label{sec:comp_power_impact_on_mission_energy}
Compute impacts MAV's overall energy consumption through its power consumption (power cluster shown in Figure~\ref{fig:CIG_power_paths} with red-color/fine-grained paths). The more the power consumption associated with the compute platform, the more the overall MAV's energy consumption.

To study this impact path, we present the power breakdown of a commonly used off the shelf drone, the \solo~\cite{solo3DR}. We use an Eagle~Tree Systems
eLogger~V4~\cite{eLoggerV4} setup to measure power consumption (Figures ~\ref{fig:elogger_placement} and ~\ref{fig:elogger_outside}).
eLogger allows us to collect power consumption data at 50~Hz during flight. We command the drone to fly for \SI{50}{\second} and pull the data off of the power meter after the drone lands. Note that during this section, we isolate the impact of the compute power. Later on, we examine the power and performance impact together on mission metrics in Section~\ref{sec:impact_holistic}.
% impact, we
% measure the rotor's power with 0g compute payload although section~\ref{sec:impact_holistic}
% brings back the load for more holistically examination.



% The wattmeter gave us the total power consumed by the drone, without a deeper breakdown. To estimate the portion of the instantaneous power that would typically be consumed by a MAV's processor, we subtracted the idle power consumption of the \solo's default onboard computer and added to it the power consumed by the TX2 during typical workloads.

\begin{figure}[!t]
\begin{subfigure}{.4\linewidth}
\centering
    \includegraphics[trim=0 2cm 0 0, clip, height=.8\columnwidth]{figs/elogger_close_view.pdf}
    %\vspace{10pt}
     %\vspace*{-18pt}
    \caption{eLogger inside view.}
    \label{fig:elogger_placement}
\end{subfigure}%
%\hfill
\begin{subfigure}{.4\linewidth}
%\vspace{10pt}
\centering
    \includegraphics[trim=0 2cm 0 0, clip, ,height=.8\columnwidth]{figs/elogger_full_view.pdf}
    \caption{eLogger outside view.}
    \label{fig:elogger_outside}
    \end{subfigure}    
    \caption{Power collection. Drone is instrumented with eLogger and data is collected during flight.}
\label{fig:elogger}
\end{figure}

\begin{figure}
\begin{subfigure}[!t]{.4\linewidth}
\vspace{5pt}
\centering
    \includegraphics[trim=0 0 0 0, clip, width=\columnwidth]{figs/power_break_down}
     \vspace{18pt}
    \caption{Measured power breakdown.}
    \label{fig:power_break_down}
\end{subfigure}%
%\hspace{10pt}
\begin{subfigure}[!t]{.52\linewidth}
   \vspace{2pt}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=\columnwidth]{figs/drone-power-time-series}
    \caption{Power during flight at 5 and 10~m/s.}
    \label{fig:drone-power-time-series}
\end{subfigure}
\caption{Power profiling and breakdown. Compute generally makes up a small portion of the MAV's overall power pie. Velocity has a minor impact on power consumption for our MAV.}
\end{figure}

A drone with higher compute capability generally spends a higher budget of its total power on the compute subsystem in order to improve its performance. \Fig{fig:power_break_down} demonstrates this point by showing the power consumption of both the compute and the rotors for the
four platforms described earlier in Table~\ref{compute_platform_data}. Depending on the type of onboard compute system (i.e., TX2, Xavier, i7 or i9), the compute subsystem will directly consume 3\% to 24\% of the total system power. Hence, system designers must pay attention to such breakdowns since power-efficient designs will have a more significant impact on systems in which compute currently uses a more substantial proportion of total system power. 

%the higher portion of the pie is consumed by the compute, the higher its impact and demand for power efficient designs. 



\begin{figure}[t!]
    %\vspace{-3pt}
    \centering
    \begin{subfigure}[t!]{.18\linewidth}
    \centering
    \includegraphics[width=\linewidth] {figs/scanning_energy_operating_point}
    \label{fig:benchmarks:OPA:scanning:energy}
    \vspace*{-12pt}
    \caption{\scriptsize Scanning.}
    \end{subfigure}
    \begin{subfigure}[t!]{.18\linewidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/pd_energy_operating_point}
     \label{fig:benchmarks:OPA:pd:energy}
     \vspace{-12pt}
       \caption{\scriptsize Package Delivery.}
    \end{subfigure}%
    \begin{subfigure}[t!]{.18\linewidth}
    \includegraphics[width=\linewidth] {figs/mapping_energy_operating_point}
     \label{fig:benchmarks:OPA:mapping:energy}
       \vspace{-12pt}
        \caption{\scriptsize 3D Mapping.}
    \end{subfigure}%
    \begin{subfigure}[t!]{.18\linewidth}
    \centering
    \includegraphics[width=\linewidth] {figs/SAR_energy_operating_point}
     \label{fig:benchmarks:OPA:sar:energy}
      \vspace{-12pt}
      \caption{\scriptsize Search \& Rescue.}
    \end{subfigure}%
    \begin{subfigure}[t!]{.18\columnwidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/aerial_photography_energy_operating_point}
     \label{fig:benchmarks:OPA:ap:energy}
     \vspace{-12pt}
     \caption{\scriptsize Aer Photography.}
    \end{subfigure}
    \caption{Core/frequency sensitivity analysis of mission energy for various benchmarks.}
    \label{fig:benchmarks_mission_energy}
\end{figure}

\subsection{Compute Performance Impact on Mission Energy}
\label{sec:comp_perf_impact_on_mission_energy}

%\textit{\;\;\;\;Impact Path: Compute Subsystem -> latency -> Velocity -> Power -> Mission Energy}
%\textit{Impact Path: Compute Subsystem -> throughput -> Velocity -> Power -> Mission Energy}
Compute impacts mission energy through cyber quantities such as sensing-to-actuation latency, throughput, and etc, in other words, through the performance cluster (Figure~\ref{fig:CIG_performance_paths}, blue-color/coarse-grain-dashed paths). All such impacts start with cyber quantities
and then go through velocity, a physical quantity, to ultimately influence mission energy. 

Compute performance impacts a MAV's velocity (\Sec{sec:comp_perf_impact_on_mission_time}), which then impacts power consumption and ultimately impacts the MAVs total energy consumption.  To measure this impact, we used our eLogger~V4 setup.
As \Fig{fig:drone-power-time-series} shows, power variation as a result of velocity, be it 5~m/s (top) or 10~m/s (bottom), is rather minor for our MAV. This is because the majority of the rotor's power is spent keeping the drone airborne ($T_y$ from Figure~\ref{fig:quad_FBD_2D}), and a 
%This is because, majority of the rotor powers are spent to keep the drone in the air (hovering),
%but once in the air, 
relatively small amount is used for moving forward during the flight ($T_x$ from Figure~\ref{fig:quad_FBD_2D}) for our allowed velocities.

%\textit{\;\;\;\;Impact Path: Compute Subsystem -> Latency -> Velocity -> Mission Time -> Mission Energy}
%\textit{Impact Path: Compute Subsystem -> Throughput -> Velocity -> Mission Time -> Mission Energy}
In addition to the impact on energy through power, velocity can significantly reduce the total mission energy by reducing the mission time.
This is because as was shown in the previous section, rotors consume a bigger portion of the power consumption pie. Hence, by reducing the mission time, rotors spend less time in the air and hence consume less power and energy. 
%This is similar to techniques studied in the system and architecture community to reduce overall energy by reducing the run time (\red{have some papers here}).

Using the models provided in Section~\ref{sec:energy}, we profiled the mission time and the energy associated with the micro and end-to-end benchmarks discussed in the previous section, a SLAM microbenchmark and the MAVBench end-to-end benchmark suite. For the SLAM microbenchmark, as
shown in the previous section in Figure~\ref{fig:slam-velocity-energy}, a higher compute capability increases velocity (bottom graph) and lowers the total system energy (top graph). We see that by increasing processing speed from 1 FPS to 8 FPS, i.e., a 8X speed up, we are able to reduce the drone's energy consumption from \SI{76.9}{\kilo\joule} to \SI{21.1}{\kilo\joule}, i.e., close to 4X reduction.
For our end-to-end benchmarks, by conducting a core-frequency sensitivity analysis,
we show that more compute reduces the mission energy by as much as 5.8X (In 3D Mapping energy consumption is reduced from \SI{2213}{\kilo \joule} to \SI{283}{\kilo\joule}). These results are shown as a heatmap (Figure~\ref{fig:benchmarks_mission_energy}). Note that energy values closely follows the mission time trend discussed in Section~\ref{sec:comp_mission_time}, since a faster mission time lowers mission energy. 
%\red{I think somewhere in this paragraph you need to connect mission time to energy by noting that the majority of the power is in the rotors and you showed that rotor power is constant for flight and hovering --- so longer flight = more energy}

\subsection{Compute Mass Impact on Mission Energy}
\label{sec:comp_mass_impact_on_mission_energy}
%\textit{\;\;\;\;Impact Path: Compute Subsystem -> Mass-> Acceleration-> Velocity -> Mission Time-> Mission Energy}
% \textit{\;\;\;\;\;\;\;Compute Subsystem -> Mass -> Acceleration -> Velocity -> Power} 
%\textit{\;\;\;\;\;\;\;Compute Subsystem -> Mass -> Acceleration -> Power}
%\textit{\;\;\;\;\;\;\;Compute Subsystem -> Mass -> Power}
Compute mass both directly and indirectly impacts rotor power consumption (mass cluster shown in Figure~\ref{fig:CIG_mass_paths} with green-color/double-sided paths). This is because mass itself, as shown in Section~\ref{sec:comp_mass_impact_on_mission_time}, impacts acceleration and velocity, and all three impact power. This can be seen in the mechanical power model provided in Section~\ref{sec:energy}. Equation~\ref{eq:DJI_power} shows this model specifically for our DJI quad. 
 \begin{equation}
    \begin{aligned}
    P = \begin{bmatrix}
            -1.526 \\
            3.934 \\
            0.968
        \end{bmatrix}^{T}
        \begin{bmatrix}
            \norm{\vec{v}_{xy}} \\
            \norm{\vec{a}_{xy}} \\
            \norm{\vec{v}_{xy}}\norm{\vec{a}_{xy}}
        \end{bmatrix}
        +
        \begin{bmatrix}
            18.125 \\
            96.613 \\
            -1.085
        \end{bmatrix}^{T}
        \begin{bmatrix}
            \norm{\vec{v}_{z}} \\
            \norm{\vec{a}_{z}} \\
            \norm{\vec{v}_{z}}\norm{\vec{a}_{z}}
        \end{bmatrix}
        +
        \begin{bmatrix}
            .22\\
            1.332\\
            433.9
        \end{bmatrix}^{T}
        \begin{bmatrix}
            m \\
            \vec{v}_{xy} \cdot \vec{w}_{xy} \\
            1
        \end{bmatrix}
    \end{aligned}
    \label{eq:DJI_power}
    \end{equation}
 
As mass increases, so does power. Figure \ref{fig:mass_power} shows this effect for the DJI quadrotor across different compute platforms. An increase in the compute mass from \SI{144}{\g}, associated with the lightest MAV with a TX2, to \SI{1109}{\g}, associated with the heaviest MAV with an i9, i.e., a 7.9X increase, causes the total MAV mass to exacerbate from \SI{2544}{\g} to \SI{3509}{\g}, i.e., a 1.4X increase. This then heightens the power consumption from \SI{527}{\watt} to \SI{687}{\watt}, i.e., 20\% increase in total power (for SDR of 4). Note that the slow down ratio has a minor impact on power as all the lines are very close to one another. This is because the velocity has a minor impact on power as discussed in Section~\ref{sec:comp_perf_impact_on_mission_energy}.  
\begin{figure}[t!]
\centering
     \begin{subfigure}{0.4\linewidth}
   \includegraphics[width=.9\linewidth]{figs/mass_impact/mass_power.pdf}
   \vspace{-20pt}
   \caption{Impact on power.}
   \label{fig:mass_power}
    \end{subfigure} 
    \begin{subfigure}{0.4\linewidth}
   \includegraphics[width=.9\linewidth]{figs/mass_impact/mass_energy.pdf}
     %\vspace{-20pt}
    \vspace{-20pt}
    \caption{Impact on energy.}
    \label{fig:mass_energy}
    \end{subfigure}
   \caption{Impact of compute mass, a physical quantity, on power and energy.}
      \label{fig:comp_stop_distance}
\end{figure}

Compute mass impacts energy consumption by impacting both power and mission time. An increase in compute mass exacerbates the energy consumption by increasing power as was detailed in the previous paragraph. In addition, an increase in mass exacerbates energy consumption by increasing the mission time. This is due the reduction in velocity and acceleration that was discussed in Section~\ref{sec:comp_mass_impact_on_mission_time}. \Fig{fig:mass_energy} shows an overall system energy consumption increase from \SI{180}{\kilo\joule} to \SI{490}{\kilo\joule}, i.e. a 2.7X increase, between the lightest (TX2) and the heaviest (i9) platforms (for SDR of 4). Note that like our observation for mission time, this impact grows with the environment's difficulty level, i.e., the environment's congestion. Therefore, as the environment becomes harder to navigate, the MAV requires more power-efficient designs.


==> tex/role_of_comp_on_mission_power.tex <==
\section{Compute's Power Impact}
\label{sec:impact_through_power}

\subsection{Impact on Mission Energy}
\label{sec:impact_2}
\textit{\;\;\;\;Impact Path: Compute Subsystem -> Latency -> Velocity -> Mission Time -> Mission Energy}

\textit{Impact Path: Compute Subsystem -> Throughput -> Velocity -> Mission Time -> Mission Energy}

The compute subsystem can also have a significant role in reducing total MAV's energy consumption. 
At the high-level, by reducing the mission time, we can reduce the total system's energy by flying the
quad for a shorter period of time. This is similar to techniques studied in the system and architecture community to reduce overall energy by cutting down on the run time (\red{have some papers here}).
Using the models provided in section ~\ref{sec:energy}, we profiled the mission time and the energy associated with the aforementioned micro-benchmark. 
As the bottom plot in \Fig{fig:slam-velocity-energy} shows, a higher compute capability increase velocity (bottom graph) which results in total system energy (top graph). By increasing processing speed by 5X, we were able to reduce the drone's energy consumption by close to 4X.

\begin{figure}[!t]
    \centering
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=.5\columnwidth]{figs/drone-power-time-series}
    \caption{Total measured power consumption while the drone is "Flying" at two different steady-state velocities. Minor change in values are observed}
    \label{fig:drone-power-time-series}
\end{figure}


\subsection{Impact on Quad's Power}
\label{sec:impact_3}

\textit{\;\;\;\;Impact Path: Compute Subsystem -> latency -> Velocity -> Power -> Mission Energy}

\textit{Impact Path: Compute Subsystem -> throughput -> Velocity -> Power -> Mission Energy}

The velocity with which the drone flies with impacts the amount of power and hence energy it consumes. To measure the variation in power 
under different velocities (within the velocity bounds that
compute allows), we attached a watt meter known as Eagle~Tree Systems eLogger~V4~\cite{eLoggerV4} to the \solo~\cite{solo3DR}, a popular off-the-shelf MAV. eLogger allows us to collect battery data during flight time at 50~Hz. We command the drone to fly for fifty seconds and pull the data off of the watt meter after the drone lands.
As \Fig{fig:drone-power-time-series} shows, this variation is minor. 
This is because, majority of the rotor powers are spent to keep the drone in the air (hovering),
but once in the air, relatively a small amount is used for moving forward. 


\textit{\;\;\;\;Impact Path: Compute Subsystem -> Power -> Mission Energy}

This section discusses the third cluster. These are the paths with which the 
compute impacts mission energy directory through compute subsystem's power.

%\subsection{Compute Power and Quad's Mission Energy Relationship}
To understand the impact of compute's power consumption on the entire system's power and energy, 
first, we present the power distribution associated with \solo~\cite{solo3DR} using our Eagle~Tree Systems
eLogger~V4~\cite{eLoggerV4} setup. Note that to isolate the impact of compute power and cut out the mass impact, we
measure the rotor's power with 0g load. However, section~\ref{sec:impact_holistic}
brings back the load and holistically examines at all impact paths at once.

\begin{figure}[!t]
\centering
       \vspace{-50pt}
    \includegraphics[trim=0 0 0 0, clip, width=\columnwidth]{figs/power_break_down}
     \vspace{-90pt}
    \caption{Measured power breakdown.}
   
    \label{fig:power_break_down}
\end{figure}
% The wattmeter gave us the total power consumed by the drone, without a deeper breakdown. To estimate the portion of the instantaneous power that would typically be consumed by a MAV's processor, we subtracted the idle power consumption of the \solo's default onboard computer and added to it the power consumed by the TX2 during typical workloads.

\Fig{fig:power_break_down} shows the power consumption of both the compute and the rotors for the
four platforms mentioned above. As illustrated, depending on the on board's compute capability, 5\% to 38\% of the system power will be directly consumed by the compute subsystem power. \red{I wonder if there is a take away here, besides reporting number}






\begin{figure}[t!]
    \centering
    \begin{subfigure}[t!]{.19\linewidth}
    \centering
    \includegraphics[width=\linewidth] {figs/scanning_energy_operating_point}
    \label{fig:benchmarks:OPA:scanning:energy}
    \caption{Scanning Energy.}
    \end{subfigure}
    \begin{subfigure}[t!]{.19\linewidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/pd_energy_operating_point}
     \label{fig:benchmarks:OPA:pd:energy}
       \caption{Package Delivery Energy.}
    \end{subfigure}%
    \begin{subfigure}[t!]{.19\linewidth}
    \includegraphics[width=\linewidth] {figs/mapping_energy_operating_point}
     \label{fig:benchmarks:OPA:mapping:energy}
        \caption{Mapping Energy.}
    \end{subfigure}%
    \begin{subfigure}[t!]{.19\linewidth}
    \centering
    \includegraphics[width=\linewidth] {figs/SAR_energy_operating_point}
     \label{fig:benchmarks:OPA:sar:energy}
      \caption{Search and Rescue Energy.}
    \end{subfigure}%
    \begin{subfigure}[t!]{.19\columnwidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/aerial_photography_energy_operating_point}
     \label{fig:benchmarks:OPA:ap:energy}
     \caption{Aerial Photography Energy.}
    \end{subfigure}
\end{figure}



%the majority of the power consumption is 
%dedicated to rotors (locomotion) and the compute only occupies a relatively
%small portion of the entire pie and its role seemingly trivial. 
%This pie for four different platforms discussed in the previous section are shown.

%Although small in quantity, compute can have a grand effect on the system's power. This is because by reducing the mission time (as explained in the previous section), more compute power can, in fact, reduce the bigger portion of the pie, namely rotors energy consumption (due to a shorter flight). Note that although more compute can lead to more energy consumption of the compute subsystem, the reduction in rotor's energy can easily outweigh such an increase.  




% \setlength{\belowcaptionskip}{-2ex}




==> tex/role_of_comp_on_mission_time.tex <==
\section{compute impact on mission time}
\label{sec:comp_mission_time}
In this section, we take a deep dive exploring how compute impacts mission time through a combination of analytical models, simulation, and micro and end-to-end benchmarking.
Briefly, compute impacts mission time through both cyber and physical quantities. It impacts cyber quantities such as sensing-to-actuation latency, throughput and ultimately response time, and also impacts
physical quantities such as drone's mass, velocity, and acceleration. Such impacts percolate down to the bottom of the \csig influencing mission metrics such as mission time. 
This section studies each impact cluster separately to isolate their effect so that we gain better insights into their inner working. First, we explain the impact paths in the performance cluster (Figure~\ref{fig:CIG_performance_paths}, blue-color/coarse-grained-dashed paths), and
then, we explain the paths in the mass cluster (Figure~\ref{fig:CIG_mass_paths}, green-color/double-sided paths).



\subsection{Compute Performance Impact on Mission Time}
\label{sec:comp_perf_impact_on_mission_time}
Compute reduces mission time through performance cluster by impacting physical quantities, such as the drone's average velocity (performance cluster shown in Figure~\ref{fig:CIG_performance_paths} with the  blue-color/coarse-grained-dashed paths). A MAV's average velocity is a function of its response time, i.e., how quickly it can respond to a new event, such as the emergence of an obstacle in its environment. By improving response time, compute allows the drone to fly faster while being safe (i.e., with no collisions), and flying faster in return reduces the mission time. To achieve a high average velocity throughout the mission, the drone needs to be capable of reaching a high velocity (maximum velocity) and also quickly arrive at it (high acceleration). We discuss compute-maximum velocity relationship and leave the compute-acceleration discussion to the next section.   

 \begin{figure}[t!]
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=.4\columnwidth]{figs/fig_13}
    \caption{Theoretical max velocity and response time relationship.}
    \label{fig:process-time-velocity}
    \end{figure}



%We identify the reduction in hover time and the increase in maximum allowed velocity as two major ways with which more compute can contribute to a higher average velocity. 
%In this section, we show how compute's impact on perception, planning and control effects hover time, maximum velocity, and consequently average
%velocity, mission time and mission energy.

%sensory information it has collected through the 3 stage
%Compute can play an essential role in reducing the drone's mission time by increasing the mission's average velocity. To attain a high average velocity the drone needs to maintain a high velocity throughout its mission. To do this the drone needs to 1.have a high maximum velocity to traverse the trajectory with 2.maintain this high velocity and reduce deviation from it. 

\paragraph{Improving Maximum Velocity By \textit{Reducing Response Time:}}
%A safe flight with higher velocity requires more compute capability to shorten the response time. %Simply put, to guarantee collision avoidance a drone's maximum velocity needs to be bounded based on a cyber quantity called response time. 
%This is the time drone takes 
%to respond to an event emerging (e.g. emergence of an obstacle in drone's field of view) 
%in its surrounding environment.
%\emph{A higher velocity requires more compute capability to
%shorten such response time}.
Drone's maximum velocity is not only mechanically bounded but also computationally bounded. Equation~\ref{eq:runtime-compute-bound} shows this where response time, a cyber quantity determined by compute, impacts velocity, a physical quantity. The variables $\delta{t}_{response}$, $d$, $a_{max}$ and $v_{max}$ denote response time, distance from obstacle,
maximum acceleration limit of the drone and maximum allowed velocity, respectively. Applying Equation~\ref{eq:runtime-compute-bound} for out simulated DJI Matric 100 drone,  Figure~\ref{fig:process-time-velocity} shows that, in theory, the drone's maximum velocity takes a value between 1.57 m/s to 8.83 m/s given a response time ranging from 0 to 4~seconds.

\begin{equation}
\label{eq:runtime-compute-bound}
\boxed{
v_{max} = a_{max}(~\sqrt[]{\delta{t_{response}}^2 + 2\frac{d}{a_{max}}} - \delta{t_{response}})}
\end{equation}

% Equation~\ref{eq:runtime-compute-bound} captures the impact of a cyber quantity on a physical quantity

To help explain the relationship between compute and velocity, we step through a typical obstacle avoidance task whose maximum velocity obeys this equation. At a high level, a MAV periodically takes snapshots of its environment and then spends some processing time responding to the emerging obstacles in its path ($\delta{t}_{response}$). However, if the motion planner fails to find a trajectory that circumvents the obstacle, the drone needs to decelerate immediately ($a_{max}$) to avoid running into the obstacle. In the worst case, the drone needs to be able to decelerate from its maximum speed ($v_{max}$).

Figure~\ref{fig:vmax_gen} shows the progression of this task for two snapshots, $snap_{0}$ and $snap_{1}$. We call the rate with which these snapshots occur sensing-to-actuation throughput (denoted by $\delta_{SA\_throughput}$). Between the two snapshots, i.e, inverse of the throughput, the drone is blind (Equation~\ref{eq:blind}). This is because \textbf{no} new snapshot are taken, and hence the drone is unaware of any changes in the environment during this period. In the
worst-case scenario, an obstacle (O) can be hiding within the blind space caused by $\delta{t}_{blind}$. This reduces the 
distance between the drone and the obstacle by 
$v_{max}$*$\delta{t}_{blind}$ (Equation~\ref{eq:distance_to_obs_after_blind}). After this blind period, at point $snap_{1}$, the second snapshot is taken and the drone spends sensing-to-actuation latency ($\delta{t}_{SA\_latency}$), 
to perceive ($\delta{t}_{pr}$), plan ($\delta{t}_{pl}$) and control ($\delta{t}_{c}$), traversing the PPC pipeline, to formulate and follow a trajectory to circumvent the obstacle (Equation \ref{eq:reaction_latency}).
Equation~\ref{eq:distance_to_obs_after_reaction_formulation} shows the distance between the drone and the obstacle
after this traversal.

 \begin{figure}[t!]
\centering
    \begin{subfigure}{\columnwidth}
    \centering
   \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/vmax_gen.pdf}
    %\caption{Measured max velocity.}
    
    \end{subfigure}
%\vspace{5pt}
\caption{Obstacle avoidance in action, a bird's-eye view. Note the progression in time as a result of cyber quantities such as sensing-to-actuation latency, and the progression in space as the result of physical quantities such as $v$.}
\label{fig:vmax_gen}
\end{figure}



\begin{equation}
\label{eq:blind}
\delta{t}_{blind} = \frac{1}{\delta_{SA\_throughput}}
\end{equation}
 

\begin{equation}
\begin{aligned}
\label{eq:distance_to_obs_after_blind}
Distance\;to\;Obstacle\;After\;Blind\;Time &=  \left d - v_{max}*\delta{t}_{blind} \right \\ &= d - v_{max}*\frac{1}{\delta_{SA\_throughput}} \right
\end{aligned}
\end{equation}




\begin{equation}
\label{eq:reaction_latency}
\delta{t}_{SA\_latency} = \delta{t}_{pr} + \delta{t}_{pl} + \delta{t}_{c}
\end{equation}

\begin{equation}
    \label{eq:distance_to_obs_after_reaction_formulation}
\begin{aligned}
Distance\;to\;Obstacle\;After\;PPC\;Traversal  =  d - v_{max}*\frac{1}{\delta_{SA\_throughput}} - v_{max}*\delta{t}_{SA\_latency}
\end{aligned}
\end{equation}
 
At this point, if the drone fails to generate a plan, it must decelerate and ideally come to a halt before running into the obstacle in its current path. 
Equation \ref{eq:stop-distance} shows the distance that it takes for a moving body to come to a complete stop. Setting \ref{eq:distance_to_obs_after_reaction_formulation} and \ref{eq:stop-distance}
equal to one another and solving for $v$ results in Equation~\ref{eq:runtime-general}, the absolute maximum velocity with which the drone is allowed to fly and still be able to guarantee a collision-free mission. This equation shows the relationship between two cyber quantities, i.e.,
$\delta{t}_{SA\_latency}$ and
$\delta_{SA\_throughput}$, and a physical quantity, i.e., $v$.\footnote{If we pair this equation with Equation~\ref{eq:runtime-compute-bound}, we see that for a drone to be able to respond to an obstacle in the worst case scenario, it needs to spend a total of $\delta{t}_{SA\_latency}$ plus inverse of
$\delta_{SA\_throughput}$ which indeed is the response time (Equation~\ref{eq:response_time}) of the MAV to an emerging event (obstacle).}
%Note that since in the sequential design, throghput is simply inverse of latency, $v_{max}$ equation can be rewritten to to equation{eq:runtime-compute-seq}


\begin{equation}
\label{eq:stop-distance}
Stopping\;Distance= \frac{v^2}{2*a_{max}} 
\end{equation}

\begin{equation}
\label{eq:runtime-general}
\boxed{
v_{max} = a_{max}\left(~\sqrt[]{\left(\delta{t}_{SA\_latency} + \frac{1}{\delta_{SA\_throughput}}\right)^2 + 2\frac{d}{a_{max}}}
- \left(\delta{t}_{SA\_latency} + \frac{1}{\delta_{SA\_throughput}}\right)\right)}
\end{equation}

\begin{equation}
\label{eq:response_time}
\delta{t}_{response} = \delta{t}_{SA\_latency} + \delta_{SA\_throughput}
\end{equation}

\begin{figure}[t!]
\centering
    \begin{subfigure}{.49\columnwidth}
    \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/vmax_seq1.pdf}
    %\vspace{-10pt}
    \caption{Sequential paradigm.}
    \label{fig:vmax_seq}
    \end{subfigure}
    \begin{subfigure}{.49\columnwidth}
   \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/vmax_pipe.pdf}
    %\vspace{-10pt}
    \caption{Pipelined paradigm.}
    \label{fig:vmax_pipe}
    \end{subfigure}
       \caption{Obstacle avoidance with the PPC pipeline. Latency associated with each stage is denoted with $\delta$. Two different design paradigms are presented.}
      \label{fig:comp_stop_distance}
\end{figure}



Investigating how system design choices impact $\delta_{SA\_throughput}$ and  $\delta{t}_{SA\_latency}$ (and hence response time and velocity)
demands computer and system architects' attention. For example, consider the sequential versus a pipelined design paradigm.
In the sequential processing paradigm, while the drone is going through one iteration of the PPC pipeline, no new snapshots are taken (Figure~\ref{fig:vmax_seq}). This means that the
sensing-to-actuation throughput is the inverse of sensing-to-actuation latency (Equation~\ref{eq:reaction_throughput}).
\begin{equation}
\label{eq:reaction_throughput}
\delta_{SA\_throughput} = \frac{1}{\delta{t}_{SA\_latency}}
\end{equation} 
 
This implies that we can rewrite Equations
~\ref{eq:distance_to_obs_after_blind},~\ref{eq:distance_to_obs_after_reaction_formulation}, 
~\ref{eq:runtime-general} and
~\ref{eq:response_time} as such:

% sequential here
\begin{equation}
\label{eq:distance_to_obs_after_blind_seq}
Distance\;to\;Obstacle\;After\;Blind\;Time  = d - v_{max}*\delta{t}_{SA\_latency}
\end{equation}

\begin{equation}
    \label{eq:distance_to_obs_after_reaction_formulation_seq}
\begin{aligned}
Distance\;to\;Obstacle\;After\;SA\;Traversal  =  
d -  v_{max}*2*\delta{t}_{SA\_latency}
\end{aligned}
\end{equation}

\begin{equation}
\label{eq:response_time_seq}
\delta{t}_{response} = 2*\delta{t}_{SA\_latency}
\end{equation}

resulting in a $v_{max}$ of:
\begin{equation}
\label{eq:runtime-compute_seq}
\boxed{
v_{max} = a_{max}\left(~\sqrt[]{4*\delta{t}_{SA\_latency}^2 + 2\frac{d}{a_{max}}} - 2*\delta{t}_{SA\_latency}\right)}
\end{equation}
\setlength{\belowcaptionskip}{-1ex}

However, in a pipelined processing paradigm (Figure~\ref{fig:vmax_pipe}), perception, planning and control stages overlap with one another. Hence, it is possible for us to reduce the $\delta_{SA\_throughput}$ and thereby cut down $\delta{t}_{blind}$ to the minimum of latency of each stage (Equation~\ref{eq:throughput}). Note that in this design $\delta{t}_{SA\_latency}$ stays intact.
Using the pipeline approach, the velocity is calculated using Equation~\ref{eq:runtime-pipelined}. 

\begin{equation}
\label{eq:throughput}
\begin{aligned}
 \delta{t}_{blind} = \left  \frac{1}{\delta_{SA\_throughput}} = \frac{1}{Min(\frac{1}{\delta{t}_{pr}},\frac{1}{\delta{t}_{pl}}, \frac{1}{\delta{t}_{c}})} \right = 
 \left Max(\delta{t}_{pr},\delta{t}_{pl}, \delta{t}_{c}) \right
 \end{aligned}
\end{equation}

\setlength{\belowcaptionskip}{-1ex}

\begin{equation}
\label{eq:runtime-pipelined}
\boxed{
\begin{aligned}
v_{max} = a_{max}\left(& ~\sqrt[]{(\delta{t}_{SA\_latency} +  Max(\delta{t}_{pr}, \delta{t}_{pl}, \delta{t}_{c})^2 + 2\frac{d}{a_{max}}}  - \\ 
&(\delta{t}_{SA\_latency} +  Max(\delta{t}_{pr}, \delta{t}_{pl}, \delta{t}_{c}))\right)
\end{aligned}
}
\end{equation}

There is a tradeoff in opting between the sequential versus pipeline paradigms. However, the choice is not straightforward. Opting for one or the other requires a rigorous and thorough investigation by system designers. For example, simply pipelining the design does not necessarily improve the velocity. This is because the response time is equal to the addition of $\delta{t}_{SA\_latency}$ (see above) and inverse of $\delta_{SA\_throughput}$. Therefore, if the pipelined design increases $\delta{t}_{SA\_latency}$ (e.g., due to the communication overhead between parallel processes), the overall response time might increase. %We believe that investigations of this sort are necessary for optimal robot designs. Hence, we spend the rest of this section studying such examinations through micro and end-to-end benchmarking.

\begin{figure}[t!]
\centering
    \begin{subfigure}{.4\columnwidth}
    \centering
   \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/slam_fps_velocity_energy}
    %\caption{Measured max velocity.}
    
    \end{subfigure}
\caption{Relationship between SLAM throughput (FPS) and maximum velocity and energy of UAVs.}
\label{fig:slam-velocity-energy}
\end{figure}


\paragraph{Improving Max Velocity by \textit{Reducing Perception Latency:}} Another way to improve velocity is to reduce perception processing time. 
The faster a drone wants to fly, the faster it must process its sensory feed
to extract the MAV's and its environment's relevant states. In other words, \textit{faster flights require faster perception}. This can be seen with perception related compute intensive kernels such as
Simulateneous Localization and Mapping (SLAM)~\cite{SLAM_survey}. SLAM localizes a MAV by tracking sets of features in the environment. Since a faster flight results in more rapid changes in the MAV's environment, fast flight can be problematic for this kernel leading to catastrophic effects such as permanent loss or a flight time increase (for example by backtracking due to re-localization). Minimizing or avoiding localization-related failures is highly favorable, if not necessary.

To examine the relationship between the compute, maximum velocity and localization failure, we evaluated a micro-benchmark in which the drone was tasked to follow a predetermined circular path of the radius 25~meters. For the localization kernel, we used ORB-SLAM2~\cite{orbslam2} and to emulate different compute powers, we inserted a sleep into the kernel. We swept velocities and sleep times and bounded the failure rate to 20\%. As \Fig{fig:slam-velocity-energy} shows, increasing FPS values from 1 to 8, which is enabled by more
compute, allows for an increase in maximum velocity from \SI{1}{\meter/\second} to \SI{5}{\meter/\second} (for a bounded failure rate), which shows that the maximum velocity is affected by perception latency.

%\paragraph{Improving hover Time by  reducing Planning Latency:} Hover time and the average velocity have an inverse relationship; namely, the more drone spends time on hovering, the lower its average velocity. Similar to
%an idling CPU, a hovering drone is unfavorable since it is not working toward its mission, but yet wasting its limited energy. A hovering drone typically is waiting for its planning stage to make a
%decision (e.g., deciding on a path to follow). \emph{More compute power can help reduce hovering by reducing the planning's decision-making time, hence decreasing the negative effect hovering has on the average velocity.} 


%\setlength{\belowcaptionskip}{-4ex}

%\label{SOLO_power_breakdown}


%This means that at design time, careful analysis of the tradeoffs between throughput and latency needs to be accounted for.  

%\begin{figure}[h]
%\includegraphics[]{figs/blank.pdf}
%\caption{Measurement set up to collect power data for 3DR Solo.}
%\label{sec:powerbreakdown}
%\end{figure}
% \begin{comment}
% \paragraph{Maintaining Max Velocity}
% As was discussed before, to reduce the mission time, it's not enough to have a high bound on v ($v_{max}$), but we need to reach $v_{max}$ and maintain it during the flight. In other words, once $v_{max}$
% is reached, the drone should attempt at reducing deviation from it. This means that the trajectories of low curvature are desired.  \red {this is a point about acceleration. Not sure if I should bring.
% if we decide to bring it, then I need to add another picture and formula}
% \end{comment}

% \textbf{Core and Frequency Scaling:}
%\label{sec:operating-spoints}
Expanding on the microbenchmark insight from \Fig{fig:slam-velocity-energy}, 
we conducted a series of performance sensitivity analysis using processor core count and
frequency scaling.
We study the effect of compute on all of the MAVBench applications.
%TX2 has two sets of cores, namely a \textit{HMP Dual Denver cores} and a \textit{Quad ARM A57}. We turned off the Denver cores so that the indeterminism caused by process to core mapping variations across runs would not affect our results.
Average velocity and mission times of various operating points are profiled and presented as heat maps (Figures~\ref{fig:benchmarks_mission_velocity} and \ref{fig:benchmarks_mission_time}) for a DJI Matrice 100 drone. \emph{In general, compute can improve mission time by as much as 5X.} 

red\textit{Scanning:} In this application, we observe trivial differences for velocity and endurance across all three operating points (\Fig{fig:benchmarks:OPA:scanning:velocity}, \Fig{fig:benchmarks:OPA:scanning:time}) despite seeing a 3X boost in the motion planning kernel, i.e. lawn mower planning, which is its bottleneck (\Fig{fig:kernel-breakdown}). This is because, for this application, planning is only done once at the beginning of the mission and amortized over the rest of the mission time. For example, the overhead of planning for a five-minute flight is less than .001\%.

\textit{Package Delivery}:  As compute scales with the number of cores and/or frequency values, we observe a reduction of up to 84\% for the mission time (\Fig{fig:benchmarks:OPA:pd:time}). With frequency scaling, this improvement is due to the speed up of the sequential bottlenecks, i.e., motion planning and OctoMap generation kernel. On the other hand, there does not seem to be a clear trend with regard to core scaling, specifically between three and four cores. We conducted investigations and determined that the anomalies are caused by the non-real-time aspects of ROS, AirSim, and the TCP/IP protocol used for the communication between the companion computer and the host. Overall, we achieve up to 2.9X improvement in OctoMap generation which leads to maximum velocity improvement. It is important to note that although we also gain up to 9.2X improvements for the motion planning kernel, the low number of re-plannings and its short computation time relative to the entire mission time render its impact trivial. Overall the aforementioned improvements translate to up to 4.8X improvement in the average velocity. Therefore, mission time and MAV's total energy consumption are reduced.  
{ 
    \begin{figure}[t!] \centering \begin{subfigure}[t!]{.18\columnwidth} \centering \includegraphics[width=\columnwidth]{figs/scanning_velocity_operating_point} 
    %\vspace{-20pt}
    \caption{\scriptsize Scanning.}
    \label{fig:benchmarks:OPA:scanning:velocity} \end{subfigure}%
    \begin{subfigure}[t!]{.18\columnwidth} \centering \includegraphics[width=\columnwidth]{figs/pd_velocity_operating_point}
    %\vspace{-20pt}
\caption{\scriptsize Package Delivery.} \label{fig:benchmarks:OPA:pd:velocity} \end{subfigure}%
    \begin{subfigure}[t!]{.18\columnwidth} \centering
\includegraphics[width=\columnwidth]{figs/mapping_velocity_operating_point}
%\vspace{-20pt}
\caption{\scriptsize 3D Mapping.} \label{fig:benchmarks:OPA:mapping:velocity} \end{subfigure} %  
\begin{subfigure}[t!]{.18\columnwidth}
\centering \includegraphics[width=\columnwidth]{figs/SAR_velocity_operating_point} 
%\vspace{-20pt}
\caption{\scriptsize Search \& Rescue.} \label{fig:benchmarks:OPA:sar:velocity} \end{subfigure}% 
\begin{subfigure}[t!]{.18\columnwidth} \centering \includegraphics[width=\columnwidth]{figs/aerial_photography_error_operating_point}
   %\vspace{-20pt}
    \caption{\scriptsize Aer Photography.}
     \label{fig:benchmarks:OPA:ap:velocity}
    \end{subfigure}
\caption{Core/frequency sensitivity analysis of mission average velocity for various benchmarks.}
\label{fig:benchmarks_mission_velocity}
\end{figure}
   
  
   \begin{figure}[t!]
   \centering
   \begin{subfigure}[t!]{.18\columnwidth}
    \centering 
    \includegraphics[width=\columnwidth]{figs/scanning_flight_time_operating_point}
     %\vspace{-20pt}
    \caption{\scriptsize Scanning.}
    \label{fig:benchmarks:OPA:scanning:time}
    \end{subfigure}%
    \begin{subfigure}[t!]{.18\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/pd_flight_time_operating_point}
     %\vspace{-20pt}
    \caption{\scriptsize Package Delivery.}
    \label{fig:benchmarks:OPA:pd:time}
    \end{subfigure}%
    \begin{subfigure}[t!]{.18\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/mapping_flight_time_operating_point}
    % \vspace{-20pt}
    \caption{\scriptsize 3D Mapping.}
    \label{fig:benchmarks:OPA:mapping:time}
    \end{subfigure}%
     \begin{subfigure}[t!]{.18\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/SAR_flight_time_operating_point}
     %\vspace{-20pt}
    \caption{\scriptsize Search \& Rescue.}
    \label{fig:benchmarks:OPA:sar:time}
    \end{subfigure}%
    \begin{subfigure}[t!]{.18\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/aerial_photography_flight_time_operating_point}
   %\vspace{-20pt}
    \caption{\scriptsize Aer Photography.}
    \label{fig:benchmarks:OPA:ap:time}
    \end{subfigure}
    \caption{Core/frequency sensitivity analysis of mission time for various benchmarks.}
    \label{fig:benchmarks_mission_time}
\end{figure}
}

\textit{3D Mapping:} As compute scales, mission time reduces by as much as 86\% (\Fig{fig:benchmarks:OPA:mapping:velocity}, \Fig{fig:benchmarks:OPA:mapping:time}). The concurrency present in this application (all nodes denoted by circles with a filled arrow connection or none at all in \Fig{fig:benchmarks:data-flow:mapping} run in parallel) justifies the performance boost from core scaling. The sequential bottlenecks, i.e., motion planning and OctoMap generation explains the frequency scaling improvements. We achieve up to 6.3X improvement in motion planning (\Fig{fig:kernel-breakdown}) which leads to hover time reduction. We achieve a 6X improvement in OctoMap generation which leads to a maximum velocity improvement. Combined the improvements translate to a 5.3X improvement in average velocity. Improving average velocity reduces mission time.

\textit{Search and Rescue:} As compute scales, we see a reduction of up to 67\% for the mission time (\Fig{fig:benchmarks:OPA:sar:velocity}, \Fig{fig:benchmarks:OPA:sar:time}). Similar to the case of 3D Mapping, more compute allows for the reduction of hover time and an increase in maximum velocity which contribute to the overall reduction in mission time and energy. In addition, a faster object detection kernel prevents the drone from missing sampled frames during any motion. We achieve up to 1.8X, 6.8X, and 6.6X speedup for the object detection, motion planning and OctoMap generation kernels, respectively. In aggregate, these improvements translate to a 2.2X improvement in the MAV's average velocity.

\textit{Aerial Photography:} As compute scales, we observe an improvement of up to 53\% and 267\% for \emph{error} and mission time, respectively (\Fig{fig:benchmarks:OPA:ap:velocity}, \Fig{fig:benchmarks:OPA:ap:time}). Note that this application is a special case. In aerial photography, as compared to other applications, higher mission time is more desirable than a lower mission time. The drone only flies while it can track the person; hence, a longer mission time means that the target has been tracked for a longer duration. In addition to maximizing the mission time, error minimization is also desirable for this application. We define error as the distance between the person's bounding box (provided by the detection kernel) center to the image frame center.  Clock and frequency improvements translate to 2.49X and 10X speedup for the detection and tracking kernels and that allows for longer tracking with a lower error.

%\label{sec:comp_mass_impact_on_mission_time}
%\textit{\;\;\;\;Impact Path: Compute Subsystem -> Mass-> Acceleration-> Velocity-> Mission Time}
%\begin{figure}[!htb]

\subsection{Compute Mass Impact on Mission Time}
\label{sec:comp_mass_impact_on_mission_time}
Compute impacts mission time through its physical mass (mass cluster shown in Figure~\ref{fig:CIG_mass_paths} with green-color/double-sided paths). Increasing onboard compute affects the total weight of the MAV, which impacts the MAV's maximum acceleration and velocity, and consequently, that affects mission metrics (i.e., flight time).
To understand this impact, first, we need to understand the forces acting on a quadcopter. The free-body diagrams shown in Figures~\ref{fig:quad_FBD_2D}
and~\ref{fig:quad_FBD_3D} illustrate these forces in steady flight.\footnote{In a steady flight, the vehicle's linear and angular velocities are constant.}
The force generated by the motor is called thrust. In steady flight, the $y$ component of this thrust vector ($T_y$) compensates gravity ($W$) to keep the drone in the air while the $x$ component ($T_x$) combats the air drag ($D$). When decelerating, both thrust and drag act in the direction opposite to flight and make the vehicle slow down. The resulting maximum acceleration can be derived from Equation~\ref{eq:mass_acceleration}, where $m$ is the total vehicle mass, $D$ is the total drag and $T_{x_{max}}$ the maximum applicable thrust in the horizontal direction (negative when slowing down). Note that since we would like to calculate the worst case deceleration, we remove drag from the equation. 


\begin{figure*}[t!]
\centering
\includegraphics[width=\columnwidth]{figs/kernel-breakdown_2}
%\vspace{-18pt}
\caption{Kernel breakdown for MAVBench. The abbreviations are as follows: \emph{OD-}Object detection, \emph{MP-}Motion Planning, \emph{OMG-}OctoMap Generation for kernels and \emph{SC-}Scanning, \emph{PD-}Package Delivery,  \emph{MAP-}3D Mapping, \emph{SAR-}Search and Rescue, and \emph{AP-}Aerial Photography for applications. The $x$-axis lists the kernel-application names and $y$-Axis represents the runtime in seconds. Each bar graph represents one of the configurations used in the hardware. The cores are varied from 2 to 4 and the frequency goes from from 0.8 GHz , 1.5 GHz or 2.2 GHz.}
\label{fig:kernel-breakdown}
\end{figure*}



%I believe this is described properly in the text
% \begin{equation}
% \label{eq:mass_ty}
%     W = T_{y}
% \end{equation}
% \setlength{\belowcaptionskip}{-1ex}

\begin{equation}
\label{eq:mass_acceleration}
    a_{max} = \frac{T_{x_{max}}-D}{m}
\end{equation}
\setlength{\belowcaptionskip}{-1ex}


%Note that modelling the complex drag force would lead to great inaccuracy, hence we focus on thrust induced acceleration instead. In a quadcopter, the total thrust is a constrain of the platform. Using this information, it is possible to derive a relationship between the different thrust components:
Adding more mass to the drone demands a higher portion of thrust to battle weight, i.e., the drone requires higher $T_y$. Given the limited total thrust ($T_{max}$) that the motors can generate, a higher $T_y$ leaves the drone with less $T_x$ to accelerate with (Equation~\ref{eq:t_max}).
\begin{equation}
\label{eq:t_max}
    T_{x} = ~\sqrt[]{T_{max}^2 - T_{y}^2}
\end{equation}

Putting this all together, Equation~\ref{eq:mass_all} captures the relationship between mass and acceleration.

\begin{equation}
\label{eq:mass_all}
\boxed{
    a_{max} = \frac{~\sqrt[]{T_{max}^2 - W^2}}{m}}
\end{equation}
\setlength{\belowcaptionskip}{-1ex}


\begin{figure}[t!]
\begin{subfigure}[t]{0.45\textwidth}
\centering
\includegraphics[width=0.6\columnwidth]{figs/FBD_Quad.png}
%\vspace{-5pt}
\caption{2D free body diagram.}
\label{fig:quad_FBD_2D}
\end{subfigure}
\begin{subfigure}[t]{0.45\textwidth}
\centering
\includegraphics[width=0.7\columnwidth]{figs/FBD_Quad_2.png}
%\vspace{-5pt}
\caption{3D free body diagram.}
\label{fig:quad_FBD_3D}
\end{subfigure}
\caption{Forces acting on a quadcoptor. Knowing these forces is necessary in understanding how cyber and physical quantities impact one another.}
\end{figure}

Increasing onboard compute capability increases the weight of a MAV. As the amount of onboard compute increases, the thermal design power ($TDP$) escalates. Higher TDP requires more cooling effort and that automatically necessitates a more robust and heavier cooling system. %In other words, an increase in the onboard compute capability exacerbate the weight that the quad needs to carry.

To study the effect of mass, we consider four different system-on-chips (SoCs)
each with a different compute capability. Table~\ref{compute_platform_data} shows  
the mass associated with the different chipsets.\footnote{The weights are collected either through direct inquiry of the developing company or a thorough online search. We could not find a heat sink for the Xavier online, hence we exacted the heat sink weight through linear interpolation of the rest of data points.} 
We observe that the overall compute subsystem's weight vary from \SI{144}{\g} to \SI{1109}{\g}, i.e., a 7.9X increase, increasing the total MAV mass from \SI{2544}{\g} to \SI{3509}{\g}, i.e., a 1.4X increase.

\begin{table*}[!b]
\caption{Characteristics of the compute platforms we use for mass and holistic experiments. The platforms range from light yet high-end embedded platforms such as Jetson TX2 to heavy yet powerful high-end server such as an Intel Core i9.}
\label{compute_platform_data}
\resizebox{\columnwidth}{!}{    
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{10}{|c|}{MAV Compute subsystem}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & \begin{tabular}[c]{@{}c@{}}MAV \\ Robot \\ Complex\end{tabular}     \\ \hline
\multicolumn{3}{|c|}{Platform}                                                                                                                    & \multicolumn{3}{c|}{Performance}                                                                                                                                                                                                                   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Thermal\\  Power \\ (W)\end{tabular}} & \multicolumn{3}{c|}{Mass}                                                                                                                                                                 & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Mass\\ (g)\end{tabular}} \\ \cline{1-6} \cline{8-10}
Name          & \begin{tabular}[c]{@{}c@{}}Number\\  of \\ Cores\end{tabular} & \begin{tabular}[c]{@{}c@{}}CPU \\ Frequency\\  (GHz)\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}c@{}}Latency \\     (s)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}c@{}}Throughput\\      (Hz)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}c@{}}Total\\   (s)\end{tabular}} &                                                                                  & \begin{tabular}[c]{@{}c@{}}Board and\\  processor\\  (g)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Heat \\ Sink\\ (g)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Total \\ (g)\end{tabular} &                                                                     \\ \hline
i9-9940X      & 14                                                            & 1.2                                                               & .243                                                                            & 13.3                                                                                & .318                                                                       & 165                                                                              & 506                                                                   & 603                                                        & 1109                                                 & 3509                                                                \\ \hline
i7-4790K      & 7                                                             & 2                                                                 & .426                                                                            & 4.46                                                                                & .65                                                                        & 88                                                                               & 483                                                                   & 285                                                        & 768                                                  & 3168                                                                \\ \hline
Jetson Xavier & 8                                                             & 2.2                                                               & .586                                                                            & 3.25                                                                                & .894                                                                       & 30                                                                               & 280                                                                   & 100                                                        & 380                                                  & 2780                                                                \\ \hline
Jetson Tx2    & 6                                                             & 2                                                                 & .717                                                                            & 2.49                                                                                & 1.119                                                                      & 15                                                                               & 85                                                                    & 59                                                         & 144                                                  & 2544                                                                \\ \hline
\end{tabular}
}
\vspace{2pt}
\end{table*}


\begin{comment}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{3}{|c|}{Compute Platform}                                                                                                       & \multicolumn{3}{c|}{Performance}                                                                                                                                                                                                                   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Thermal\\  Power \\ (W)\end{tabular}} & \multicolumn{3}{c|}{Mass}                                                                                                                                                                                                                                 \\ \cline{1-6} \cline{8-10} 
Name          & \multicolumn{1}{l|}{Number of Core} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}CPU \\ Frequency\\  (GHz)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Latency \\     (s)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Throughput\\      (Hz)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Total\\   (s)\end{tabular}} &                                                                                  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Board and\\  processor\\  (g)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Heat \\ Sink \\ (g)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Total \\ (g)\end{tabular}} \\ \hline
i9-9940X      & 14                                  & 1.2                                                                                    & .243                                                                            & 13.3                                                                                & .318                                                                       & 165                                                                              & 453                                                                                        & 603                                                                              & 1109                                                                      \\ \hline
i7-4790K      & 7                                   & 2                                                                                      & .426                                                                            & 4.46                                                                                & .65                                                                        & 88                                                                               & 453                                                                                        & 285                                                                              & 768                                                                       \\ \hline
Jetson Xavier & 8                                   &    2.2                                                                                    & .586                                                                            & 3.25                                                                                & .894                                                                       & 30                                                                               & 280                                                                                        & 100                                                                               & 380                                                                       \\ \hline
Jetson TX2    & 6                                   &     2                                                                                   & .717                                                                            & 2.49                                                                                & 1.119                                                                      & 15                                                                               & 85                                                                                         & 59                                                                               & 144                                                                       \\ \hline
\end{tabular}
}
\vspace{2pt}


\end{table*}
\end{comment}
Using Equation~\ref{eq:mass_acceleration} and Table~\ref{compute_platform_data}, we study the impact of compute's added mass on the mission time (mass cluster denoted with green-color/double-sided impact paths in Figure~\ref{fig:CIG_mass_paths}) of a DJI Quadcopter, assuming it is equipped with the different compute platforms. We also study the effects of different environmental congestion levels (e.g., number of obstacles in the flight path). To study congestion levels, we introduce the notion of ``slow down ratio'' (SDR). This ratio is calculated as $v_{max}$, denoting maximum allowed velocity of a MAV, over $v_{avg}$, average velocity which the MAV maintains across its mission (Equation~\ref{eq:slow_down}), and it indicates environment's congestion. The higher the environment congestion, the higher the slow down ratio, resulting in a lower average velocity relative to maximum allowed velocity. This is because a congested space does not allow the drone to reach its top speed for long periods of time due to the frequent slowdowns caused by the numerous obstacles. 
\begin{equation}
\label{eq:slow_down}
    Slow\;Down\;Ratio\;(SDR) = \frac{V_{max}}{V_{avg}}
\end{equation}


\begin{figure}[t!]
\centering
     \begin{subfigure}{.4\linewidth}
   \centering
   %\setlength{\abovecaptionskip}{10pt}
   %\setlength{\abovecaptionskip}{-1pt}
   \includegraphics[width=.9\linewidth]{figs/mass_impact/mass_acc_vel.pdf}
   \vspace{-20pt}
   \caption{Impact on velocity and acceleration.}
   \label{fig:vel_acc_mass_impact}
    \end{subfigure}% 
    \begin{subfigure}{.4\linewidth}
  \vspace{-7pt}
  \centering
  %\setlength{\abovecaptionskip}{-3pt}
   %\hspace{-4pt}
   \includegraphics[width=.9\linewidth]{figs/mass_impact/mass_mission_time.pdf}
   %\setlength{\abovecaptionskip}{5pt}
    \vspace{-20pt}
    \caption{Impact on mission time.}
    \label{fig:comp_mt_mass_impact}
   \end{subfigure}
   \caption{Impact of compute mass, a physical quantity, on velocity, acceleration and mission time.}
      \label{fig:comp_stop_distance}
\end{figure}


Compute platform mass can considerably impact acceleration and velocity. Figure~\ref{fig:vel_acc_mass_impact} shows the impact of compute platform mass on $a_{max}$ and $v_{max}$. Different points on a line correspond to the different platforms in Table~\ref{compute_platform_data}. We see an acceleration of \SI{9.8}{\meter/\second\squared} vs. \SI{2.3}{\meter/\second\squared}, i.e., a 4.4X difference, for our lightest (TX2) and heaviest (i9) platforms, respectively. This difference leads to a velocity of \SI{11.7}{\meter/\second} vs. \SI{5.6}{\meter/\second}, respectively, i.e., a 2.1X difference, for our lightest and heaviest platform.

%4.4X improvement in acceleration leading to a 2.1X improvement in velocity as a result of mass difference between the heaviest (i9) and lightest (TX2) platform, respectively. 

Since compute mass impacts acceleration and velocity, it impacts mission time. Figure~\ref{fig:comp_mt_mass_impact}
shows this impact. Different points on a line correspond to the different platforms, and different lines correspond to different slow down ratios (SDRs). The acceleration and velocity differences discussed previously result in mission time of \SI{341}{\second} and \SI{713}{\second}, i.e., a 2X difference for TX2 and i9, respectively (for the most congested environment with the SDR of 4). Note that higher environment congestion grows the difference between the two extreme designs. For example, the mission time of the best and worse designs for SDR of 2 are \SI{170}{\second} and \SI{356}{\second} resulting in a difference of \SI{186}{\s} whereas same mission times for SDR of 4 are \SI{341}{\second} and \SI{713}{\second} resulting in a difference of \SI{372}{\s}. 

In summary, given these numbers, we conclude that lighter compute systems are of high value. Since the compute induced mass is mainly the result of cooling solutions to meet $TDP$, system designers need to target power-efficient designs. Furthermore, the analysis shows that dealing with congested spaces (such as in an indoor search and rescue mission) requires more compute efficiency from a mass perspective, and thus warrants greater demand for attention from system designers.




==> tex/role_of_comp_perf.tex <==
\section{Compute's Performance Impact}
\label{sec:char}
\blueDebug{old flow: compute-flight-time relationship:compute impacts average velocity through max velocity, hover time and localization,
compute-energy-relationship: energy pie char and hence reducing mission time leads to reducing energy}

\blueDebug{Section flow: 
                    - cluster 1 (examples) //subsection
                    - cluster 1 extensively studies with benchmarks
                   }                      
\blueDebug{
    #breakdown of experiments to show for each section
lets specify what we are planning to show for each one the paths:
-- through compute-performance:
    #mission time
    compute->throughput->velocity->missiontime  (theory, explanation, experiment(including benchmark based experiments))
    compute->latency->velocity->missiontime (theory, explanation, experiment (including benchmark based experiments))
    #energy 
    compute->latency->velocity->missiontime->energy (experiment)
    compute->latency->velocity->power->energy  (experiment (graph where velocity doesn't have an impact))

}

This section explores the paths within the first cluster in detail. These are the paths with which 
the compute subsystem impacts mission time and energy through performance variables such as latency and throughput.
To understand these interactions, first, we need to familiarize ourselves with a generic MAV mission task-flow (section~\ref{sec:task_flow}). Then, we illustrate how various impacts paths affect this flow and consequently mission time (section~\ref{sec:impact_1}). And finally,
we move beyond mission time to study impact paths that originate with performance variables and impact power and energy.  
We provide theoretical backgrounds and experimental results to quantify each impact path.


\begin{figure*}[t]
\centering
\includegraphics[height=1.65in, keepaspectratio]{figs/software_pipeline}
\caption{High-level application pipeline for a typical MAV application. The upper row presents a universal pipeline that all our MAVBench applications follow, which involves \emph{perception}, \emph{planning} and \emph{control}. The lower row presents how a specific workload in MAVBench (e.g. package delivery) maps to the universal high-level application pipeline.}
\label{fig:software_pipeline}
\end{figure*}


\textit{Impact Path: Compute Subsystem -> Throughput -> Velocity -> Mission Time}

Any MAV's application continuously samples sensory information and feeds them through the 3 stages mentioned above to generate actuation commands.
In this section, we show how by improving the latency and the throughput associated with this 3 stages, compute can increase mission's average velocity
and in turn reducing the mission time. We identify the reduction in hover time and the increase in maximum allowed velocity as two major ways with which more compute can contribute to a higher average velocity. 
%In this section, we show how compute's impact on perception, planning an control effects hover time, maximum velocity, and consequently average
%velocity, mission time and mission energy.

%sensory information it has collected through the 3 stage
%Compute can play an essential role in reducing the drone's mission time by increasing the mission's average velocity. To attain a high average velocity the drone needs to maintain a high velocity throughout its mission. To do this the drone needs to 1.have a high maximum velocity to traverse the trajectory with 2.maintain this high velocity and reduce deviation from it. 

\paragraph{Improving Max Velocity by improving Perception latency:} 
The maximum velocity of the drone is not only mechanically bounded, but also compute bounded. 
The faster the drone flies, the faster it needs to be able to process its sensory feed
to extract the MAV's and its environment's relevant states. In other words, \textit{faster flights require faster perception}. This can be easily seen with perception related compute intensive kernels such as
SLAM. SLAM localizes the drone by tracking a set of points/features through successive camera frames. A faster flight resulting in more rapid changes in drone's and environment
can be problematic for this kernel causing catastrophic effects such as permanent loss or a flight time increase (for example by backtracking) due to re-localization. Minimizing or avoiding localization-related failures is highly favorable, if not necessary.

 To examine the relationship between the compute, maximum velocity and localization failure, we
devised a micro-benchmark in which the drone was tasked to follow a predetermined circular path of the radius 25~meters. For the localization kernel, we used ORB-SLAM2 and to emulate different compute
powers; we inserted a sleep in the kernel. We swept different velocities and sleep times and bounded the failure rate to 20\%. As \Fig{fig:slam-velocity-energy} shows, higher FPS values, i.e., more
compute, allows for a higher maximum velocity for a bounded failure rate \footnote{Our simulation setup are extensively discussed in section ~\ref{sec:simulation}}. 


\paragraph{Reducing hover Time by  Improving Planning Latency:} Hover time and the average velocity have an inverse relationship; namely, the more drone spends time on hovering, the lower its average velocity. Similar to
an idling CPU, a hovering drone is unfavorable since it is not working toward its mission, but yet wasting its limited energy. A hovering drone typically is waiting for its planning stage to make a
decision (e.g., deciding on a path to follow). \emph{More compute power can help reduce hovering by reducing the planning's decision-making time, hence decreasing the negative effect hovering has on the average velocity.} 

\begin{figure}[t!]
\centering
    \begin{subfigure}{.49\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/fig_13}
    \caption{Theoretical max velocity.}
    \label{fig:process-time-velocity}
    \end{subfigure}
    \begin{subfigure}{.49\columnwidth}
    \centering
   \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/slam_fps_velocity_energy}
    \caption{Measured max velocity.}
    \label{fig:slam-velocity-energy}
    \end{subfigure}
\vspace{3pt}
%\setlength{\belowcaptionskip}{-4ex}
\caption{\emph{(a)} Theoretical relationship between processing time and maximum velocity. \emph{(b}) Relationship between SLAM throughput (FPS) and maximum velocity and energy of UAVs.}
%\label{SOLO_power_breakdown}
\end{figure}

\paragraph{Improving Max Velocity By Improving Sensory-to-Actuation Latency and Throughput:} For a given flight velocity, a
collision-free flight is only possible if the drone can process its surrounding fast enough to react to it. Therefore, \emph{a higher velocity requires a faster processing capability}. The collision
avoidance task can be rather compute-intensive exercising various stages of the pipeline starting from the pixel processing in the perception stage and ending with the command issue in control. To guarantee collision avoidance a  drone's maximum velocity is determined based on the aforementioned sensor to actuator response time.

Equation~\ref{eq:runtime-compute-bound} specifies the components involved in setting this velocity where $t$, $d$, $a_{max}$ and $v$ denote process time, required stopping distance, maximum acceleration limit of the drone and maximum velocity. By using this equation, we can show that our simulated drone, in theory, is bounded by the max velocity anywhere between 8.83 to 1.57 m/s given a pixel to response time of the range 0 to 4~seconds (\Fig{fig:process-time-velocity}). %\cite{high-speed-nav}. 

\begin{equation}
\label{eq:runtime-compute-bound}
v_{max} = a_{max}(~\sqrt[]{2*t^2 + 2\frac{d}{a_{max}}} - t)
\end{equation}
\setlength{\belowcaptionskip}{-1ex}
 
To understand this equation, let's consider a drone that periodically takes a snapshot of its environment (using its sensors), generates a trajectory and then follows it. In doing so, at any point if the
drone realizes that there is an obstacle on its path, it attempts to plan around it. However, if the motion planner fails to converge, the drone needs to decelerate immediately to avoid running into
the obstacle. Figures ~\ref{fig:comp_stop_distance_seq} and ~\ref{fig:comp_stop_distance_par} depict two design paradigms (i.e. sequential and pipe-lined) to capture this scenario in action.  

\begin{figure}[t!]
\centering
    \begin{subfigure}{.49\columnwidth}
    \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/vmax_seq.pdf}
    \vspace{5pt}
    \caption{stopping distance in a sequential design}
    \label{fig:comp_stop_distance_seq}
    \end{subfigure}
    \begin{subfigure}{.49\columnwidth}
   \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/vmax_pipe.pdf}
    \caption{stopping distance in a parallel design}
    \label{fig:comp_stop_distance_par}
    \end{subfigure}
      \label{fig:comp_stop_distance}
\end{figure}

\textit{Sequential Design:}
In figure~\ref{fig:comp_stop_distance_seq}, at point $Snap_{0}$, the drone takes a snap shot of the world, and spends a total 
of $\delta{t}_{SA\_latency}$ (SA stands for sensor to actuation) to perceive (latency denoted by $\delta_{Pr}$), plan (latency denoted by
$\delta_{Pl}$) and control (latency denoted by $\delta_{C}$) its maneuvers within its visible distance (d). This time is shown equation \ref{eq:latency}.

 In the sequential design, while the drone is going through one iteration of the PPC pipeline, no new snapshot is taken. This results in the
drone to be blind ($\delta{t}_{blind}$) for the entirety of the PPC pipeline, i.e. $\delta{t}_{blind}$ = $\delta{t}_{SA\_latency}$ and causing a \texit{momentarily} blind space until the next snapshot. In the
worst-case scenario, an obstacle (O) can be hiding within the blind space d - $v_{max}$*$\delta{t}_{blind}$ away from the drone. Point $Snap_{1}$ marks the second snapshot when the drone spends $\delta{t}_{reaction}$ to digest and respond to the new realization that it needs to plan around the unaccounted obstacle. This demands another pass through the PPC pipeline hence spending another $\delta{t}_{SA\_latency}$. At this point, if the drone fails to converge on a plan, it needs to slam on its breaks and hope to stop within distance calculated in equation \ref{eq:obstacle-distance}.
Equation \ref{eq:stop-distance} shows the distance that it takes for a moving body to come to a complete stop. Setting \ref{eq:obstacle-distance} and \ref{eq:stop-distance} equal to one another and solving for v results in \ref{eq:runtime-compute-seq}, the absolute maximum velocity with which the drone is allowed to fly in while guaranteeing a collision-free mission. 
 
 \begin{equation}
\label{eq:latency}
\delta{t}_{SA\_latency} = \delta{t}_{perception} + \delta{t}_{planning} + \delta{t}_{control}
\end{equation}

\begin{equation}
\label{eq:blind}
\delta{t}_{blind} = \delta{t}_{SA\_latency}
\end{equation}

\begin{equation}
\label{eq:reaction}
\delta{t}_{reaction} = \delta{t}_{SA\_latency}
\end{equation}

\begin{equation}
\label{eq:process_time}
t = \delta{t}_{blind} + \delta{t}_{reaction}
\end{equation}


\begin{equation}
\label{eq:obstacle-distance}
Worst Case Obstacle\;Distance= d - v_{max}*\delta{t}_{reaction} - v_{max}*\delta{t}_{blind}
\end{equation}

\begin{equation}
\label{eq:stop-distance}
Stopping\;Distance= \frac{v^2}{2*a_{max}} 
\end{equation}



\begin{equation}
\label{eq:runtime-compute-seq}
v_{max} = a_{max}(~\sqrt[]{4*\delta{t}_{SA\_latency}^2 + 2\frac{d}{a_{max}}} - 2*\delta{t}_{SA\_latency})
\end{equation}
\setlength{\belowcaptionskip}{-1ex}

 

\textit{Pipelined Design:}
As shown in figure~\ref{fig:comp_stop_distance_par}, by overlapping perception, planning and control, we can reduce the blind time to the inverse of the system's throughput.
Note that since each stage has a different latency, throughput needs to be calculated as shown in equation \ref{eq:throughput} where $\Delta{t}$ is the throughput's inverse. note that in this design $\delta{t}_{reaction}$ stays intact i.e, equal to $\delta_{SA\_latency}$.
Using the pipeline approach the velocity can be calculated using equation \ref{eq:runtime-pipe}. 



\begin{equation}
\label{eq:throughput-blind}
\delta{t}_{blind} =\Delta{t} 
\end{equation}

\begin{equation}
\label{eq:throughput}
 \delta_{SA\_throughput} = \frac{1}{\Delta{t}} = Min(\frac{1}{\delta{t}_{perception}},  \frac{1}{\delta{t}_{planning}}, \frac{1}{\delta{t}_{control}})
\end{equation}

\begin{equation}
\label{eq:runtime-pipe}
v_{max} = a_{max}(~\sqrt[]{(\delta{t}_{SA\_latency} + \Delta{t})^2 + 2\frac{d}{a_{max}}} - (\delta{t}_{SA\_latency} + \Delta{t}))
\end{equation}
\setlength{\belowcaptionskip}{-1ex}

It's important to note that the pipelined design does not necessarily improve the velocity. This is because process time $t$ is equal to $\delta{t}_{SA\_latency}$ + $\Delta{t}$; hence, if the pipelined design increases $\delta{t}_{SA\_latency}$ (e.g. due to the communication overhead between parallel processes),  the overall process time might increase. This means that at design time, careful analysis of the tradeoffs between throughput and latency needs to be accounted for.  

%\begin{figure}[h]
%\includegraphics[]{figs/blank.pdf}
%\caption{Measurement set up to collect power data for 3DR Solo.}
%\label{sec:powerbreakdown}
%\end{figure}
\begin{comment}
\paragraph{Maintaining Max Velocity}
As was discussed before, to reduce the mission time, it's not enough to have a high bound on v ($v_{max}$), but we need to reach $v_{max}$ and maintain it during the flight. In other words, once $v_{max}$
is reached, the drone should attempt at reducing deviation from it. This means that the trajectories of low curvature are desired.  \red {this is a point about acceleration. Not sure if I should bring.
if we decide to bring it, then I need to add another picture and formula}
\end{comment}

\subsection{Core and Frequency Scaling}
\label{sec:operating-spoints}
To understand the impact of compute performance and power on the MAV's system complex, 
we conducted a series of performance and power sensitivity analysis using core and
frequency scaling. TX2 has two sets of cores, namely a \textit{HMP Dual Denver cores} and a \textit{Quad ARM A57}. We turned off the Denver cores so that the indeterminism caused by process to core mapping variations across runs would not affect our results.
Average velocity, mission, and energy values of various operating points are profiled and presented as heat maps (\Fig{fig:benchmarks:OPA:scanning}---\Fig{fig:benchmarks:OPA:ap}) for a DJI Matrice 100 drone. \emph{In general, compute can improve mission time and lower energy consumption by as much as 5X.}

\paragraph{Scanning:}
We observe trivial differences for velocity, endurance and energy across all three operating points (\Fig{fig:benchmarks:OPA:scanning:velocity}, \Fig{fig:benchmarks:OPA:scanning:time}, and \Fig{fig:benchmarks:OPA:scanning:energy}). This is despite seeing a 3X boost in the motion planning kernel, i.e. lawn mower planning, which is its bottleneck (\Fig{fig:kernel-breakdown}). The trivial effect of compute on this application is because planning is done once at the beginning of the mission and its overhead is amortized over the rest of the mission time. For example the overhead of planning for a 5 minute flight is less than .001\%.  
 
\paragraph{Package Delivery}:  As compute scales with the number of cores and/or frequency values, we observe a reduction of up to 84\% and 82\% for the mission time and energy consumption, respectively (\Fig{fig:benchmarks:OPA:pd:time}, and \Fig{fig:benchmarks:OPA:pd:energy}). The sequential bottlenecks i.e. motion planning and OctoMap generation kernel are sped up by frequency scaling to enable the observed improvements. There does not seem to be a clear trend with core scaling, concretely between 3 and 4 cores. We conducted investigation and determine that such anomalies are caused by the non-real-time aspects of ROS, AirSim and the TCP/IP protocol used for the communication between the companion computer and the host. We achieve up to 2.9X improvement in OctoMap generation and that leads to maximum velocity improvement. It is important to note that although we also gain up to 9.2X improvements for the motion planning kernel, the low number of re-plannings and its short computation time relative to the entire mission time render its impact trivial. Overall the aforementioned improvements translate to up to 4.8X improvement in the average velocity. Therefore, mission time and the MAV's total energy consumption are reduced.

{
\begin{figure}[t!]
    \centering
    \begin{subfigure}[t!]{.18\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/scanning_velocity_operating_point}
    \caption{Velocity (m/s)}
    \label{fig:benchmarks:OPA:scanning:velocity}
    \end{subfigure}%
    \begin{subfigure}[t!]{.19\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/pd_velocity_operating_point}
    \caption{Velocity (m/s)}
     \label{fig:benchmarks:OPA:pd:velocity}
    \end{subfigure}%
     \begin{subfigure}[t!]{.19\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/mapping_velocity_operating_point}
    \caption{Velocity (m/s)}
    \label{fig:benchmarks:OPA:mapping:velocity}
    \end{subfigure} %  
     \begin{subfigure}[t!]{.19\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/SAR_velocity_operating_point}
    \caption{Velocity (m/s)}
    \label{fig:benchmarks:OPA:sar:velocity}
    \end{subfigure}%
     \begin{subfigure}[t!]{.19\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/aerial_photography_error_operating_point}
    \caption{Error Rate(m/s)}
     \label{fig:benchmarks:OPA:ap:velocity}
    \end{subfigure}
    \end{figure}
   
  
   \begin{figure}[t!]
   \centering
   \begin{subfigure}[t!]{.18\columnwidth}
    \centering 
    \includegraphics[width=\columnwidth]{figs/scanning_flight_time_operating_point}
    \caption{Mission Time (s)}
    \label{fig:benchmarks:OPA:scanning:time}
    \end{subfigure}%
    \begin{subfigure}[t!]{.19\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/pd_flight_time_operating_point}
    \caption{Mission Time (s)}
    \label{fig:benchmarks:OPA:pd:time}
    \end{subfigure}%
    \begin{subfigure}[t!]{.19\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/mapping_flight_time_operating_point}
    \caption{Mission Time (s)}
    \label{fig:benchmarks:OPA:mapping:time}
    \end{subfigure}%
     \begin{subfigure}[t!]{.19\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/SAR_flight_time_operating_point}
    \caption{Mission Time (s)}
    \label{fig:benchmarks:OPA:sar:time}
    \end{subfigure}%
    \begin{subfigure}[t!]{.19\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/aerial_photography_flight_time_operating_point}
    \caption{Mission Time(s)}
    \label{fig:benchmarks:OPA:ap:time}
    \end{subfigure}
\end{figure}
}

\paragraph{Mapping:} We observe a reduction of up to 86\% and 83\% for the mission time and energy consumption, respectively, as compute scales with the number of cores and/or frequency values (\Fig{fig:benchmarks:OPA:mapping:velocity}, \Fig{fig:benchmarks:OPA:mapping:time}, and \Fig{fig:benchmarks:OPA:mapping:energy}). The concurrency present in this application (all nodes denoted by circles with a filled arrow connection or none at all in \Fig{fig:benchmarks:data-flow:mapping} run in parallel) justifies the performance boost from core scaling. The sequential bottlenecks, i.e. motion planning and OctoMap generation explains the frequency scaling improvements. We achieve up to 6.3X improvement in motion planning (\Fig{fig:kernel-breakdown}) and that leads to hover time reduction. We achieve a 6X improvement in OctoMap generation and that leads to maximum velocity improvement. The improvements translate to a 5.3X improvement in average velocity. Since mission time is reduced, total energy consumption reduces.

\paragraph{Search and Rescue:} We see a reduction of up to 67\% and 57\% for the mission time and the energy, respectively, as compute scales (\Fig{fig:benchmarks:OPA:sar:velocity}, \Fig{fig:benchmarks:OPA:sar:time}, and \Fig{fig:benchmarks:OPA:sar:energy}). Similar to mapping, more compute allows for the reduction of hover time and an increase in maximum velocity which contribute to the overall reduction in mission time and energy. In addition, a faster object detection kernel prevents the drone from missing sampled frames during any motion. We achieve up to 1.8X, 6.8X, and 6.6X speedup for the object detection, motion planning and OctoMap generation kernels, respectively. In aggregate, these improvements translate to 2.2X improvement in the MAV's average velocity.

\paragraph{Aerial Photography:} We observe an improvement of up to 53\% and 267\% for \emph{error} and mission time, respectively (\Fig{fig:benchmarks:OPA:ap:velocity}, \Fig{fig:benchmarks:OPA:ap:time}, and  \Fig{fig:benchmarks:OPA:ap:energy}). In aerial photography, as compared to other applications, higher mission time is more desirable than a lower mission time. The drone only flies while it can track the person, hence a longer mission time means that the target has been tracked for a longer duration. In addition to maximizing the mission time, error minimization is also desirable for this application. We define error as the distance between the person's bounding box (provided by the detection kernel) center to the image frame center.  Clock and frequency improvements translate to 2.49X and 10X speedup for the detection and tracking kernels and that allows for longer tracking with a lower error. No significant trend is observed in the energy data because energy depends on both the mission time and the velocity, and as opposed to the other applications, there is no need for the drone to minimize its velocity. Instead, it needs to successfully track the person.

\begin{figure*}[!t]
\centering
\includegraphics[width=\columnwidth]{figs/kernel-breakdown_2}
\vspace{-18pt}
\caption{Kernel breakdown for MAVBench. The abbreviations are as follows: \emph{OD-}Object detection, \emph{MP-}Motion Planning, \emph{OMG-}OctoMap Generation for kernels and \emph{SC-}Scanning, \emph{PD-}Package Delivery,  \emph{MAP-}3D Mapping, \emph{SAR-}Search and Rescue, and \emph{AP-}Aerial Photography for applications. The $x$-axis lists the kernel-application names and $y$-Axis represents the runtime in seconds. Each bar graph represents one of the configurations used in the hardware. The cores are varied from 2 to 4 and the frequency goes from from 0.8 GHz , 1.5 GHz or 2.2 GHz.}
\label{fig:kernel-breakdown}
\end{figure*}


\subsection{Impact on Mission Energy}
\label{sec:impact_2}
\textit{\;\;\;\;Impact Path: Compute Subsystem -> Latency -> Velocity -> Mission Time -> Mission Energy}

\textit{Impact Path: Compute Subsystem -> Throughput -> Velocity -> Mission Time -> Mission Energy}

The compute subsystem can also have a significant role in reducing total MAV's energy consumption. 
At the high-level, by reducing the mission time, we can reduce the total system's energy by flying the
quad for a shorter period of time. This is similar to techniques studied in the system and architecture community to reduce overall energy by cutting down on the run time (\red{have some papers here}).
Using the models provided in section ~\ref{sec:energy}, we profiled the mission time and the energy associated with the aforementioned micro-benchmark. 
As the bottom plot in \Fig{fig:slam-velocity-energy} shows, a higher compute capability increase velocity (bottom graph) which results in total system energy (top graph). By increasing processing speed by 5X, we were able to reduce the drone's energy consumption by close to 4X.

\begin{figure}[!t]
    \centering
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=.5\columnwidth]{figs/drone-power-time-series}
    \caption{Total measured power consumption while the drone is "Flying" at two different steady-state velocities. Minor change in values are observed}
    \label{fig:drone-power-time-series}
\end{figure}


\subsection{Impact on Quad's Power}
\label{sec:impact_3}

\textit{\;\;\;\;Impact Path: Compute Subsystem -> latency -> Velocity -> Power -> Mission Energy}

\textit{Impact Path: Compute Subsystem -> throughput -> Velocity -> Power -> Mission Energy}

The velocity with which the drone flies with impacts the amount of power and hence energy it consumes. To measure the variation in power 
under different velocities (within the velocity bounds that
compute allows), we attached a watt meter known as Eagle~Tree Systems eLogger~V4~\cite{eLoggerV4} to the \solo~\cite{solo3DR}, a popular off-the-shelf MAV. eLogger allows us to collect battery data during flight time at 50~Hz. We command the drone to fly for fifty seconds and pull the data off of the watt meter after the drone lands.
As \Fig{fig:drone-power-time-series} shows, this variation is minor. 
This is because, majority of the rotor powers are spent to keep the drone in the air (hovering),
but once in the air, relatively a small amount is used for moving forward. 



==> tex/role_of_comp_power.tex <==
\section{Compute's Power Impact}
\label{sec:impact_through_power}


\textit{\;\;\;\;Impact Path: Compute Subsystem -> Power -> Mission Energy}

This section discusses the third cluster. These are the paths with which the 
compute impacts mission energy directory through compute subsystem's power.

%\subsection{Compute Power and Quad's Mission Energy Relationship}
To understand the impact of compute's power consumption on the entire system's power and energy, 
first, we present the power distribution associated with \solo~\cite{solo3DR} using our Eagle~Tree Systems
eLogger~V4~\cite{eLoggerV4} setup. Note that to isolate the impact of compute power and cut out the mass impact, we
measure the rotor's power with 0g load. However, section~\ref{sec:impact_holistic}
brings back the load and holistically examines at all impact paths at once.

\begin{figure}[!t]
\centering
       \vspace{-50pt}
    \includegraphics[trim=0 0 0 0, clip, width=\columnwidth]{figs/power_break_down}
     \vspace{-90pt}
    \caption{Measured power breakdown.}
   
    \label{fig:power_break_down}
\end{figure}
% The wattmeter gave us the total power consumed by the drone, without a deeper breakdown. To estimate the portion of the instantaneous power that would typically be consumed by a MAV's processor, we subtracted the idle power consumption of the \solo's default onboard computer and added to it the power consumed by the TX2 during typical workloads.

\Fig{fig:power_break_down} shows the power consumption of both the compute and the rotors for the
four platforms mentioned above. As illustrated, depending on the on board's compute capability, 5\% to 38\% of the system power will be directly consumed by the compute subsystem power. \red{I wonder if there is a take away here, besides reporting number}






\begin{figure}[t!]
    \centering
    \begin{subfigure}[t!]{.19\linewidth}
    \centering
    \includegraphics[width=\linewidth] {figs/scanning_energy_operating_point}
    \label{fig:benchmarks:OPA:scanning:energy}
    \caption{Scanning Energy.}
    \end{subfigure}
    \begin{subfigure}[t!]{.19\linewidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/pd_energy_operating_point}
     \label{fig:benchmarks:OPA:pd:energy}
       \caption{Package Delivery Energy.}
    \end{subfigure}%
    \begin{subfigure}[t!]{.19\linewidth}
    \includegraphics[width=\linewidth] {figs/mapping_energy_operating_point}
     \label{fig:benchmarks:OPA:mapping:energy}
        \caption{Mapping Energy.}
    \end{subfigure}%
    \begin{subfigure}[t!]{.19\linewidth}
    \centering
    \includegraphics[width=\linewidth] {figs/SAR_energy_operating_point}
     \label{fig:benchmarks:OPA:sar:energy}
      \caption{Search and Rescue Energy.}
    \end{subfigure}%
    \begin{subfigure}[t!]{.19\columnwidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/aerial_photography_energy_operating_point}
     \label{fig:benchmarks:OPA:ap:energy}
     \caption{Aerial Photography Energy.}
    \end{subfigure}
\end{figure}



%the majority of the power consumption is 
%dedicated to rotors (locomotion) and the compute only occupies a relatively
%small portion of the entire pie and its role seemingly trivial. 
%This pie for four different platforms discussed in the previous section are shown.

%Although small in quantity, compute can have a grand effect on the system's power. This is because by reducing the mission time (as explained in the previous section), more compute power can, in fact, reduce the bigger portion of the pie, namely rotors energy consumption (due to a shorter flight). Note that although more compute can lead to more energy consumption of the compute subsystem, the reduction in rotor's energy can easily outweigh such an increase.  




% \setlength{\belowcaptionskip}{-2ex}




==> tex/scaling.tex <==
\section{compute-robot interplay: a holistic look}\label{scaling}
\blueDebug{section summary: broadening the interaction understanding. introducing the SIG as a tool. use graph for two different interaction analysis. zoom out and investigate another interaction}

To further our understanding of the compute-robot interplay, this section takes a more holistic look at various ways in which such interactions take place. We believe that understanding and examining these interactions are necessary since cyber-physical systems are a compilation of many intertwined components. Hence, similar to the cross-compute-layer optimization approach which is widely adopted by the compute system designers, robot’s cross system (compute, mechanical (actuators), electrical(battery,..)) considerations and optimizations are desirable. To this end, first, we introduce a Directed Acycle Graph as a tool to capture the robots inter-dependencies; Then, we provide three case studies where this graph is used to gain insight into system development and  guiding the design decision making process.

\subsection{cross-system interaction graph}
\blueDebug{explain graph:edges and nodes. define impact paths and do a graphical example}
Cyber physical machines are a compilation of different set of systems and sub-components all working together toward a mission at hand. An optimal design, not only should consider the individual components in isolation, but also investigate the opportunities across different systems. Designers need to understand various ways in which these subsystems impact one another and the overall robot's behavior. We introduce the cross-system interaction DAG as a tool for such considerations (Figure 
\ref{fig:CSIG_general}). The graph consists of three types of vertices: 1. robot's subsystems such as compute, actuators, sensors, battery denoted by rectangles 2.system variables such as compute's throughput, mass and system's consumed energy denoted by non-filled circles 3. models mapping one variable to another denoted by filled circles. The edges implies the existence and the direction of the interactions. In order to investigate the impact of variable on another, we need to examine all the paths (impact paths) leading from the first to the second variable. For example, in figure \ref{fig:CSIG_general}, the two paths from $subsystem_{0}$ to $var_2$ are shown in bold with different dashed patterns (i.e .. and $_.$). To examine the total impact of $subsystem_0$ on $var_2$, each one of these impact paths need to be considered and finally combined (for example by using the model marked with +)

\blueDebug{SIG for our quad. exemplify two paths with short description. explain direct/indirect interactions. outro to case studies}
Figure \ref{fig:CSIG_combined} on the left, shows this graph for our quad robot. Our mapping models range from simple addition (marked by 1), to more complicated linear functions (marked with 2) to non-linear relations (marked with 3). . For example the bold paths in figure \ref{fig:CSIG_combined} on the left show all paths 
\ref{fig:CSIG_combined} on the right, as an example, highlights the interactions and impacts of compute subsystem on mission energy. The red, blue, and purple edges respectively denote direct, indirect, and hybrid interactions between compute and other variables leading up to the mission energy. For example, the red line between compute and latency shows that compute directly impacts latency, whereas the blue line between latency and velocity shows the indirect way (i.e. through latency) in which compute impact velocity. We counted total of \red{blah} number of different paths with which compute impacts mission time. Two of such paths are illustrated with dashed paths, each with a different quantity and direction of impact. The dot/line ($._$) dashes show how compute impacts mission's energy by traversing through latency, velocity, and mission time vertices. Through this path, an increase in compute capability, reduces latency, and as a result increasing velocity, reducing mission time and finally leading to reduction in mission energy. On the other hand, the dotted lines (i.e. ..) shows this impact through power directly, where and increase in compute capability, increases the power consumption and hence increases mission energy. 

The developers can use the interaction graph to gain various insights similar to one mentioned above to guide them through the design process. The next two subsections use this approach to investigate the impact of scaling the compute capability and size on the robot. Finally the last subsection, goes beyond our specific quad to general mobile robots examining the impact of increase in robot complexity (more joints, links) on compute requirements.

\begin{figure}[t]
%\vspace{-5pt}
\centering
\includegraphics[trim=0 0 0 0, clip, width=\columnwidth]
{figs/cross_system_interaction_graph_general.pdf}
%\vspace{-23pt}
%\vspace{-15pt}
\caption{cross system interaction DAG (CSIG) captures the inter-dependencies between robot's subsystems.}
%\vspace{15pt}
\label{fig:CSIG_general}
\end{figure}


\begin{figure*}[!t]
%\vspace{-5pt}
\centering
\includegraphics[trim=0 0 0 0, clip, width=\linewidth]
{figs/cross_system_interaction_graph_combined}
%\vspace{-23pt}
%\vspace{-15pt}
\caption{cross system interaction DAG captures the inter-dependencies between robot's subsystems. left: all interactions right: compute interactions (direct/indirect)}

\label{fig:CSIG_combined}
\end{figure*}


\begin{comment}
\begin{figure*}[!t]
\vspace{-12pt}
    \centering
    \begin{subfigure}[t]{.55\linewidth}
        \centering
        \includegraphics[height=1.4in]{figs/cross_system_interaction_graph_quad.pdf}%
        \caption{All interactions.}%
        \label{CSIG_our_quad}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.4\linewidth}
        \centering
        \includegraphics[height=1.4in]{figs/cross_system_interaction_graph_colored.pdf}%
        \caption{compute (direct/indirect) interactions.}%
        \label{fig:CSIG_colored}
    \end{subfigure}
    \caption{Our quad's cross-section interaction graph.}
    \label{fig:CSIG_quad}
\end{figure*}
\end{comment}

\red{ask Brian about what to call each layer. Maybe call the second layer, kenimatic, dynamic variables}


%\blue{summary: cross system interaction needs to be captured. we introduce a graph.}
%\blue{CPS are combination of various parts. The interactions across subsystems need to be considered. We introduce a graph capturing this dependencies. An example of this graph (for our system). explain the graph. color code the graph and explain}


%Understanding how various component of the system impact one another is a necessary stop in design of cyber physical systems. To capture these interdepencies, we introduce a simple graph called "cross system interaction" graph. This graph consists of two different kind of vertices, 1. system variables,metrics (denoted by square) 2.models showing the relationship between these variables (denoted by circles). If there is an edge between two square nodes, that means the two impact one another (through the circular vertex). We constructed the the interaction graph for our system (Figure blah). Since each robot has a different interaction graph, 

%optimal design section proposes a simple methodology to accomplish this. Furthre, we use this methodology to introduces a simple graph as the starting point 


%\red{I think I should total sell the robot complexity as the increase in actuations. we should also mention that another way is to increase the number of sensors, but we don't discuss that}

\begin{figure}[t]
%\vspace{-5pt}
\centering
\includegraphics[trim=0 0 0 0, clip, width=\columnwidth]
{figs/latency_throughput_energy}
\vspace{-23pt}
%\vspace{-15pt}
\caption{impact of scaling compute on energy}
%\vspace{15pt}
\label{fig:compute_scaling}
\end{figure}

\subsection{scaling compute}
 Scaling compute impacts the mission time and mission energy in various ways (concretely blah number of ways) two examples of which were illustrated in the previous subsection. System designers need be aware of these paths during development and design space exploration stages. In this subsection we examine such scaling in details and investigate the boundaries. 
 
 if not detailed (cause the models are not accurate) then what. 
 possibly say something about how we calculated mission time and energy (assumptions made)
 what can we say. let's list all the graphs. 
 
 so we the latency, mission energy, latency, mission time (possibly combined the two).
 latency missiontime*mission*energy. 
 
 can we say something about some ratio: like latency/power*mass metric and how that impact the mission energy and mission time.
 if we can show that for common embedded platforms, that would be awesome.
 
 
 can we show different.
 
 ideally, 
 we'll show compute scaling (DMIPS), latency, throughput scaling, power and mass for real platforms.using this, maybe we can find models for:
 
 compute scaling->power scaing
                -> mass scaling
                -> throughput, latency scaling
 and extrapolate from there.
 
show, the performance/power*mass for different platforms

 but 1. we don't have DMIPS, power and mass for different systems, and even if we did, we won't be able to measure latency on all of them. 
 
 what if we show the data for different platforms such as tx2, xavier, wenzhi's machine and wills machine
                
 
 
 
 
 


\subsection{scaling size}
\red{size scaling impact on compute efficiency}
Robots of various sizes are used for various applications. For example, micro drones are used for blah and nano drones are used for blah (use same application but different environments or situations maybe). As we scale down the robot size, so does with it the amount of energy onboard,
however, the same level of intelligence is needed regardless. This requires and increase in compute efficiency to battle the onboard reduction. This sections show the impact of scaling size on compute.

\begin{equation}
\label{eq:energy-components}
E_{total} = E_{compute} + E_{actuators}
\end{equation}
\setlength{\belowcaptionskip}{-1ex}

Total energy of the system is equal to energy consumed by the compute subsystem (processor, memory, ...) and the physical/mechanical subsystem (rotors). (\ref{eq:energy-components}).
As we scale down the system's size by a factor of S in each direction, the amount of energy onboard scales down with a factor of S^3 ($E_{total}$/s^3). However, as the size scales, so does mass with S^3 reducing the necessary thrust required to lift the drone. This in turns reduces the  and hence reducing the rotor's power and energy by a factor of S^3.5 (E_{actuators}/S^3.5). equation \ref{eq:thrust} and \ref{eq:exit_velocity} shows the relationship between Thrust and power and equation \ref{eq:power_thrust_velocity}} illustrate the scaling impact. 
 

\begin{equation}
\label{eq:thrust}
T = 2\rho*A*v^2
\end{equation}
\setlength{\belowcaptionskip}{-1ex}

\begin{equation}
\label{eq:exit_velocity}
v = sqrt(\frac{T}{2\rho*A})
\end{equation}
\setlength{\belowcaptionskip}{-1ex}

\begin{equation}
\label{eq:power_thrust_velocity}
P = T*v
\end{equation}
\setlength{\belowcaptionskip}{-1ex}

\begin{equation}
\label{eq:energy-components}
P/S^3.5 = T/S^3*v/S^.5
\end{equation}
\setlength{\belowcaptionskip}{-1ex}

\begin{figure}[t]
%\vspace{-5pt}
\centering
\includegraphics[trim=0 0 0 0, clip, width=\columnwidth]
{figs/size_scaling}
\vspace{-23pt}
%\vspace{-15pt}
\caption{impact of scaling size on the available compute power/energy}
%\vspace{15pt}
\label{fig:compute_scaling}
\end{figure}


\subsection{scaling robot complexity}
To implement complicated tasks such as the robots DOF need to scale. This section shows how scaling the robot complexity impacts the compute.

\subsection{environment congestion scaling}
As the congestion of the environment increase, the visibility of the drone is reduced. This in turn reduces the maximum velocity and hence increases the energy consumed  (\ref{fig:vis_scaling})

\begin{figure}[t]
%\vspace{-5pt}
\centering
\includegraphics[trim=0 0 0 0, clip, width=\columnwidth]
{figs/visibility_energy}
\vspace{-23pt}
%\vspace{-15pt}
\caption{visibility impact on power/energy}
%\vspace{15pt}
\label{fig:vis_scaling}
\end{figure}

==> tex/scratch.tex <==
\section{misc}
// make sure the figures are placed properly
// fix the link thing that vijay talked about
// slam numbers
// add mission time values for sar and mapping
// double check the numbers
// get rid of the apostrophe at the beginning
// add links for the CIG figure
// double check figure placement, e.g., making sure that theyare not showing up before they are mentioned
// make sure all the numbers bellow 10 are written in letters


what dose this mean:
MAVBench applications are comprised of holistic end-to-end application dataflows found in a typical real-world drone application. 
"compute impact" or "comput's impact"
// in intro we have numbers in two paragraphs. Double check with vijay about that.
// double check the CCS concepts: make sure robotics is second
// To do
// either use X or percentage thruoghtout
// change computes's impact, compute's mass, compute's performance and power to without apastrophe
// double check all the numbers



// for each unit of work done in compute (you can think of it for example perforamnce/watt) or maybe MIPS how much unit of real work done (that is action base, so movement for example). Can we use this to propose a new metric (instead of performance/watt*mass so for example do cyber perforamnce/watt over physical performance/watt)
// what is the velocity distribution. That can be a way to measure the efficiency of the system. We might be able to do the same thing with acceleration. augment your QOF with velocity and it's standard deviation. 




//todos:

// define new semantics for IG
// have 3 CP-IG
// have forward refrecne in evaluation section (7) to different insights
// have forward refrance for role of compute section explaining high level insights (3.2)
//explain throughput/latency velocity better

I think I should switch to cyber physical interaction graph, but the problem is that in that
case, then 

 //consult with vijay about heat sink data for xavier
// find data for the SOC
// make sure the weights are calculated properly
is there a way to calculate how much power efficinecy (and possibly the new metric efficiency buy us for different platforms?)
make sure you are consistent about drone, quad or mav
find out how to include queueing latency into the throughput
writing
we might have to move around the intro for \section{The Role of Compute in MAVs: Performance Angle} to the previous section.

terminology:
  impact path or impact vector (if we talk about direction and magnitude the latter is better)



#------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
archived
rework the calcs with 3DR solo to be consistent //don't think we need it since all the experiments for freq,core scaling done with DJI
#------------------------------------------------------------------------------------------------------------------------------------------------------------------------------




use the ecalc:
  I think we should fix the hover throttle (and possibly do both arabotics (80\%) and photography (50\%) where each require a different \%), or possibly fix the flight time, or fix the thrust-weight. but what is the different between thrust-weight and throttle\%. or possibly fix the speed
  scaling:
  battery scaling (with size):
  https://www.all-battery.com/sizechart.aspx
  
 a graph for battery weight and capacity:https://oscarliang.com/how-to-choose-battery-for-quadcopter-multicopter/
  
  propellers effciency:
  https://web.mit.edu/16.unified/www/FALL/thermodynamics/notes/node86.html   (11.7.3)
  https://www.apcprop.com/technical-information/performance-data/   (UIUC propellers data)
  
  http://cecs.wright.edu/~sthomas/aronsconferencepaper.pdf  (page 23 at the bottom, a paper on efficiency)
  
  https://www.researchgate.net/profile/Ohad_Gur/publication/280566585_Maximum_Propeller_Efficiency_Estimation/links/55bd946808ae9289a0984b3a.pdf  (another paper)
   -------------
  comparing GFLOps for different processors:
  
  https://asteroidsathome.net/boinc/cpu_list.php
  https://www.cpubenchmark.net/CPU_mega_page.html#notes
  
  FLOPS = Number of Cores * Average Frequency * Operations per Cycle   (hence we see, by doubling the cores or increasing the frequency, we can increase FLOPS.) but is FLOPS really a good measure here?
  
  
  -------
  jetson carrier:
  http://connecttech.com/product/nvidia-jetson-tx2-tx1-active-heat-sink/
  the following is all the products that connecttech has
  http://connecttecsuch as weight)h.com/pdf/CTI_NVIDIA_TX2_brochu. search for specs (re_Web_sm.pdf
  
  ----------------------
  battery lists:
  https://www.all-battery.com/sizechart.aspx
  can we find the volume to energy scaling of these batteries
  
  different kind of batteries:
  https://batteryuniversity.com/learn/article/a_look_at_cell_formats_and_how_to_build_a_good_battery
  
  
  arm comparison (uses DMIPS/MHZ (should be devide by MHZ?)):
  https://www.wikiwand.com/en/Comparison_of_ARM_cores
  ------------------------
  
  take a look at this for for 
  Performance/watt*space: https://en.wikipedia.org/wiki/Performance_per_watt
  
  
  DMIPS and processsors:
  https://en.wikipedia.org/wiki/Instructions_per_second#Timeline_of_instructions_per_second
  die size and processors:
  https://en.wikipedia.org/wiki/Transistor_count
  
  https://en.wikipedia.org/wiki/Microprocessor_chronology
  
  power dissipatio:
  https://en.wikipedia.org/wiki/List_of_CPU_power_dissipation_figures
  -------------------
  explanation for thrust:
  https://quadstardrones.com/the-equations-for-speed/
  -------------------------
  a good list of drones and their specs
  https://www.tomsguide.com/us/best-drones,review-2412.html
  
  
  
  
  // scaling studies:
 1. Show how energy left for compute to consume reduces as the size reduces?
 2. Show how the compute needs to scale with as the complexity of the robot increases. We can model an increase in complexity of the robot in different ways. One way is to increase the 


==> tex/simulator.tex <==
%\externaldocument{./../tex/MAVBench.tex}

\section{Closed-loop Simulation}
\label{sec:simulation}
\setstcolor{red}
In this section, we present a closed-loop simulation environment for simulating and studying MAVs. We show how our setup captures MAV robot complex, i.e., MAV subsystems and their components and further their interactions in a closed-loop setup. We describe the knobs that our simulator supports to enable exploratory studies for cyber-physical co-design.
We also describe how the simulator models mission metrics such as energy consumption, in addition to functionality and performance.

\subsection{Simulation Setup}
\label{sec:setup}
Closed-loop operation is an integral component of autonomous MAVs. As described previously in \Sec{sec:background}, in such systems, the data flow in a (closed) loop, starting from the environment, going through the MAV and back to the environment, as shown in \Fig{fig:Aerial_agent_data_flow}. The process involves sensing the environment (Sensors), interpreting it and making decisions (Compute), and finally navigating within or modifying the
environment (Actuators) in a loop. In this section, 
we show how our simulation setup, shown in \Fig{fig:end-to-end}, maps to the various components corresponding to a MAV robot complex. Furthermore, we discuss the simulator's ability to capturing various cyber and physical quantities. 

\begin{figure}[t!]
\centering
\includegraphics[trim= 10 10 10 10, clip, width=0.75\columnwidth]{figs/end-to-end-simulation}
\caption{Architectural overview of our closed-loop simulation. 
%\red{change airsim to UNREAL + Airsim: possibly annotate them with env and MAV (maybe even sensors/actuators)}}
}
\label{fig:end-to-end}
\end{figure}

\paragraph{Environments, Sensors and Actuators:} Environments, sensors and actuators are simulated with the help of a game engine called Unreal~\cite{GameEngi70:online}. With a physics engine at its heart, it ``provides the ability to perform accurate collision detection as well as simulate physical interactions between objects within the world''~\cite{PhysicsS8:online}. Unreal provides a rich set of environments such as mountains, jungles, urban setups, etc. to simulate.

To simulate MAV's dynamics and kinematics, we used AirSim, an open-source Unreal based plug-in from Microsoft~\cite{Airsim:online,Airsim_paper}. Through AirSim we can study the impact of drone's physical quantities such as velocity and acceleration. We limit our sensors and actuators to the ones realistically deployable by MAVs, such as \mbox{RGB-D} cameras and IMUs. Unreal and Airsim run on a powerful computer (host) capable of physical simulation and rendering. Our setup uses an Intel Core i7 CPU and a high-end NVIDIA GTX 1080 Ti GPU.  

\paragraph{Flight Controller:} AirSim supports various flight controllers that can be either hardware-in-the-loop or completely software-simulated. For our experiments, we chose the default software-simulated flight controller provided by AirSim. However, AirSim also supports other FCs, such as the Pixhawk~\cite{Pixhawk:online}, shown in black in \Fig{fig:end-to-end} which runs the PX4~\cite{PX4Archi7:online} software stack. AirSim supports any FC which can communicate using MAVLINK, a widely used micro aerial vehicle message marshaling library~\cite{mavlinkm68:online}. %MAVLINK is supported as the communication protocol by an extensive number of autopilot systems.
%\red{we should somehow here or later mention that we actually are using the airsim's simple FC instead of pixhawk}


\paragraph{Companion Computer:} We used an NVIDIA Jetson TX2~\cite{TX2}, a high-end embedded platform from Nvidia with 256 Pacal CUDA cores GPU and a Quad ARM CPU; however, the flexibility of our setup allows for swapping this embedded board with others such as x86 based Intel Joule~\cite{joule:online}. TX2 communicates with Airsim and also FC via Ethernet. Note that the choice of the companion computer influences both cyber and physical quantities such as response time and compute mass. 

\paragraph{ROS:} Our setup uses the popular Robot Operating System (ROS) for various purposes such as low-level device control and inter-process communication~\cite{ROSorgPo80:online}.
Robotic applications typically consist of many concurrently-running processes that are known as ``nodes.'' For example, one node might be responsible for navigation, another for localizing the agent and a third for object detection. ROS provides peer-to-peer communication between nodes, either through blocking ``service'' calls, or through non-blocking FIFOs (known as the Publisher/Subscriber paradigm). % A Master node registers all other nodes in a table, allowing the communication to take place. 

\paragraph{Workloads:} Our workloads runs within the ROS runtime on TX2. Briefly, we developed five distinct workloads, each representing a real world usecase: agricultural scanning, aerial photography, package delivery, 3D mapping and search and rescue. They are extensively discussed in \Sec{sec:benchmarks}.

\paragraph{Putting It All Together:} To understand the flow of data, we walk the reader through a simple workload where the MAV is tasked to detect an object and fly toward it. The object (e.g., a person) and its environment (e.g., urban) are modeled in the Unreal Engine. As can be seen in \Fig{fig:end-to-end}, the MAV's sensors (e.g., accelerometer and \mbox{RGB-D} Camera), modeled in Airsim, feed their data to the flight controller (e.g., physics data to PX4) and the companion computer (e.g., visual and depth to TX2) using MAVLink protocol. The kernel (e.g., object detection), running within the ROS runtime environment on the companion computer, is continuously invoked until the object is detected. Once so, flight commands (e.g., move forward) are sent back to the flight controller, where they get converted to a low-level rotor instruction stream flying the MAV closer to the person. 

%\textbf{Profiling of cyber and physical quantities}
\subsection{Simulation Knobs and Extensions}
\label{sec:knobs}

With the help of Unreal and AirSim, our setup exposes a wide set of knobs. Such knobs enable the study of agents with different characteristics targeted for a range of workloads and conditions. For different environments, the Unreal market provides a set of maps free or ready for purchase. Furthermore, by using Unreal programming, we introduce new environmental knobs, such as (static) obstacle density, (dynamic) obstacle speed, and so on. In addition, Unreal and AirSim allow for the MAV and its sensors to be customized. For example, the cameras' resolution, their type, number, and positions all can be tuned according to the workloads' need.   

Our simulation environment can be extended. For the compute on edge, the TX2 can be replaced with other embedded systems or even micro-architectural simulators, such as gem5. Sensors and actuators can also be extended, and various noise models can be introduced for reliability studies. 

\subsection{Energy Simulation and Battery Model}
\label{sec:energy}
%\cite{dji-matrice}
We extended the AirSim simulation environment with an energy and a battery model to collect mission energy data in addition to mission time. Our energy model is a function of the velocity and acceleration of the MAV~\cite{energyaware}.  The higher the velocity or acceleration, the higher the amount of energy consumption. Velocity and acceleration values are sampled continuously, their associated power calculated and integrated for capturing the total energy consumed by the agent.

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

We used a parametric power estimation model proposed in \cite{3DR-energy-model}. The formula for estimating power $P$ is described below:%
\begin{equation}
\begin{aligned}
P = \begin{bmatrix}
        \beta_{1} \\
        \beta_{2} \\
        \beta_{3}
    \end{bmatrix}^{T}
    \begin{bmatrix}
        \norm{\vec{v}_{xy}} \\
        \norm{\vec{a}_{xy}} \\
        \norm{\vec{v}_{xy}}\norm{\vec{a}_{xy}}
    \end{bmatrix}
    +
    \begin{bmatrix}
        \beta_{4} \\
        \beta_{5} \\
        \beta_{6}
    \end{bmatrix}^{T}
    \begin{bmatrix}
        \norm{\vec{v}_{z}} \\
        \norm{\vec{a}_{z}} \\
        \norm{\vec{v}_{z}}\norm{\vec{a}_{z}}
    \end{bmatrix}
    +
    \begin{bmatrix}
        \beta_{7} \\
        \beta_{8} \\
        \beta_{9}
    \end{bmatrix}^{T}
    \begin{bmatrix}
        m \\
        \vec{v}_{xy} \cdot \vec{w}_{xy} \\
        1
    \end{bmatrix}
\end{aligned}
\label{eqn:power}
\end{equation}

In the Equation~\ref{eqn:power}, $\beta_{1}$, ..., $\beta_{9}$ are constant coefficients determined based on the simulated drone. $\vec{v}_{xy}$ and $\vec{a}_{xy}$ are the horizontal speed and acceleration vectors whereas  $\vec{v}_{z}$ and $\vec{a}_{z}$ are the corresponding vertical values. $m$ is the mass and $\vec{w}_{xy}$  is the vector of wind movement. 

We have a battery model that implements a coulomb counter approach~\cite{coulomb-counter}. The simulator calculates how many coulombs (product of current and time) have passed through the drone's battery over every cycle. This is done by calculating the power and the voltage associated with the battery. The real-time voltage is modeled as a function of the percentage of the remaining coulomb in the battery as described in ~\cite{battery-model}. \Sec{sec:comp_mission_energy}
 presents experimental results for a 3DR Solo MAV.

\subsection{Simulation Fidelity and Limitations}
\label{sec:accuracy}

The fidelity of our end-to-end simulation platform is subject to different sources of error, as it is with any simulation setup. The major obstacle is the \textit{reality gap}---i.e., the difference between the simulated experience and the real world. This has always posed a challenge for robotic systems. The discrepancy results in difficulties where the system developed via simulation does not function identically in the real world. 
To address the reality gap, we iterate upon our simulation components and discuss their fidelity and limitations. Specifically, this involves (1) simulating the environment, (2) modeling the drone's sensors and flight mechanics, and last but not least (3) evaluating the compute subsystem itself.

First, the Unreal engine provides a high fidelity environment. By providing a rich toolset for lighting, shading, and rendering, photo-realistic virtual worlds can be created. In prior work~\cite{unrealcv}, authors examine photorealism by running a Faster-RCNN model trained on PASCAL in an Unreal generated map. The authors show that object detection precision can vary between 1 and 0.1 depending on the elevation and the angle of the camera. Also, since Unreal is open-sourced, we programmatically emulate a range of real-world scenarios. For example, we can set the number of static obstacles and vary the speed of the dynamic ones to fit the use case.   

Second, AirSim provides high fidelity models for the MAV, its sensors, and actuators. Embedding these models into the environment in a real-time fashion, it deploys a physics engine running with 1000~\si{\hertz}.  As the authors discuss in~\cite{Airsim_paper}, the high precision associated with the sensors, actuators, and their MAV model, allows them to simulate a Flamewheel quadrotor frame equipped with a Pixhawk~v2 with little error. 
Flying a square-shaped trajectory with sides of length 5~\si{\meter} and a circle with a radius of 10~\si{\meter},  AirSim achieves  0.65~\si{\meter} and 1.47~\si{\meter} error, respectively. Although they achieve high precision, the sensor models, such as the ``camera lens models,'' ``degradation of GPS signal due to obstacles,'' ``oddities in camera,'' etc. can benefit from further improvements. %\red{somewhere we should mention that we extended airsim to use DJI Matrice}

Third, as for the compute subsystem itself, our hardware has high fidelity since we use off-the-shelf embedded platforms for the companion computer and flight controller. As for the software, ROS is widely used and adopted as the \textit{de facto} middleware software in the robotics research community.

%The details of the simulation environment components' precisions resulting in the aforementioned error is further discussed in~\cite{Airsim_paper}.

%\subsection{Simulation Limitations}
%\label{sec:limits}

%\paragraph{Network Bottleneck:} As was previously mentioned, our companion computer and Airsim are connected through Ethernet. Hence, transferring multiple high-resolution images can be throttled by the cable's bandwidth. 

\begin{comment}
Using such data, one can define  various metrics for the applications of interest. For example, using time to delivery over the amount of energy spent, one can define an efficiency metric for a package delivery application. Metrics are extensively discussed in the section \ref{MAVBench characterization}.
\end{comment}
\begin{comment}
\begin{figure*}[h]
\centering
\includegraphics[width=.3\linewidth]{figs/blank}
\includegraphics[width=.3\linewidth]{figs/blank}
\includegraphics[width=.3\linewidth]{figs/blank}
\caption{Show a picture of what AirSim is doing and what the "MAV" is seeing.}
\label{fig:end-to-end}
\end{figure*}
\end{comment}

\begin{comment}

\subsection{Workloads} \label{ssec:benchmarks}

\red{here we explain the workloads we are using for our study, going into the details of each and perhaps even explaining what computational kernels they are exercising. the table of the workloads should discuss the internal details of th apps.}

Our workloads are organized into a full benchmark suite that tests a MAV's ability to perform the tasks required for popular MAV applications today as well as MAV applications that are expected to become significant in the near-future.

Our benchmark suite is divided into two categories: a set of micro-benchmarks that test narrow MAV capabilities and a set of macro-benchmarks that test full MAV applications.

\subsubsection{Micro-benchmarks} \label{sssec:micro}

Our micro-benchmarks test a MAV's ability to execute tasks that would be part of a full MAV application, such as computational kernels or simple flight maneuvers. The micro-benchmarks themselves, however, do not represent complete MAV applications.

The micro-benchmarks primarily stress a MAV's computer vision, SLAM, and pathfinding capabilities. A few of the micro-benchmarks do not test any computational capabilities at all but are instead meant to characterize a MAV's power consumption during flight. Our micro-benchmarks are listed in full in Table~\ref{tab:micro}.




\subsubsection{Macro-benchmarks} \label{sssec:macro}

Our macro-benchmarks, described in Table~\ref{tab:macro} are complete MAV applications that characterize a MAV's performance and power consumption when performing typical MAV applications. The macro-benchmarks are made up the smaller kernels that are tested by the micro-benchmarks described in Sec.~\ref{sssec:micro}.

\begin{table*}[h!]
\begin{tabular*}{\textwidth}{l@{\extracolsep{\fill}}lllll}
\hline
Benchmark & Use Case & Kernel(s)\\\hline
\texttt{outdoor\_track} & Target tracking (sports photography) & Computer vision; object detection \\
\texttt{indoor\_track} & Target tracking (indoors) & Computer vision; object detection \\
\texttt{deliver} & Package delivery & Pathfinding; SLAM; computer vision \\
\texttt{search} & Search and rescue & Computer vision; object detection; SLAM \\
\texttt{survey} & Land surveying & \fxnote{nothing really} \\
\texttt{map} & Mapping a building & Computer vision; image stitching \\
\texttt{data\_coverage} & Wireless data coverage & \fxnote{?} \\
\texttt{driving} & Autonomous navigation & Machine learning \\
\texttt{take\_picture} & Go to target address, take picture, and return & Path planning \\
\hline
\end{tabular*}
\caption{Macro-benchmarks.}
\label{tab:macro}
\end{table*}

\subsection{Platforms} \label{ssec:MAVs}

\red{here we provide the specific platforms we have evaluated, and for the most part these will be the architectural capabilities of the compute boards that corresponds to our different MAV platforms.}

% Description of our MAV platforms, including a table giving details on each one's weight, flight controller, etc.

We characterize a variety of MAV processors and MAV platforms, both physical and simulated, using our benchmark suite. Our power characterizations are based primarily upon our physical MAVs, described in Table~\ref{tab:MAV-platforms}. Our performance characterizations are primarily based upon workloads run on a simulated MAV known as Microsoft AirSim~\cite{}, rather than on physical MAV platforms.

\paragraph{Processors} We run our computational workloads on a variety of embedded processors, described in Table~\ref{}, that are targeted towards MAVs and robotics applications. These range from state-of-the-art embedded systems with powerful CPUs and hundreds of GPU cores all the way to smartphone-level processors such as the i.MX6 with much lower performance capabilities.

\begin{table*}[t!]
\centering
\caption{Companion computer characteristics.}
\label{tab:cc-platforms}
\begin{tabular}{ l | c c c c c }
 \hline \noalign{\vskip 0.5mm}
 & Intel Aero & Jetson TX1 & Intel Joule & i.MX6 Solo & ODroid  \\
 \hline \noalign{\vskip 0.5mm}
 % SOC        & Intel Atom 7-Z8750 & \\
 CPU        & Intel Atom 7-Z8750 & ARM Cortex-A57 & Intel Atom T5700 & ARM Cortex A9 \\
\ \ Frequency    & 1.60 GHz & \fxnote{Unpublished} & 1.7 GHz & 1 GHz \\
\ \ L1 \$ (I/D) & 226 KiB & 80 KB & \fxnote{Unknown}  & 64 KB \\
\ \ L2 \$ (I/D) & 2 MiB & 2 MB  & 2x2 MB & 512 KB \\
\ \ Cores     & 4 & 4 & 4 & 1 \\
 GPU        & Intel HD Graphics 405 & 256-core Maxwell GPU & Intel HD Graphics & Two integrated 3D and 2D GPUs\\
 RAM        & 4 GB LPDDR3 & 4 GB LPDDR4 & 4 GB LPDDR4 & 512 MB \\
 OS         & Yocto 2.1 (Linux 4.4.3) & Ubuntu 16.04 & Ubuntu 16.04 & 3DR Poky (based on Yocto) \\
 \hline
\end{tabular}
\end{table*}

\paragraph{Physical MAVs} We characterized the power consumption of MAVs ranging from X to Y lbs in weight. We investigated MAVs of different weights because a MAV's weight strongly affects its power consumption and is also correlated to its maximum payload, which determines the weight of the components that can be placed upon it. 

% \paragraph{Microsoft AirSim} A simulated MAV with realistic video data. The setup is illustrated in Fig.~\ref{fig:end-to-end}.

\paragraph{Microsoft AirSim} AirSim is an HIL simulator of a micro-aerial vehicle that was developed to allow machine learning applications to easily and safely generate training data for their MAVs. AirSim runs on the Unreal engine and is thus capable of generating realistic video data for our MAV applications. Thus, AirSim allows us to develop realistic environments for our macro-benchmarks so that our characterizations can be easily run on MAV processors in a safe and repeatable fashion. The interfacing between our workloads, MAV processors, and AirSim itself in illustrated in Fig.~\ref{fig:end-to-end}.

\end{comment}


==> tex/software_pipeline.tex <==
High-level software pipeline associated with our (though not exclusive to it) workloads are shown in figure blah. 

\textbf{perception stage:}
Perception is defined as "the task- oriented interpretation of sensor data" ~\cite{Handbook_robotic}. Inputs to this stage, the sensory data (e.g. GPS) and a partial model of the environment (voxel map), are fused to develop a more elaborate model (e.g. improved voxel map) in order to extract the drone's and environment's relevant states (e.g. position of obstacles around the drone). 

\textbf{Planning:}
Using the inputs (e.g. voxel map) from the perception stage, the next two steps (namely planning and control) provide a motion generation framework \footnote{Our benchmark suit solely focuses on motion planning}. Planning involves generating (usually) a \textit{collision-free} to a target. In a nutshell, this step involves first generating a set of possible paths to the target (e.g. PRM) and then choosing an optimal one among them using a a path-planning algorithm (e.g. A*). 


\textbf{Control:}
This stage is about achieving a desired path (provided from the previous stage) while providing a set of guarantees such as feasibility, stability and robustness~\cite{tech_problem}. In this stage, drones dynamics are considered and flight commands are generated while ensuring the aforementioned guarantees.  


==> tex/suite.tex <==
\section{Benchmarking Suite}



Our benchmarking suite tests the performance of drones when executing a diverse set of tasks that are either commonly executed by drones today or that are being vigorously researched.

Our benchmarking suite is made of various workloads that are split into two categories: micro-benchmarks and macro-benchmarks. Micro-benchmarks test the capability of a drone to execute a single, very narrow task that may be used as a kernel in many other, larger applications. Macro-benchmarks test the capability of a drone to execute a complete mission, such as delivering a package or searching for and rescuing a person in need.

Our benchmarking suite records the speed with which a drone is able to complete a task, and the power it consumes in doing so, as well as certain measures that are specific to the workload being run.

\subsection{Micro-benchmarks}

\subsection{Macro-benchmarks}


==> tex/sys-arch.tex <==
\section{System Architecture} % Maybe change to "simulation architecture"

\begin{comment}
\begin{figure}[t]
\centering
\includegraphics[width=6cm, height=4cm ,keepaspectratio]{figs/robot_arch.png}
\caption{System architecture of a typical robotic agent.}
\end{figure}
\end{comment}
%In this section, we provide an architectural overview of typical drone platforms in order to provide the background necessary to understand their architectural constraints, and the requirements for a simulator that can provide insights into those constraints.

% \textcolor{red}{Like any other robotic systems, drones have 3 subsystems: ....}
%\subsection{Accuracy Impact:}
\begin{figure}[t!]
\centering
\includegraphics[width=0.9\columnwidth]{figs/agent_env.pdf}
\vspace{1.0ex}
\caption{Agent-environment model.}
\vspace{-3ex}
\label{fig:1}
\end{figure}
Given the aforementioned constrains, these agents demand architects attention. In this section, we provide the architectural overview of such agents as the first step toward a design around such constrains.  

Like other robotic agents, such systems operate by sampling the environment state, interpreting and reacting to it using three main subsystems, namely, a sensory subsystem, a perception subsystem, and an actuation subsystem. Fig.~\ref{} shows these subsystems and their corresponding data and energy flow. More concretely, Fig.~\ref{} shows the details of each subsystem \textcolor{red}{(have various sensors and actuator names on the figure.)}
\begin{comment}
\begin{figure}
\includegraphics[width=6cm, height=4cm ,keepaspectratio]{figs/drone_arch.png}
\caption{Detailed system architecture of an aerial robotic agent.}
\end{figure}
\end{comment}
\begin{comment}
Sensor subsystem: is usually comprised of a versatile set of sensors such as cameras, IMU (inertial measurement units), IR, lidar, etc depending on size, energy budget and other constraints.
Perception subsystem: This system is responsible for processing the sampled data. typical off-the-shelf UAVs, such as the 3DR Solo, are equipped with at least two onboard processors: a ``companion computer'' that handles workloads, and a ``flight controller'' responsible for high to low (and vice versa) conversion of sensing and actuation subcommands (e.g. conversion of hover (high level) command to specific rotor speed (low level)).
Actuation subsystem: this system is responsible for reacting and modifying the world around the agent. It ranges anywhere from rather simple rotors to robotic arms capable of grasping and lifting objects. 
}


\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/drone-architecture}
\caption{Architectural overview of a typical drone platform. \textcolor{red}{Iterate over this figure; it should be improved.}}
\label{fig:dronearch}
\end{figure}
\end{comment}

\textbf{Sensory Subsystem} To enable intelligent flight, drones must be equipped with a rich set of sensors that are capable of gathering visual, depth, position, and orientation data. For example, to detect possible intruders and separate them from authorized visitors, an autonomous security drone will require image data from cameras. To detect the positions of obstacles, a drone would also require depth information from stereo or RGBD cameras. Number and type of sensors is highly dependent on the workload requirement such as, and various system constraints such as perception subsystem capability to process them. 

\textbf{Perception Subsystem} To enable intelligent flight, drones must also come equipped with onboard companion computers that are capable of performing high-level cognitive \textcolor{red}{(this probably isn't the right word here)} tasks, such as object classification and obstacle avoidance. Such processors must satisfy various constraints such as drone's thermal and energy limit,form factor, etc. Therefore, many off-the-shelf drone platforms such as the Solo come equipped with small, low-power processors such as the ARM Cortex-M A9 that struggle to provide real-time cognitive capability for compute-heavy tasks such as visual classification. For higher performance, UAV designers can turn to other state-of-the-art embedded systems such as the NVIDIA TX2, although these systems incur higher power penalties. In addition to the companion computers, typically, drone platforms come with a ``flight controller'' responsible for high to low (and vice versa) conversion of sensing and actuation subcommands (e.g. conversion of hover (high level) command to specific rotor speed (low level).

\textbf{Actuation Subsystem} This system is responsible for reacting and modifying the world around the agent. It ranges anywhere from rather simple rotors to robotic arms capable of grasping and lifting objects.
Similar to sensors, their type and number is highly a function of the workload and processing power on board. 


==> tex/todos.tex <==
1. be consistent across applications for collecting the maximum allowed velocity
2. run more experiments per applications
3. what element of compute matters (improve on the heat map) and draw conclusions about whether concurrency and so on matters?
4. integrate slam. 
5. table is not clear.

6. related work include an optimization works (such as slam and knobs) 
7. related work: the duke paper (the start up)
8. cite Jason Clemons http://www.eecs.umich.edu/eecs/about/articles/2012/Clemons-NVIDIA.html


